Fashion Meets Computer Vision: A Survey

Fashion is the way we present ourselves to the world and has become one of the world's largest industries. Fashion, mainly conveyed by vision, has thus attracted much attention from computer vision researchers in recent years. Given the rapid development, this paper provides a comprehensive survey of more than 200 major fashion-related works covering four main aspects for enabling intelligent fashion: (1) Fashion detection includes landmark detection, fashion parsing, and item retrieval, (2) Fashion analysis contains attribute recognition, style learning, and popularity prediction, (3) Fashion synthesis involves style transfer, pose transformation, and physical simulation, and (4) Fashion recommendation comprises fashion compatibility, outfit matching, and hairstyle suggestion. For each task, the benchmark datasets and the evaluation protocols are summarized. Furthermore, we highlight promising directions for future research.

==> ACMCSUR – Fashion/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> ACMCSUR – Fashion/src/abstract.tex <==
\begin{abstract}
Fashion is the way we present ourselves to the world and has become one of the world's largest industries. Fashion, mainly conveyed by vision, has thus attracted much attention from computer vision researchers in recent years. Given the rapid development, this paper provides a comprehensive survey of more than 200 major fashion-related works covering four main aspects for enabling intelligent fashion: (1) Fashion detection includes landmark detection, fashion parsing, and item retrieval, (2) Fashion analysis contains attribute recognition, style learning, and popularity prediction, (3) Fashion synthesis involves style transfer, pose transformation, and physical simulation, and (4) Fashion recommendation comprises fashion compatibility, outfit matching, and hairstyle suggestion. For each task, the benchmark datasets and the evaluation protocols are summarized. Furthermore, we highlight promising directions for future research.


%--------------------------original-----------------------------
%Fashion, mainly conveyed by vision, has attracted more attention from computer vision researchers recently. Given the rapid development, this paper provides a comprehensive survey of more than 200 major fashion-related works covering four main aspects: (1) Fashion detection includes landmark detection, fashion parsing, and item retrieval, (2) Fashion analysis contains attribute recognition, style learning, and popularity prediction, (3) Fashion synthesis involves style transfer, pose transformation, and physical simulation, and (4) Fashion recommendation comprises fashion compatibility, outfit matching, and hairstyle suggestion. For each task, the benchmark datasets and the evaluation protocols are summarized. Furthermore, we highlight promising directions for future research.



%Fashion, which is mainly conveyed by vision, has attracted more attention from computer vision researchers in recent years. Many technologies have been developed to detect fashion, analyze fashion, synthesis fashion and recommend fashion, which takes a step further to benefit our daily life. Given these rapid development, this paper aims to provide a comprehensive survey of the recent advances of computer vision methods in fashion domain. More than 200 major publications from the top conferences and journals are included in this survey covering many aspects of fashion, from fundamental research to application frameworks, including fashion image detection, retrieval, human clothing segmentation, analysis, synthesis, and the recommendation applications. The benchmark datasets for each task are also summarized and compared. Furthermore, we highlight some promising directions for future research.

%We believe this survey will provide researchers and practitioners a comprehensive view on the state-of-the-art artificial intelligence for visual fashion computation studies and facilitate the process of expanding this research field.
\end{abstract}


==> ACMCSUR – Fashion/src/applications.tex <==
\section{Applications and Future Work}
\label{sec:application}

%Fashion always keeps moving.
The future of the fashion world will be shaped in large part by advancements in the technology, which is currently creeping into the creative domains by starting to mimic human neurons. In the following, we discuss emerging uses of fashion technology in some application areas and future work that is needed to achieve the promised benefits.

\subsection{Applications}

The most popular AI application from the top global apparel industry leaders 
%\footnote{\url{https://www.forbes.com/pictures/592331454bbe6f1b730a8fae/2017-global-2000-apparel/#2c75336f6372}} 
currently implementing AI appears to be AI chatbots, also called smart assistants, which is used to interact with their customers. The common use-cases that are covered are: (1) Responding to customer service inquiries and providing suggestions related to product searches through a social media messaging platform, \textit{e.g.}, ``Dior Insider'', (2) Helping customers navigate products online or in-store to find product(s) that align with their interests, \textit{e.g.}, ``Levi's Virtual Stylist'', ``VF Corporation'', ``Macy's On Call'', and ``Nordstrom'', and (3) Virtual assistant to encourage exercise/behavior adherence, \textit{e.g.}, ``Nike on Demand''.

Moving forward, AI technology will have explosive growth to power fashion industry. In addition to connecting with the customers with the use of AI chatbots, we identify there are four other ways that AI is transforming the future of fashion and beauty, which include: (1) \textbf{Improving product discovery.} Visual search makes it easier for shoppers to find, compare, and purchase products by taking or uploading a photo. One example is Google Lens\footnote{\url{https://lens.google.com}} that allows mobile users to perform searches for similar styles through Google Shopping from the photos they take. (2) \textbf{Tailor recommendation.} In order to keep costs low, brands need to better predict customer preferences by gathering and analyzing purchase behavior, customer profile, as well as customer feedback. Using this data alongside AI and machine learning allows fashion retailers to deliver a personalized selection of clothes to customers. Stitch Fix\footnote{\url{https://www.stitchfix.com}} is one of the most popular AI fashion companies in this category. (3) \textbf{Reducing product return.} Customers have more options to choose from than ever when it comes to making purchases. To gain the loyalty of the consumers, one recent focus of the fashion retailer has been to extend an excellent customer service experience not only at the point of purchase but at the point of return as well. AI technology has the power to better engage customers with the personalized shopping experience that leads them to make more informed and confident purchase decisions, which in turn helps retailers lower return rates. Sephora\footnote{\url{https://www.sephora.com}} is an example of a retailer that has developed this strategy. (4) \textbf{Powering productivity and creativity.} The promise of AI for fashion brands that can marry design creativity with digital innovation has a powerful competitive advantage in the market. The AI technology enables fashion brands to sift through consumer data to gain insights on which product features their customers are likely to prefer. 
%\begin{itemize}
%    \item \textbf{Improving product discovery.} %Another AI-powered retail trend, 
%    Visual search makes it easier for shoppers to find, compare, and purchase products by taking or uploading a photo. One example is Google Lens\footnote{\url{https://lens.google.com}} that allows mobile users to perform searches for similar styles through Google Shopping from the photos they take.
%    \item \textbf{Tailor recommendation.} In order to keep costs low, brands need to better predict customer preferences by gathering and analyzing purchase behavior, customer profile, as well as customer feedback. Using this data alongside AI and machine learning allows fashion retailers to deliver a personalized selection of clothes to customers. Stitch Fix\footnote{\url{https://www.stitchfix.com}} is one of the most popular AI fashion companies in this category.
%    \item \textbf{Reducing product return.} Customers have more options to choose from than ever when it comes to making purchases. To gain the loyalty of the consumers, one recent focus of the fashion retailer has been to extend an excellent customer service experience not only at the point of purchase but at the point of return as well. AI technology has the power to better engage customers with the personalized shopping experience that leads them to make more informed and confident purchase decisions, which in turn helps retailers lower return rates. Sephora\footnote{\url{https://www.sephora.com}} is an example of a retailer that has developed this strategy.
    %\item \textbf{Inventory management.} Having effective and accurate inventory management is crucial for any apparel brand. Also, brands need to be able to predict demand. AI-powered tools for demand forecasting use machine learning algorithms by analyzing historical data to make predictions and choices automatically.
    %Having effective and accurate inventory management is crucial for any apparel brand. This can help with efficiency and in turn create greater customer satisfaction. To do this, brands need to be able to predict demand. AI-powered tools for demand forecasting use machine learning algorithms by analyzing historical data to make predictions and choices automatically.
%    \item \textbf{Powering productivity and creativity.} The promise of AI for fashion brands that can marry design creativity with digital innovation has a powerful competitive advantage in the market. The AI technology enables fashion brands to sift through consumer data to gain insights on which product features their customers are likely to prefer. 
%\end{itemize}


%\subsection{Fashion and Beauty Assessment}

%There are many difficulties in comparing the performance of different models, both generally and in particular tasks. The difficulties arise from several sources, including: (1) The use of different evaluation metrics in the different studies severely hinders a direct comparison of model performance to identify the most effective approach to a given purpose. This problem also raises the question of whether the differences in performance reported are sufficient to indicate the real differences in the model ability. (2) The absence of a standardized dataset specifically tailored for particular tasks results in difficulty in verifying the significance of the model. In addition, this makes it unclear whether the results are sufficiently general to predict the results of similar tests using a different dataset. (3) The differences in modalities used to assess the function of particular frameworks.


%\begin{itemize}
%    \item The use of different evaluation metrics in the different studies severely hinders a direct comparison of model performance to identify the most effective approach to a given purpose. This problem also raises the question of whether the differences in performance reported are sufficient to indicate the real differences in the model ability.
%    \item The absence of a standardized dataset specifically tailored for particular tasks results in difficulty in verifying the significance of the model. In addition, this makes it unclear whether the results are sufficiently general to predict the results of similar tests using a different dataset. 
%    \item The differences in modalities used to assess the function of particular frameworks.
%\end{itemize}


%The solutions that we believe will be able to meet the above challenges are as follows: (1) Consider a broad range of metrics in model evaluation, which not only provide statistically significant results but also allow to gain in-depth insight on model behavior. (2) Provide a unified benchmark dataset that serves as a standard reference to enable researchers to compare their algorithms. (3) For a fair comparison among different models on each topic, there is a need for a public evaluation server to report evaluation results automatically on a preserved test set.


%\begin{itemize}
%    \item Consider a broad range of metrics in model evaluation, which not only provide statistically significant results but also allow to gain in-depth insight on model behavior.
%    \item Provide a unified benchmark dataset that serves as a standard reference to enable researchers to compare their algorithms.
%    \item For a fair comparison among different models on each topic, there is a need for a public evaluation server to report evaluation results automatically on a preserved test set.
%\end{itemize}

%\subsection{Human Body Parameters Modeling}

%Knowledge about the human body is essential for boosting fashion and beauty analysis. The success of previous studies has proven the potential of modeling the human body as a knowledge base to represent the informative semantic parts of fashion and beauty items. However, parameters modeling the human body with large-scale pose variations is still an open problem that needs both theoretical and experimental exploration. 


\subsection{Break the Limitations of Annotation}

Large-scale data annotation with high quality is indispensable. However, current studies are mainly based on relatively small-scale datasets, which is usually constrained by annotation costs and efforts. Faced with such enormous amounts of fashion and beauty related data, how to generate high coverage and high precision annotations to considerably reduce the cost while preserving quality remains a hot issue. Therefore, more efforts in the development of cost-effective annotations approach on fashion and beauty related data are necessary to address the problem.

\subsection{Overcome the Industry Challenges}

There are still many challenges in adopting fashion and beauty technologies in industry because real-world fashion and beauty are much more complex and strict than in the experiments. The main issue is related to system performance which is still far from human performance in real-world settings. The demand for a more robust system consequently grows with it. Accordingly, it is crucial to continue to pay attention to handling data bias and variations to improve the true-positive rate while maintaining a low false-positive rate. Moreover, with the rising interest in mobile applications, there is a definite need to perform the task in a light but timely fashion. It is thus also beneficial to consider how to optimize the model to achieve higher performance and better computation efficiency.



\begin{comment}
Uniform the benchmark: outfit matching and retrieval. There is no unified benchmark.
Assessment for fashion generation. 

http://dbgroup.cs.tsinghua.edu.cn/ligl/papers/vldb19-crowd.pdf
https://pdfs.semanticscholar.org/daa7/a19e8fdeb7ae475e7a2f7e27d18ccafaf8c2.pdf

https://arxiv.org/pdf/1707.07435.pdf
Q. Fang, J. Sang, and C. Xu, “Giant: Geo-informative attributes for location recognition and exploration,” in Proceedings of the 21st ACM international conference on Multimedia. ACM, 2013, pp. 13–22.

The main challenge in automated methods for face attractiveness computation is the development
of accurate models for predicting the score from an image.

%Due to ubiquity of fashion and clothing, it is important that the dataset is collected from general user-contributed images to cover a broad range of clothing and fashion items from diﬀerent social spheres.

Recently there have been a lot of works on generative image modeling with deep learning techniques.
These works fall into two categories. 

The  process  of  generating  realistic-looking  images  of
persons has several applications, like image editing, person
re-identification (re-ID), inpainting or on-demand generated
art for movie production. 

[ChenECCV2012]
Attribute prediction technique has a great impact on many emerging applications, such as customer profile analysis for shopping recommendations. With a collection of personal or event photos, it is possible to infer the dressing style of the per- son or the event by analyzing the attributes of clothes, and subsequently make shopping recommendations. The application of dressing style analysis is shown in Fig.9.
Another important application is context-aware person identification, where many researchers have demonstrated superior performance by incorporating clothing infor- mation as a contextual cue that complements facial features [2–4]. Indeed, within a certain time frame (i.e., at a given event), people are unlikely to change their clothing. By accurately describing the clothing, person identification accuracy can be improved over conventional techniques that only rely on faces. In our study, we also found that clothing carry significant information to infer the gender of the wearer. This observa- tion is consistent with the prior work of [5, 6], which exploits human body information to predict gender. Consequently, a better gender classification system can be developed by combining clothing information with traditional face-based gender recognition al- gorithms.

[ChenCVPR2015]
criminal investigation processes often involve searching for suspects based on detailed descriptions provided by eyewitnesses or compiled from images captured by surveillance cameras. The FBI list of nationwide wanted bank robbers\footnote{https://bankrobbers.fbi.gov/} has clear examples of such fine-grained descriptions, including attributes covering detailed color information (e.g., “light blue” “khaki”, “bur- gundy”), a variety of clothing types (e.g., ‘leather jacket”, “polo-style shirt”, “zip-up windbreaker”) and also detailed clothing patterns (e.g., “narrow horizontal stripes”, “LA printed text”, “checkered”).

http://openaccess.thecvf.com/content_ECCV_2018/papers/Amit_Raj_SwapNet_Garment_Transfer_ECCV_2018_paper.pdf

There are many interesting applications derived from this task. For example, in movie making, we can directly manipulate a character’s human body to a desired pose or, for human pose estimation, we can generate training data for rare but important poses.

https://www.researchgate.net/publication/289833793_DBpediaNYD_-_A_silver_standard_benchmark_dataset_for_semantic_relatedness_in_DBpedia

\end{comment}


==> ACMCSUR – Fashion/src/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

With the significant advancement of information technology, research in computer vision (CV) and its applications in fashion have become a hot topic and received a great deal of attention% from both researchers and practitioners
. Meanwhile, the enormous amount of data generated by social media platforms and e-commerce websites provide an opportunity to explore knowledge %that is 
relevant to support the development of intelligent fashion %analysis 
techniques. Arising from the above, there has much CV-based fashion technology been proposed to handle the problems of fashion image detection, analysis, synthesis, recommendation, and its applications. The long-standing semantic gap between computable low-level visual features and high-level intents of customers now seems to be narrowing down. Despite recent progress, investigating and modeling complex real-world problems when developing intelligent fashion solutions remain challenging. Given the enormous profit potential in the ever-growing consumer fashion and beauty industry, the studies on intelligent fashion-related tasks will continue to grow and expand. 


==> ACMCSUR – Fashion/src/fashion_analysis.tex <==
\section{Fashion Analysis}
\label{sec:fashion_analysis}




\subsection{Fashion Modelling}



\subsubsection{State-of-the-art methods}



\subsubsection{Benchmark datasets}

%Each study in this task has developed its own dataset varying in the number, modality, and attractiveness score. A summary of characteristics of the benchmark datasets is presented in Table~\ref{tab:modeling_fashionbeauty_datasets}.

%\begin{table*}[t!]
%\footnotesize
%    \centering
%        \caption{Summary of the benchmark datasets for modeling fashion/beauty task.}
%        \vspace{-3mm}
%    \begin{tabular}{l|c|c|c|c|c}
%    \Xhline{1.0pt}
%      \multicolumn{2}{c|}{Dataset name} & \makecell{Publish \\ time} &  \makecell[c]{\# of photos\\ (video clips)} & Key features & Source \\
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{HOTorNOT~\cite{gray:eccv2010}}} & 2010 & 2,056 & \makecell[l]{Female frontal faces aged 18-40; annotated with ratings\\ collected from 30 labelers} & \makecell[l]{Hotornot.com}\\
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{Multi-Modality (face, dressing,\\ and voice) Beauty (M$^2$B)~\cite{nguyen:mm2012}}} & 2012 & \makecell[c]{1,240\\(280)} & \makecell[l]{Annotated with attractiveness scores, attribute categories,\\ and ethnic groups (Western or Eastern)} & \makecell[l]{YouTube.com}\\
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{Chen~\emph{et al.}~\cite{chen:icme2013}}} & 2013 & 2,648 & \makecell[l]{Annotated with fashionable or non-fashionable labels} & \makecell[l]{N/A}\\
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{Fashion144k\tablefootnote{\url{https://esslab.jp/~ess/en/data/fashion144k_stylenet/}}~\cite{simoserra:cvpr2015}}} & 2015 & 144,169 & \makecell[l]{Annotated with user-provided description, tags, number of\\ \textit{likes}, geographic location; each photo generally shows a\\ different angle of the user or zooms in on different garments} & \makecell[l]{Chictopia.com}\\
%    \hline 
%        \multicolumn{2}{c|}{\makecell[l]{Fashion products ~\cite{wang:icip2015}}} & 2015 & 500 & \makecell[l]{Annotated with the attractiveness score} & \makecell[l]{Photo sharing sites}\\
%    \hline
%        \multirow{6}{*}{\makecell[l]{Jia~\emph{et al.}\\\cite{jia:aaai2016}}} & \makecell[l]{D1: Labeled\\ Dataset} & \multirow{6}{*}{2016} & 5,500 & \makecell[l]{Annotated with 11 categories of upper-body menswear and\\ the coordinate values in the imagescale space} & \makecell[l]{Amazon.com}\\
%    \cline{2-2}\cline{4-6}
%         & \makecell[l]{D2: Unlabeled\\ Dataset} &  & 130,316 & \makecell[l]{Annotated with 11 categories of upper-body menswear} & \makecell[l]{JD.com}\\
%    \cline{2-2}\cline{4-6}
%        & \makecell[l]{D3: Demonstra-\\tion Dataset} &  & 77,160 & \makecell[l]{Consists of 76,360 menswear images from 277 brands cov-\\ering the Spring menswear and Fall menswear and 800 mens-\\wear images appearing in 2016 New York fashion week} & \makecell[l]{Style.com,\\ Thefashionisto.com}\\
%    \hline
%       \multirow{4}{*}{\makecell[l]{Chen and\\ Zhang\cite{chen:neurocomp2016}}} & \makecell[l]{Celebrity face\\ images} & \multirow{2}{*}{2016} & 390 & \multirow{4}{*}{\makecell[l]{Annotated with attractiveness score; confined to be female,\\ frontal with near neutral expressions}} & \makecell[l]{Websites}\\
%    \cline{2-2}\cline{4-4}\cline{6-6}
%        & \makecell[l]{Common face\\ images} & & 390 &  & \makecell[l]{Faceresearch.org, Flickr,\\ XM2VTS database~\cite{messer:avbpa1999},\\ Shanghai database~\cite{zhang:patternrecog2011}}\\
%    \hline
%        \multirow{2}{*}{\makecell[l]{Clothing\\ dataset\\\cite{chen:www2017}}} & \makecell[l]{Online Clothing\\ Shopping Dataset} & \multirow{2}{*}{2017} & 50,000 & \makecell[l]{Clothing products sold on Taobao from June 2014 to June\\ 2015; the associated images and user transaction data} & \makecell[l]{Taobao.com}\\
%    \cline{2-2}\cline{4-6}
%        & \makecell[l]{New York Fashion\\ Show} &  & 7,914 & \makecell[l]{Annotated with fine-grained clothing attributes} & \makecell[l]{Vogue.com}\\
%    \Xhline{1.0pt}
%    \end{tabular}
%    \label{tab:modeling_fashionbeauty_datasets}
%    \begin{tablenotes}
%      \scriptsize
%      \item N/A: there is no reported information to cite.
%    \end{tablenotes}
%\end{table*}

%\subsubsection{Performance evaluations}

%The qualitative analysis of this task uses subjective judgment, while the quantitative analysis is formulated as a classification or regression problem. The most widely used  measures to quantitatively evaluate the model performances are the classification accuracy~\cite{chen:icme2013, simoserra:cvpr2015, rothe:cvpr2016}, Mean Absolute Error (MAE)~\cite{nguyen:mm2012, jia:aaai2016, chen:neurocomp2016}, and Pearson's correlation~\cite{gray:eccv2010, rothe:cvpr2016, xu:iccasp2017}. Besides, some studies also reported their performances in terms of precision~\cite{chen:icme2013, simoserra:cvpr2015}, recall~\cite{chen:icme2013, simoserra:cvpr2015}, F1 measure~\cite{chen:icme2013}, Mean Squared Error (MSE)~\cite{jia:aaai2016}, intersection over union (IOU)~\cite{simoserra:cvpr2015}, and L1 norm~\cite{simoserra:cvpr2015}. Unfortunately, we are not able to compare the performance of each approach discussed in this section due to the unavailability of a standardized evaluation protocol.

%The MAE is defined as the average of the absolute errors between the predicted attractiveness score and the ground 
%Since the classification metrics such as accuracy, precision, recall, and intersection over union (IOU) do not capture the relationship between the different fashionability levels, we also report the L1 norm between the ground truth and the predicted label.
%the average accuracy, which is the percentage of correctly predicted ratings of the testing set, and the Pearson’s correlation.
%The Pearson Correlation is used to evaluate the performance between the ground-truth and the predicted result.


\subsection{Sociological Understanding}

\begin{comment}
In our society and century, clothing is not anymore used only as a means for body protection.
This work presents some research questions that are related to the investigation of the social signals associated to clothing.

Some research works investigated fashion within the social sciences, yang mana fashion styles correlate with personality traits, influencing the impression and behaviour of others towards a person .
clothing affects behavioral responses in the form of impression formation or person self-perception 
st systematic study on which social signals are conveyed by clothing, proposing a framework within the scope of com- puter vision to measure the clothing effect on the impression that we have on ourselves and that we trigger in the others. 
\end{comment}


%\textbf{Clothing Style and Identity.} Clothing is a visual linguistic that every piece of item conveys about the wearer to the viewer. Accordingly, analysing the clothing that people wear gives valuable information in the wearer's identity and personality.
%focuses on exploring the inherent relationship between wearer’s personality type and expressive wearing

%Aghaei~\emph{et al.}~\cite{aghaei:fg2017} presented some research questions to investigate the relationship between clothing styles and social signals. The investigation had two phases: investigation of the basic clothing behavioral cues that could be associated to an individual social signal, and investigation of the types of behaviors that might result from a social interaction taking into account the clothing styles worn by the interacting people. Jaha and Nixon~\cite{jaha:tifs2016} exploited low level image features to derive a biometric signature of soft clothing attributes for an individual. The approach enables subject identification and retrieval by using either an image or a verbal description as a query. a set of 21 soft clothing attributes is proposed for this purpose, including: (1) Head clothing; (2) Head coverage; (3) Face covered; (4) Hat; (5) Upper body clothing; (6) Neckline shape; (7) Neckline size; (8) Sleeve length; (9) Lower body clothing; (10) Shape of lower clothing; (11) Leg length of lower clothing; (12) Belt presence; (13) Shoes category; (14) Heel level; (15) Attached object category; (16) Size of bag; (17) Gun; (18) Object in hand; (19) Gloves; (20) Style category; and (21) Tattoos. %Fig.\ref{fig:sociological_understanding_pipelines} illustrates the overview of the proposed soft clothing biometrics framework in~\cite{jaha:tifs2016}. 

%The correlation between personality type and their wearing was explored in~\cite{wei:mtap2017}. To characterize different style of clothing, Wei~\emph{et al.} first segmented clothing region, verified the significance level of extracted features correlated with personality types through Binary Logistic regression, and then adopted SVM classifier to predict a person's personality.

%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=1\linewidth]{img/sociological_understanding_jahaTIFS2016.png}
%  \caption{The pipeline of soft clothing biometrics framework proposed by Jaha and Nixon~\cite{jaha:tifs2016}.}
%  \label{fig:sociological_understanding_pipelines}
%\end{figure}







%In particular, these models were evaluated in terms of .

%related to CY's recommendation
\textbf{Interaction styles.} Past research~\cite{vaccaro:chi2018} also explored personalized fashion interactions. Specifically, Vaccaro~\emph{et al.}~\cite{vaccaro:chi2018} conducted two independent studies: \textit{in-person} interaction by interviewing five personal stylists that offer in-person wardrobe and image consultations, and \textit{online} stylist interactions by developing a Facebook Messenger bot, namely PSBot, that connects users to one-on-one sessions with a stylist. 




%\cite{yamaguchi:mm2014} - The performance is measured in terms of accuracy
%\cite{park:cscw2016} - AUROC (Area Under the Receiver Operating Characteristic curve), and accuracy scores
%\cite{ha:icwsm2017} -- t-value


==> ACMCSUR – Fashion/src/fffashion_analysis.tex <==
\section{Fashion Analysis}
\label{sec:fffashion_analysis}

Fashion is not only about what people are wearing but also reveals personality traits and other social cues. With immense potential in the fashion industry, precision marketing, sociological analysis, \emph{etc.}, intelligent fashion analysis on what style people choose to wear has thus gained increasing attention in recent years. In this section, we mainly focus on three fields of fashion analysis: attribute recognition, style learning, and popularity prediction. For each field, state-of-the-art methods, the benchmark datasets, and the performance comparison are summarised.

\subsection{Attribute Recognition}
\label{subsec:attribute_recognition}

Clothing attribute recognition is a multi-label classification problem that aims at determining which elements of clothing are associated with attributes among a set of $n$ attributes. As illustrated in Fig.~\ref{fig:_retrieval_attribute_example}(b), a set of attributes is a mid-level representation generated to describe the visual appearance of a clothing item. 
%The representation necessary to support attribute recognition is also helpful for encoding the location of fashion landmarks, such as in~\cite{liu2016deepfashion, wang2018attentive}.%, and for recognizing the clothing style, which will be described later in this section.

%describing the appearances of clothes via semantic attributes

%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=0.8\linewidth]{img/attribute_prediction_clothingAttributes.jpg}
%  \caption{An example for clothing attributes recognition.}
%  \label{fig:attribute_example}
%\end{figure}

\subsubsection{State-of-the-art methods}

Chen \emph{et al.}~\cite{chen2012describing} learned a list of attributes for clothing on the human upper body. They extracted low-level features based on human pose estimation and then combined them for learning attribute classifiers. Mutual dependencies between the attributes capturing the rules of style (\textit{e.g.}, neckties are rarely worn with T-shirts) were explored by a Conditional Random Field (CRF) to make attribute predictions. A CRF-based model was also presented in~\cite{yamaguchi:iccv2015}. The model considered the location-specific appearance with respect to a human body and the compatibility of clothing items and attributes, which was trained using a max-margin learning framework.
%Kovashka and Grauman~\cite{kovashka:ijcv2015_agt} proposed to address the gap between language and visual perception by discovering the shades of attribute meaning. An attribute shade is a visual interpretation of an attribute name shared by some group of annotators. For example, given an attribute ``open'' of shoes, an annotator can interpret it as peep-toed (open at toe), slip-on (open at heel), or sandal-like (open at toe and heel). They used crowdsourced image labels to capture the latent interpretations of an attribute, then learned visual classifiers that can generalize to new images.

Motivated by the large discrepancy between images captured in constrained and unconstrained environments, Chen \emph{et al.}~\cite{chen2015deep} studied a cross-domain attribute mining. They mined the data from \textit{clean} clothing images obtained from online shopping stores and then adapted it to unconstrained environments by using a deep domain adaptation approach. Lu~\emph{et al.}~\cite{lu:neurocomp2016} further presented a study on part-based clothing attribute recognition in a search and mining framework. The method consists of three main steps: (1) Similar visual search with the assistance of pose estimation and part-based feature alignment; (2) Part-based salient tag extraction that estimates the relationship between tags and images by the analysis of intra-cluster and inter-cluster of clothing essential parts; and (3) Tag refinement by mining visual neighbors of a query image. In the meantime, Li~\emph{et al.} \cite{li:eccv2016} learned to score the human body and attribute-specific parts jointly in a deep Convolutional Neural Network, and further improved the results by learning collaborative part modeling among humans and global scene re-scoring through deep hierarchical contexts. %Another work~\cite{lu2017fully} designed a deep learning based model as a dynamic branching procedure by considering task relatedness at each layer of the network. %\textcolor{red}{The idea behind this is that the space of possible multi-task deep architectures is combinatorially large, and quite often the designed network architectures are biased by the designer's perception of the relationship among different tasks.}

Different from the above methods that conducted attribute recognition only based on annotated attribute labels,~\cite{vittayakorn2016automatic, corbiere2017leveraging, han2017automatic} proposed to identify attribute vocabulary using weakly labeled image-text data from shopping sites. They used the neural activations in the deep network that generated attribute activation maps through training a joint visual-semantic embedding space to learn the characteristics of each attribute. In particular, Vittayakorn \emph{et al.}~\cite{vittayakorn2016automatic} exploited the relationship between attributes and the divergence of neural activations in the deep network. Corbiere \emph{et al.}~\cite{corbiere2017leveraging} trained two different and independent deep models to perform attribute recognition. Han~\emph{et al.}~\cite{han2017automatic} derived spatial-semantic representations for each attribute by augmenting semantic word vectors for attributes with their spatial representation. 
%Compared to the method in~\cite{vittayakorn2016automatic}, \cite{corbiere2017leveraging} and \cite{han2017automatic} do not involve training a single model for each individual attribute.

%In addition to the above studies, 
Besides, there are research works exploring attributes for recognizing the type of clothing items. Hidayati~\emph{et al.}~\cite{hidayati:mm2012} introduced clothing genre classification by exploiting the discriminative attributes of style elements, with an initial focus on the upperwear clothes. The work in~\cite{hidayati:tcyb2018} later extended \cite{hidayati:mm2012} to recognize the lowerwear clothes. Yu and Grauman~\cite{yu:cvpr2014} proposed a local learning approach for fine-grained visual comparison to predict which image is more related to the given attribute. Jia~\emph{et al.}~\cite{jia:aaai2016} introduced a notion of using the two-dimensional continuous image-scale space as an intermediate layer and formed a three-level framework, \textit{i.e.}, visual features of clothing images, image-scale space based on the aesthetic theory, and aesthetic words space consisting of words like ``formal'' and ``casual''. A Stacked Denoising Autoencoder Guided by Correlative Labels was proposed to map the visual features to the image-scale space. Ferreira~\emph{et al.}~\cite{ferreira2019iccv} designed a visual semantic attention model with pose guided attention for multi-label fashion classification.
%In~\cite{nogueira:mtap2016}, Nogueira~\emph{et al.} proposed two approaches that combine visual and textual features from fashion-related social media data for clothing attribute prediction: (1) Multi-modal and Multi-label Clothing Annotation (MMCA), which is a pointwise approach that uses a single image as the instance, and (2) Multi-label, Multi-modal and Multi-instance Clothing Annotation (M3CA), which is a pairwise approach that employs a pair of images as the instances. Both the MMCA and M3CA methods use association rules that exploit usual similarities of social networks and build classifiers on a demand-driven basis using Lazy Association Classifiers (LAC)~\cite{veloso:icdm2006}. A set of predicted labels for each classifier is generated using an entropy-minimization multi-instance approach. 
Besides the clothing attribute recognition works, micro expression recognition is also an interesting task~\cite{ME2020mipr, ME2020acmmm}.



\subsubsection{Benchmark datasets}

There have been several clothing attribute datasets collected, as the older datasets are not capable of meeting the needs of the research goals. In particular, more recent datasets have a more practical focus. We summarize the clothing attribute benchmark datasets in Table~\ref{tab:attribute_recognition_datasets} and provide the links to download if they are available. 
%Note that some of these datasets, \emph{e.g.}, \cite{chen2015deep} and \cite{vittayakorn2016automatic}, are composed of several sub-datasets. 
%Compared to~\cite{chen2012describing}, their dataset has a much larger set of garments, including attribute sub-categories and a massive volume of training images per class.

\begin{table*}[t!]
%\footnotesize
\notsotiny
    \centering
        \caption{Summary of the benchmark datasets for clothing attribute recognition task.}
        \vspace{-3mm}
    \begin{tabular}{l|c|c|c|c|c|l|c}
    \Xhline{1.0pt}
        \multicolumn{2}{c|}{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ photos} & \makecell{\# of\\categories} & \makecell{\# of\\ attributes} & \makecell[c]{Key features} & Sources \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://purl.stanford.edu/tb980qz1002}{Clothing Attributes}%\tablefootnote{\url{https://purl.stanford.edu/tb980qz1002}}
        ~\cite{chen2012describing}}} & 2012 & 1,856 & 7 & 26 & \makecell[l]{Annotated with 23 binary-class attri-\\butes and 3 multi-class attributes} & \makecell[l]{Thesartorialist.com,\\Flickr.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Hidayati~\emph{et al.}~\cite{hidayati:mm2012}}} & 2012 & 1,077 & 8 & 5 & \makecell[l]{Annotated with clothing categories} & \makecell[l]{Online shopping sites}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{http://vision.cs.utexas.edu/projects/finegrained/}{UT-Zap50K shoe}%\tablefootnote{\url{http://vision.cs.utexas.edu/projects/finegrained/}}
        ~\cite{yu:cvpr2014}}} & 2014 & 50,025  & N/A & 4 & \makecell[l]{Shoe images annotated with associated\\ metadata (shoe type, materials, gender,\\ manufacturer, \emph{etc}.)} & \makecell[l]{Zappos.com}\\ 
    \hline
        \multirow{4}{*}{\makecell[l]{Chen~\emph{et al.}\\\cite{chen2015deep}}} & \makecell[l]{Online-data} & \multirow{4}{*}{2015} & 341,021 & 15 & 67 & \makecell[l]{Each attribute has 1000+ images} &
        \makecell[l]{Online shopping sites}\\ 
    \cline{2-2}\cline{4-8}
        & \makecell[l]{Street-data-a} &  & 685 & N/A & N/A & \multirow{3}{*}{\makecell[l]{Annotated with fine-grained attributes}} & \makecell[l]{Fashionista~\cite{KYamaguchi2012CVPR}}\\
    \cline{2-2}\cline{4-6}\cline{8-8}
        & \makecell[l]{Street-data-b} &  & 8,000 & N/A & N/A &  & \makecell[l]{Parsing~\cite{dong:cvpr2014}}\\ 
    \cline{2-2}\cline{4-6}\cline{8-8}
        & \makecell[l]{Street-data-c} &  & 4,200 & N/A & N/A &  & \makecell[l]{Surveillance videos}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Lu~\emph{et al.}~\cite{lu:neurocomp2016}}} & 2016 & $\sim$1,1 M & N/A & N/A & \makecell[l]{Annotated with the associated tags} & \makecell[l]{Taobao.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{http://mmlab.ie.cuhk.edu.hk/projects/WIDERAttribute}{WIDER Attribute}%\tablefootnote{\url{http://mmlab.ie.cuhk.edu.hk/projects/WIDERAttribute}}
        ~\cite{li:eccv2016}}} & 2016 & 13,789 & N/A & N/A & \makecell[l]{Annotated with 14 human attribute la-\\bels and 30 event class labels} & \makecell[l]{The 50574 WIDER\\ images~\cite{xiong:cvpr2015}}\\ 
    \hline
        \multirow{2}{*}{\makecell[l]{Vittayakorn\\\emph{et al.}~\cite{vittayakorn2016automatic}}} & \makecell[l]{Etsy} & \multirow{2}{*}{2016} &  173,175 & N/A & 250 & \makecell[l]{Annotated with title and description of\\ the product} & \makecell[l]{Etsy.com}\\  
    \cline{2-2}\cline{4-8}
        & \makecell[l]{Wear} &  &  212,129 & N/A & \makecell{250} & \makecell[l]{Annotated with the associated tags} & \makecell[l]{Wear.jp}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{http://mmlab.ie.cuhk.edu.hk/projects/DeepFashion/AttributePrediction.html}{DeepFashion-C}%\tablefootnote{\url{http://mmlab.ie.cuhk.edu.hk/projects/DeepFashion/AttributePrediction.html}}
        ~\cite{liu2016deepfashion}}} & 2016 & 289,222 & 50 & 1,000 & \makecell[l]{Annotated with clothing bounding box,\\ type, category, and attributes} & \makecell[l]{Online shopping sites,\\ Google Images}\\  
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{Nogueira~\emph{et al.}~\cite{nogueira:mtap2016}}} & 2016 & 3,885 & 31 & N/A & \makecell[l]{Annotated with tags/comments} & \makecell[l]{Chictopia.com,\\ Pose.com}\\  
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://github.com/xthan/fashion-200k}{Fashion200K}%\tablefootnote \url{https://github.com/xthan/fashion-200k}}
        ~\cite{han2017automatic}}} &  2017 & 209,544 & 5 & 4,404 & \makecell[l]{Annotated with product descriptions} & \makecell[l]{Lyst.com}\\ 
     \hline
        \multicolumn{2}{c|}{\makecell[l]{Hidayati~\emph{et al.}~\cite{hidayati:tcyb2018}}} & 2018 & 3,250 & 16 & 12 & \makecell[l]{Annotated with clothing categories} & \makecell[l]{Online shopping sites}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{CatalogFashion-10x~\cite{Heilbron2019ICCV}}} & 2019 & 1M & 43 & N/A & \makecell[l]{The categories are identical to the\\ DeepFashion dataset~\cite{liu2016deepfashion}} & \makecell[l]{Amazon.com}\\ 
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:attribute_recognition_datasets}
    \begin{tablenotes}
      \scriptsize
      \item N/A: there is no reported information to cite
    \end{tablenotes}
\end{table*}

\subsubsection{Performance evaluations}

\begin{table*}[t!]
\notsotiny
\center
\caption{Performance comparisons of attribute recognition methods in terms of top-\textit{k} classification accuracy.}
\vspace{-3mm}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
  \Xhline{1.0pt}
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Category} & \multicolumn{2}{c|}{Texture} & \multicolumn{2}{c|}{Fabric} & \multicolumn{2}{c|}{Shape} & \multicolumn{2}{c|}{Part} & \multicolumn{2}{c|}{Style} & \multicolumn{2}{c}{All} \\
   & top-3 & top-5 & top-3 & top-5 & top-3 & top-5 & top-3 & top-5 & top-3 & top-5 & top-3 & top-5 & top-3 & top-5 \\
  \hline
  \makecell[l]{Chen \emph{et al.}~\cite{chen2012describing}} & 43.73 & 66.26 & 24.21 & 32.65 & 25.38 & 36.06 & 23.39 & 31.26 & 26.31 & 33.24 & 49.85 & 58.68 & 27.46 & 35.37 \\
  \hline
  \makecell[l]{DARN~\cite{huang2015cross}} & 59.48 & 79.58 & 36.15 & 48.15 & 36.64 & 48.52 & 35.89 & 46.93 & 39.17 & 50.14 & 66.11 & 71.36 & 42.35 & 51.95 \\
  \hline
  \makecell[l]{FashionNet~\cite{liu2016deepfashion}} &  82.58 & 90.17 & 37.46 & 49.52 & 39.30 & \textbf{49.84} & 39.47 & 48.59 & \textbf{44.13} & 54.02 & 66.43 & 73.16 & 45.52 & 54.61 \\
%  \hline
%  Lu \emph{et al.}~\cite{lu2017fully} & 86.72 & 92.51 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
  \hline
  \makecell[l]{Corbiere \emph{et al.}~\cite{corbiere2017leveraging}} & 86.30 & 92.80 & \textbf{53.60} & 63.20 & 39.10 & 48.80 & 50.10 & 59.50 & 38.80 & 48.90 & 30.50 & 38.30 & 23.10 & 30.40 \\
  \hline
  \makecell[l]{AttentiveNet~\cite{wang2018attentive}} & \textbf{90.99} & \textbf{95.78} & 50.31 & \textbf{65.48} & \textbf{40.31} & 48.23 & \textbf{53.32} & \textbf{61.05} & 40.65 & \textbf{56.32} & \textbf{68.70} & \textbf{74.25} & \textbf{51.53} & \textbf{60.95} \\
  \Xhline{1.0pt}
\end{tabular}
    \begin{tablenotes}
      \scriptsize
      \item The best result is marked in bold. %``--'' represents detailed results are not available.
\end{tablenotes}
\label{table:attribute_recognition_result}
\end{table*}

Metrics that are used to evaluate the clothing attribute recognition models include the top-\textit{k} accuracy, mean average precision (MAP), and Geometric Mean (G-Mean). The top-\textit{k} accuracy and MAP have been described in Sec.~\ref{sec:item_retrieval_PE}, %The top-\textit{k} accuracy is the ratio of correct predictions among the top-\textit{k} predicted attributes, mAP is the mean of the average precision scores over all queries
while G-mean measures the balance between classification performances on both the majority and minority classes. Most authors opt for a measure based on top-\textit{k} accuracy. We present the evaluation for general attribute recognition on the DeepFashion-C Dataset with different methods in Table~\ref{table:attribute_recognition_result}. %(the best result is marked in bold).
The evaluation protocol is released in~\cite{liu2016deepfashion}. %From this table, we found that more recent methods have higher predictive performance than the older methods, with the newest attentiveNet~\cite{wang2018attentive} obtaining the highest average score.

\subsection{Style Learning}

A variety of fashion styles is composed of different fashion designs. Inevitably, these design elements and their interrelationships serve as the powerful source-identifiers for understanding fashion styles. The key issue in this field is thus how to analyze discriminative features for different styles and also learn what style makes a trend.

%\textbf{Spatial Analysis} Fashion spatial analysis refers to the discovery of patterns of fashion styles related to spatial or geographical aspects. To date, there are only a few studies that explored this area. 

%\textbf{Temporal Analysis} In this subsection, we discuss existing fashion research on the topic of temporal analysis, aiming to extract and characterize the trends, patterns, and variations within a fashion style over time using time series data. 


\subsubsection{State-of-the-art methods}

An early attempt in fashion style recognition was presented by Kiapour~\emph{et al.}~\cite{MHKiapour2014}. They evaluated the concatenation of hand-crafted descriptors as style representation. Five different style categories are explored, including hipster, bohemian, pinup, preppy, and goth.

In the following studies~\cite{ESimo-Serra2016CVPR,SJiang2016AAAI, ma:aaai2017, vaccaro:uist2016, hsiao:iccv2017}, deep learning models were employed to represent fashion styles. In particular, Simo-Serra and Ishikawa~\cite{ESimo-Serra2016CVPR} developed a joint ranking and classification framework based on the Siamese network. The proposed framework was able to achieve outstanding performance with features being the size of a SIFT descriptor. To further enhance feature learning, Jiang \emph{et al.}~\cite{SJiang2016AAAI} used a consensus style centralizing auto-encoder (CSCAE) to centralize each feature of certain style progressively. Ma~\emph{et al.} introduced Bimodal Correlative Deep Autoencoder (BCDA)~\cite{ma:aaai2017}, a fashion-oriented multimodal deep learning based model adopted from Bimodal Deep Autoencoder~\cite{ngiam:icml2011}, to capture the correlation between visual features and fashion styles. The BCDA learned the fundamental rules of tops and bottoms as two modals of clothing collocations. The shared representation produced by BCDA was then used as input of the regression model to predict the coordinate values in the fashion semantic space that describes styles quantitatively. Vaccaro \emph{et al.} \cite{vaccaro:uist2016} presented a data-driven fashion model that learned the correspondences between high-level style descriptions (\textit{e.g.}, ``valentines day'' %, ``vintage'') 
and low-level design elements (\textit{e.g.}, ``red cardigan'' %, ``lightweight shirt'') 
by training polylingual topic modeling. This model adapted a natural language processing technique to learn latent fashion concepts jointly over the style and element vocabularies. Different from previous studies that sought coarse style classification, Hsiao and Grauman~\cite{hsiao:iccv2017} treated styles as discoverable latent factors by exploring style-coherent representation. An unsupervised approach based on polylingual topic models was proposed to learn the composition of clothing elements that are stylistically similar. Further, interesting work for learning the user-centric fashion information based on occasions, clothing categories, and attributes was introduced by Ma \emph{et al.}~\cite{ma2019acmmm}. Their main goal is to learn the information about ``what to wear for a specific occasion?'' from social media, \emph{e.g.}, Instagram. They developed a contextualized fashion concept learning model to capture the dependencies among occasions, clothing categories, and attributes.

\textbf{Fashion Trends Analysis}. A research pioneer in automatic fashion trend analysis was presented by Hidayati~\emph{et al.}~\cite{hidayati:mm2014}. They investigated fashion trends at ten different seasons of New York Fashion Week %(NYFW)
by analyzing the coherence (to occur frequently) and uniqueness (to be sufficiently different from other fashion shows) of visual style elements%through unsupervised and supervised learning
. Following~\cite{hidayati:mm2014}, Chen~\emph{et al.}~\cite{chen:mm2015} utilized a learning-based clothing attributes approach to analyze the influence of the New York Fashion Show on people's daily life. Later, Gu~\emph{et al.}~\cite{gu:mm2017} presented QuadNet for analyzing fashion trends from street photos. The QuadNet was a classification and feature embedding learning network that consists of four identical CNNs, where the shared CNN was jointly optimized with a multi-task classification loss and a neighbor-constrained quadruplet loss. The multi-task classification loss aimed to learn the discriminative feature representation, while the neighbor-constrained quadruplet loss aimed to enhance the similarity constraint. A study on modeling the temporal dynamics of the popularity of fashion styles was presented in~\cite{he:www2016}. It captured fashion dynamics by formulating the visual appearance of items extracted from a deep convolutional neural network as a function of time.

Further, for statistics-driven fashion trend analysis,~\cite{chen:www2017} analyzed the best-selling clothing attributes corresponding to specific season via the online shopping websites statistics, e.g., (1) winter: gray, black, and sweater; (2) spring: white, red, and v-neckline. They designed a machine learning based method considering the fashion item sales information and the user transaction history for measuring the real impact of the item attributes to customers. Besides the fashion trend learning related to online shopping websites was considered, Ha~\emph{et al.}~\cite{ha:icwsm2017} used fashion posts from Instagram to analyze visual content of fashion images and correlated them with likes and comments from the audience. Moreover, Chang \emph{et al.} achieved an interesting work~\cite{YChang2017} on what people choose to wear in different cities. The proposed ``Fashion World Map'' framework exploited a collection of geo-tagged street fashion photos from an image-centered social media site, Lookbook.nu. They devised a metric based on deep neural networks to select the potential iconic outfits for each city and formulated the detection problem of iconic fashion items of a city as the prize-collecting Steiner tree (PCST) problem. A similar idea was proposed by Mall~\emph{et al.}~\cite{GeoStyle2019} in 2019; they established a framework\footnote{\url{https://github.com/kavitabala/geostyle}} for automatically analyzing the fashion trend worldwide in item attributes and style corresponding to the city and month. Specifically, they also analyzed how social events impact people wear, e.g., ``new year in Beijing in February 2014'' leads to red upper clothes.

%Chen and Luo~\cite{chen:www2017} further analyzed fashion content to investigate the marketing strategies of fashion brands by mining attractive and profitable clothing features. They first learned a classifier based on a deep learning architecture to automatically pruning noisy and unrelated images. After that, they adopted a learning-based clothing attributes approach to discover fine-grained clothing attributes as the representation of attractive and popular clothing style elements.

%Besides, 
Temporal estimation is an interesting task for general fashion trend analysis, the goal of which is to estimate when a style was made. Although visual analysis of fashion styles have been much investigated, this topic has not received much attention from the research community. %For temporal estimation of fashion trend, 
Vittayakorn~\emph{et al.}~\cite{vittayakorn:wacv2017} proposed an approach to the temporal estimation task using %a deep-learning based method. They utilized Convolutional Neural Network 
CNN features and fine-tuning new networks to predict the time period of styles directly. This study also provided estimation analyses of what the temporal estimation networks have learned. %To our best knowledge, to date, \cite{vittayakorn:wacv2017} is the only work devoted to the interests of the fashion temporal estimation.

%\textbf{spatial Analysis}
% CY think that brambila:www2017 is nothing about fashion
%In the meantime, Brambilla~\emph{et al.}~\cite{brambila:www2017} discussed how social content responds to live events which appear in the official calendar, in terms of spatial features of dispersion/concentration of social media signals related to each specific fashion show. They first built different clusters of fashion brands by characterizing several features that describe the spatial dispersion of posts following an event, and then correlated them to a specific class of social responses in the two dimensions.

%\begin{figure}[ht]
%  \centering
%  \includegraphics[width=1\linewidth]{img/spatial_analysis_ChangMM2017.png}
%  \caption{The pipeline of Fashion World Map framework in~\cite{YChang2017}.}
%  \label{fig:spatial_analysis_pipelines}
%\end{figure}

%\textbf{Temporal Analysis}
%Existing works relevant to the temporal analysis of fashion styles can be categorized into three main groups, \textit{i.e.}, fashion trends analysis, styles forecasting, and temporal estimation.



%\textbf{Fashion Forecasting}. 


%\textbf{Temporal Estimation.} The goal of temporal estimation is to estimate when a style was made. Although visual analysis of fashion styles have been much investigated, this topic has not received much attention from the research community. 



%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=1\linewidth]{img/temporal_analysis_guMM2017.png}
%  \caption{The pipeline of fashion temporal analysis framework proposed by Gu~\emph{et al.}~\cite{gu:mm2017}.}
%  \label{fig:temporal_analysis_pipelines}
%\end{figure}

\subsubsection{Benchmark datasets}

Table~\ref{tab:style_analysis_datasets} compares the benchmark datasets used in the literature. Hipster Wars% dataset
~\cite{MHKiapour2014} is the most popular dataset for style learning. We note that, instead of using the same dataset for training and testing, the study in~\cite{ESimo-Serra2016CVPR} used Fashion144k dataset~\cite{simoserra:cvpr2015} to train the model and evaluated it on Hipster Wars% dataset
~\cite{MHKiapour2014}. Moreover, the datasets related to fashion trend analysis %~\cite{hidayati:mm2014, chen:mm2015, he:www2016, gu:mm2017, YChang2017, vittayakorn:wacv2017, GeoStyle2019}
were mainly collected from online media platforms during a specific time interval. 



\begin{table*}[t!]
\notsotiny
    \centering
        \caption{Summary of the benchmark datasets for style learning task.}
        \vspace{-3mm}
    \begin{tabular}{l|c|c|c|l|c}
    \Xhline{1.0pt}
        \multicolumn{2}{c|}{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ photos} & \makecell[c]{Key features} & Sources \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{http://tamaraberg.com/hipsterwars/}{Hipster Wars}~\cite{MHKiapour2014}%\tablefootnote{\url{http://tamaraberg.com/hipsterwars/}}
        }} & 2014 & 1,893 & \makecell[l]{Annotated with Bohemian, Goth, Hipster, Pinup,\\ or Preppy style} & \makecell[l]{Google Image Search}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Hidayati~\emph{et al.}~\cite{hidayati:mm2014}}} & 2014 & 3,276 & \makecell[l]{Annotated with 10 seasons of New York Fashion Week\\ (Spring/Summer 2010 to Autumn/Winter 2014)} & \makecell[l]{FashionTV.com}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://esslab.jp/~ess/en/data/fashion144k_stylenet/}{Fashion144k}~\cite{simoserra:cvpr2015}%\tablefootnote{\url{https://esslab.jp/~ess/en/data/fashion144k_stylenet/}}
        }} & 2015 & 144,169 & \makecell[l]{Each post contains text in the form of descriptions and gar-\\ment tags. It also consists of ``likes'' for scaling popularity} & \makecell[l]{Chictopia.com}\\
    \hline
        \multirow{3}{*}{\makecell[l]{Chen~\emph{et al.}~\cite{chen:mm2015}}} & \makecell[l]{Street-chic} & \multirow{2}{*}{2015} & 1,046 &  \makecell[l]{Street-chic images in New York from April 2014 to July\\ 2014 and from April 2015 to July 2015} & \makecell[l]{Flickr.com,\\ Pinterest.com}\\
        \cline{2-2}\cline{4-6}
        & \makecell[l]{New York\\ Fashion Show} &  & 7,914 & \makecell[l]{2014 and 2015 summer/spring New York Fashion Show} & \makecell[l]{Vogue.com}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Online Shopping ~\cite{SJiang2016AAAI}}} & 2016 & 30,000 & \makecell[l]{The 12 classes definitions are based on the fashion maga-\\zine~\cite{classesBased}} & \makecell[l]{Nordstrom.com,\\ barneys.com}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Fashion Data ~\cite{vaccaro:uist2016}}} & 2016 & 590,234 & \makecell[l]{Annotated with a title, text description, and a list of items\\ the outfit comprises} & \makecell[l]{Polyvore.com}\\
    \hline
        \multirow{2}{*}{\makecell[l]{He and McAuley\\\emph{et al.}~\cite{he:www2016}}} & \makecell[l]{Women} & \multirow{2}{*}{2016} & 331,173 &  \multirow{2}{*}{\makecell[l]{Annotated with users' review histories, time span between\\ March 2003 and July 2014}} & \makecell[l]{Amazon.com}\\
        \cline{2-2}\cline{4-4}
        & \makecell[l]{Men} &  & 100,654  &  & \\
    \hline
        \multirow{2}{*}{\makecell[l]{Vittayakorn~\emph{et al.}\\\cite{vittayakorn:wacv2017}}} & \makecell[l]{Flickr Clothing} & \multirow{2}{*}{2017} & 58,350 & \makecell[l]{Annotated with decade label and user provided metadata} & \makecell[l]{Flickr.com}\\
    \cline{2-2}\cline{4-6}
        & \makecell[l]{Museum Dataset} & & 9,421 & \makecell[l]{Annotated with decade label} & \makecell[l]{museum}\\
%The Metropolitan Museum\\ of Art, Europeana Fashion        
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Street Fashion Style (SFS)~\cite{gu:mm2017}}} & 2017 & 293,105 & \makecell[l]{Annotated with user-provided tags, including geographical\\ and year information} & \makecell[l]{Chictopia.com}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Global Street Fashion\\(GSFashion)~\cite{YChang2017}}} & 2017 & 170,180 &  \makecell[l]{Annotated with (1) city name, (2) anonymized user ID,\\ (3) anonymized post ID, (4) posting date, (5) number of\\ likes of the post, and (6) user-provided metadata descri-\\bing the categories of fashion items along with the brand\\ names and the brand-defined product categories} & \makecell[l]{Lookbook.nu}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://pan.baidu.com/s/1boPm2OB}{Fashion Semantic Space (FSS)}%\tablefootnote{\url{https://pan.baidu.com/s/1boPm2OB}}
        ~\cite{ma:aaai2017}}} & 2017 & 32,133 & \makecell[l]{Full-body fashion show images; annotated with visual\\ features (\textit{e.g.}, collar shape, pants length, or color theme.)\\ and fashion styles (\textit{e.g.}, casual, chic, or elegant).} & \makecell[l]{Vogue.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{http://vision.cs.utexas.edu/projects/StyleEmbedding/}{Hsiao and Grauman}%\tablefootnote{\url{http://vision.cs.utexas.edu/projects/StyleEmbedding/}}
        ~\cite{hsiao:iccv2017}}} &  2017 & 18,878 & \makecell[l]{Annotated with associated attributes} & \makecell[l]{Google Images}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Ha~\emph{et al.}~\cite{ha:icwsm2017}}} &  2017 & 24,752 & \makecell[l]{It comprises description of images, associated  metadata,\\ and annotated and predicted visual content variables} & \makecell[l]{Instagram}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Geostyle~\cite{GeoStyle2019}}} & 2019 & 7.7M &\makecell[l]{This dataset includes categories of 44 major world cities\\ across 6 continents, person body and face detection, and\\ canonical cropping} & \makecell[l]{Street Style~\cite{StreetStyle2017},\\Flickr100M~\cite{vittayakorn:wacv2015}}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{FashionKE~\cite{ma2019acmmm}}} & 2019 & 80,629 &\makecell[l]{With the help of fashion experts, it contains 10 common\\ types of occasion concepts, e.g., dating, prom, or travel} & \makecell[l]{Instagram}\\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:style_analysis_datasets}
    \begin{tablenotes}
      \scriptsize
      \item M means million.%N/A: there is no reported information to cite.
    \end{tablenotes}
\end{table*}

%\textbf{spatial Analysis - benchmark datasets}

%We summarize the benchmark dataset used in fashion spatial analysis in Table~\ref{tab:spatial_analysis_datasets}. Both \cite{YChang2017} and \cite{brambila:www2017} exploited social media platforms, but different in data modality. 

%\begin{table*}[t!]%[htbp]
%\footnotesize
%    \centering
%        \caption{Summary of the benchmark datasets for fashion spatial analysis task.}
%        \vspace{-3mm}
%    \begin{tabular}{c|c|c|c|c}
%    \Xhline{1.0pt}
%      Dataset name & \makecell{Publish \\ time} & \makecell{\# of \\ photos} &  Key features & Source \\
%    \hline
%        \makecell[l]{Global Street Fashion\\(GSFashion)~\cite{YChang2017}} & 2017 & 170,180 & \makecell[l]{Annotated with (1) city name, (2) anonymized user ID, (3) anonymized post ID, \\(4) posting date, (5) number of likes of the post, and (6) user-provided metadata\\ describing the categories of fashion items along with the brand names\\ and the brand-defined product categories} & \makecell[l]{Lookbook.nu}\\
    %\hline
    %    \makecell[l]{Brambila~\emph{et al.}~\cite{brambila:www2017}} & \makecell{2017} & -- & \makecell[l]{106K tweets from Twitter and 556K Instagram posts annotated with a set of 21\\ hashtags and keywords provided by domain experts in the fashion sector} & \makecell[l]{Twitter, Instagram} \\
%    \Xhline{1.0pt}
%    \end{tabular}
%    \label{tab:spatial_analysis_datasets}
%\end{table*}

%\textbf{temporal Analysis - benchmark datasets}

%Since fashion temporal analysis is a highly diverse topic, there are several datasets for different fashion temporal analysis tasks. These datasets were mainly collected from online media platforms during a specific time interval. We summarize a collection of benchmark datasets used for fashion temporal analysis in Table~\ref{tab:temporal_analysis_datasets}. 

%\begin{table*}[t!]%[htbp]
%\footnotesize
%    \centering
%        \caption{Summary of the benchmark datasets for fashion temporal analysis task.}
%        \vspace{-3mm}
%    \begin{tabular}{l|c|c|c|c|l}
%    \Xhline{1.0pt}
%      \multicolumn{2}{c|}{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ photos} &  Key features & \makecell[c]{Source} \\
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{Hidayati~\emph{et al.}~\cite{hidayati:mm2014}}} & 2014 & 3,276 & \makecell[l]{Annotated with 10 seasons of New York Fashion Week\\ (Spring/Summer 2010 to Autumn/Winter 2014)} & \makecell[l]{FashionTV.com}\\
    %\hline
    %    \multicolumn{2}{c|}{\makecell[l]{Ren~\emph{et al.}~\cite{ren:tcybsystems2015}}} & 2015 & 216 & \makecell[l]{Annotated with 6 fashion items with 7 kinds of color,\\ price, and sales data} & \makecell[l]{Fashion boutique}\\
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{McAuley~\emph{et al.}~\cite{mcauley:sigir2015}}} & 2015 & 78,024 & \makecell[l]{Annotated with three garment categories, a short textual\\ description, a set of tags, and the dates each time the item\\ was purchased} & \makecell[l]{Amazon.com}\\
%    \hline
%        \multirow{2}{*}{\makecell[l]{Chen~\emph{et al.}~\cite{chen:mm2015}}} & \makecell[l]{Street-chic} & \multirow{2}{*}{2015} & 1,046 & \makecell[l]{Street-chic images in New York from April 2014 to July\\ 2014 and from April 2015 to July 2015} & \makecell[l]{Flickr.com,\\ Pinterest.com}\\
%        \cline{2-2}\cline{4-6}
%        & \makecell[l]{New York\\ Fashion Show} &  & 7,914 & \makecell[l]{2014 and 2015 summer/spring New York Fashion Show} & \makecell[l]{Vogue.com}\\
%    \hline
%        \multirow{2}{*}{\makecell[l]{He and McAuley\\\emph{et al.}~\cite{he:www2016}}} & \makecell[l]{Women} & \multirow{2}{*}{2016} & 331,173 & \multirow{2}{*}{\makecell[l]{Annotated with users' review histories, time span between\\ March 2003 and July 2014}} & \multirow{2}{*}{\makecell[l]{Amazon.com}}\\
%        \cline{2-2}\cline{4-4}
%        & \makecell[l]{Men} &  & 100,654 &  & \\
%    \hline
%        \multirow{3}{*}{\makecell[l]{Vittayakorn~\emph{et al.}\\\cite{vittayakorn:wacv2017}}} & \makecell[l]{Flickr Clothing} & \multirow{2}{*}{2017} & 58,350 & \makecell[l]{Annotated with decade label and user provided metadata} & \makecell[l]{Flickr.com}\\
%    \cline{2-2}\cline{4-6}
%        & \makecell[l]{Museum Dataset} & & 9,421 & \makecell[l]{Annotated with decade label} & \makecell[l]{The Metropolitan Museum\\ of Art, Europeana Fashion}\\
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{Street Fashion Style (SFS)~\cite{gu:mm2017}}} & 2017 & 293,105 & \makecell[l]{Annotated with user-provided tags, including geographical\\ and year information} & \makecell[l]{Chictopia.com}\\
%    \Xhline{1.0pt}
%    \end{tabular}
%    \label{tab:temporal_analysis_datasets}
%\end{table*}



\subsubsection{Performance evaluations}

The evaluation metrics used to measure the performance of existing fashion style learning models are precision, recall, and accuracy. %, and Normalized Discounted Cumulative Gain (NDCG). 
Essentially, precision measures the ratio of retrieved results that are relevant, recall measures the ratio of relevant results that are retrieved, while accuracy measures the ratio of correct recognition. %, while NDCG measures the ranking quality. 
%We present the performances of fashion style learning methods on Hipster Wars dataset in Table~\ref{table:style_recognition_result}. In this table, $p$ denotes the percentage of top ranked data according to their style level and $\phi$ denotes the style level.
%\textbf{Temporal Analysis - Performance Evaluations}
% Moreover, the studies in \cite{hidayati:mm2014, chen:mm2015, he:www2016, gu:mm2017} that focused on fashion trends analysis adopted the accuracy metric to measure the overall performance. In addition to accuracy, \cite{gu:mm2017} also quantified the performance of their method using per-class precision, per-class recall, overall precision, and overall recall. 
Although several approaches for fashion temporal analysis have been proposed, there is no extensive comparison between %those approaches have been undertaken. 
them. It is an open problem to determine which of the approaches perform better than others. 

%\begin{table*}[t!]
%\footnotesize
%\center
%\caption{Performance comparisons for style learning methods in terms of accuracy.}
%\vspace{-3mm}
%\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
%  \hline
%   \multirow{2}{*}{Method} & \multicolumn{5}{c|}{Hipster Wars Dataset~\cite{MHKiapour2014}} & \multicolumn{5}{c}{Online Shopping Dataset~\cite{SJiang2016AAAI}}\\
%  
%   & $p=0.1$ & $p=0.2$ & $p=0.3$ & $p=0.4$ & $p=0.5$ & $\phi=7$ & $\phi=6$ & $\phi=5$ & $\phi=4$ & $\phi=3$ \\
%  \hline
%  \makecell[l]{Kiapour~\emph{et al.}~\cite{MHKiapour2014}} & 77.73 & 62.86 & 53.34 & 37.74 & 34.61 & 60.92 & 58.52 & 54.57 & 48.63 & 42.40 \\
%  \hline
%  \makecell[l]{Yamaguchi~\emph{et al.}}~\cite{KYamaguchi2013} & 75.75 & 62.42 & 50.53 & 35.36 & 33.36 & 55.00 & 53.96 & 51.73 & 45.38 & 37.91 \\
%  \hline
%  \makecell[l]{Bossard~\emph{et al.}~\cite{bossard:ACCV2012}} & 76.36 & 62.43 & 52.68 & 34.64 & 33.42 & 54.58 & 59.43 & 52.47 & 41.39 & 35.42 \\
%  \hline
%  \makecell[l]{CSCAE~\cite{SJiang2016AAAI}} & \textbf{89.21} & \textbf{75.32} & \textbf{64.55} & \textbf{52.88} & \textbf{43.77} & \textbf{70.41} & \textbf{68.42} & \textbf{63.84} & \textbf{51.18} & \textbf{50.31} \\
%  \hline
%\end{tabular}
%\label{table:style_recognition_result}
%\end{table*}

%\textbf{Spatial Analysis - Performance Evaluations}


%The work in \cite{YChang2017} conducted a user study to evaluate the iconic fashion items of the corresponding city, then adopted the agreement ratio as an evaluation metric to asses the performance.



%\cite{vittayakorn:wacv2017} -- The mean absolute error 
%\cite{alhalah:iccv2017} - The mean absolute error, the mean absolute percentage error
%\cite{chen:mm2015} -- accuracy
%\cite{gu:mm2017} -- precision, recall, accuracy
%\cite{hidayati:mm2014} -- accuracy


%------------------------------------------------------------


\subsection{Popularity Prediction.}
Precise fashion trend prediction is not only essential for fashion brands to strive for the global marketing campaign but also crucial for individuals to choose what to wear corresponding to the specific occasion. Based on the fashion style learning via the existing data (e.g., fashion blogs), it can better predict fashion popularity and further forecast future trend, which profoundly affect the fashion industry about multi-trillion US dollars.

\subsubsection{State-of-the-art methods}

%Despite the active research in popularity prediction of online content on general photos with diverse categories~\cite{khosla:www2014, SMP2016aaai, SMP2017ijcai, hidayati:mm2017, massip:icmew2018, wen2018ijcai},
Despite the active research in popularity prediction of online content on general photos with diverse categories~\cite{SMP2016aaai, SMP2017ijcai, hidayati:mm2017, massip:icmew2018, wen2018ijcai}, the popularity prediction on online social network specialized in fashion and style is currently understudied. The work in~\cite{yamaguchi:mm2014} presented a vision-based approach to quantitatively evaluate the influence of visual, textual, and social factors on the popularity of outfit pictures. They found that the combination of social and content information yields a good predictory for popularity. In~\cite{park:cscw2016}, Park~\emph{et al.} applied a widely-used machine learning algorithm to uncover the ingredients of success of fashion models and predict their popularity within the fashion industry by using data from social media activity. Recently, Lo~\emph{et al.}~\cite{lo2019icip} proposed a deep temporal sequence learning framework to predict the fine-grained fashion popularity of an outfit look.

Discovering the visual attractiveness has been the pursuit of artists and philosophers for centuries. Nowadays, the computational model for this task has been actively explored in the multimedia research community, especially with the focus on clothing and facial features. Nguyen~\emph{et al.}~\cite{nguyen:mm2012} studied how different modalities (\textit{i.e.}, face, dress, and voice) individually and collectively affect the attractiveness of a person. A tri-layer learning framework, namely Dual-supervised Feature-Attribute-Task %(DFAT) 
network, was proposed to learn attribute models and attractiveness models simultaneously. Chen~\emph{et al.} \cite{chen:icme2013} focused on modeling fashionable dresses. The framework was based on two main components: basic visual pattern discovery using active clustering with humans in the loop, and latent structural SVM learning to differentiate fashionable and non-fashionable dresses. Next, Simo-Serra~\emph{et al.}~\cite{simoserra:cvpr2015} not only predicted the fashionability of a person's look on a photograph but also suggested what clothing or scenery the user should change to improve the look. For this purpose, they utilized a Conditional Random Field model to learn correlation among fashionability factors, such as the type of outfit and garments, the type of the user, and the scene type of the photograph.  

Meanwhile, the aesthetic quality assessment of online shopping photos is a relatively new area of study. A set of features related to photo aesthetic quality is introduced in~\cite{wang:icip2015}. To be more specific, in this work, Wang and Allebach investigated the relevance of each feature to aesthetic quality via the elastic net. They trained an SVM predictor with an optimal feature subset constructed by a wrapper feature selection strategy with the best-first search algorithm.

Other studies built computational attractiveness models to analyze facial beauty. A previous survey on this task was presented in \cite{liu:mtap2016}. Since some remarkable progress have been made on this subject, we extend \cite{liu:mtap2016} to cover recent advancements. %In~\cite{gray:eccv2010}, Gray~\emph{et al.} presented a hierarchical feed-forward approach to learn facial appearance and a regression model to predict the beauty scores. 
Chen and Zhang~\cite{chen:neurocomp2016} introduced a causal effect criterion to evaluate facial attractiveness models. It proposed two-way measurements, \textit{i.e.}, by imposing interventions according to the model and by examining the change of attractiveness. To alleviate the need for rating history for the query, which prior works could not cope when there are none or few, Rothe~\emph{et al.}~\cite{rothe:cvpr2016} proposed to regress visual query to a latent space derived through matrix factorization for the known subjects and ratings. Besides, they employed a visual regularized collaborative filtering approach to infer inter-person preferences for attractiveness prediction. A psychologically inspired deep convolutional neural network (PI-CNN), which is a hierarchical model that facilitates both the facial beauty representation learning and predictor training, was later proposed in ~\cite{xu:iccasp2017}. To optimize the performance of the PI-CNN facial beauty predictor, \cite{xu:iccasp2017} introduced a cascaded fine-tuning scheme that exploits appearance features of facial detail, lighting, and color. To further consider the facial shape, Gao~\emph{et al.}~\cite{gao2018icpr} designed a multi-task learning framework that took appearance and facial shape into account simultaneously and jointly learned facial representation, landmark location, and facial attractiveness score. They proved that learning with landmark localization is effective for facial attractiveness prediction. For building flexible filters to learn the mapping adaptive for different attributes within a deep modal, Lin~\emph{et al.}~\cite{lin2019ijcai} proposed an attribute-aware convolutional neural network (AaNet) whose filter parameters were controlled adaptively by facial attributes. They also considered the cases without attribute labels and presented a pseudo attribute-aware network (P-AaNet), which learned to utilize image context information for generating attribute-like knowledge. Moreover, Shi~\emph{et al.}~\cite{shi2019icassp} introduced a co-attention learning mechanism that employed facial parsing masks for learning accurate representation of facial composition to improve facial attractiveness prediction.

%Within the field of popularity prediction, 
There was a Social Media Prediction (SMP) challenge\footnote{\url{http://www.smp-challenge.com/}} held by Wu~\emph{et al.}~\cite{Wu2019SMPCA} in ACM Multimedia 2019 which aimed at the work focused on predicting future clicks of new social media posts before they were posted in social feeds. The participated teams need to build a new algorithm based on understanding and learning techniques and automatically predict popularity (formulated by clicks or visits) to achieve better performances. 

\textbf{Fashion Forecasting}.
%There are strong practical interests in fashion sales forecasting, either by utilizing traditional statistical models~\cite{lin:jti2010, ni:expertsyst2011, choi:tcyb2012},
There are strong practical interests in fashion sales forecasting, either by utilizing traditional statistical models~\cite{ni:expertsyst2011, choi:tcyb2012}, applying artificial intelligence models~\cite{banica:iffs2014}, or combining the advantages of statistics-based methods and artificial intelligence-based methods into hybrid models~\cite{kaya:iffs2014, ren:tcybsystems2015, chen:nca2017}. However, the problem of visual fashion forecasting, where the goal is to predict the future popularity of styles discovered from fashion images, has gained limited attention in the literature. In~\cite{alhalah:iccv2017}, Al-Halah~\emph{et al.} proposed to forecast the future visual style trends from fashion data in an unsupervised manner. The proposed approach consists of three main steps: (1) learning a representation of fashion images that captures clothing attributes using a supervised deep convolutional model; (2) discovering the set of fine-grained styles that are distributed across images using a non-negative matrix factorization framework; and (3) constructing styles' temporal trajectories  based on statistics of past consumer purchases for predicting the future trends.


%------------------------------------------------------------
\subsubsection{Benchmark datasets}
We summarize the benchmark datasets used to evaluate the popularity prediction models reviewed above in Table~\ref{tab:popularity_prediction_datasets}. There are datasets focused on face attractiveness called SCUT-FBP~\cite{xie:smc2015} and SCUT-FBP5500~\cite{liang2018SCUT}. Also, SMPD2019~\cite{Wu2019SMPCA} is specific for social media prediction.

\begin{table*}[t!]
\scriptsize
    \centering
        \caption{Summary of the benchmark datasets for popularity prediction task.}
        \vspace{-3mm}
    \begin{tabular}{c|c|c|c|c|c}
    \Xhline{1.0pt}
      \multicolumn{2}{c|}{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ photos} & Key features & Source \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Yamaguchi~\emph{et al.}~\cite{yamaguchi:mm2014}}} & \makecell{2014} & 328,604 & \makecell[l]{Annotated with title, description, and user-provided labels} & \makecell[l]{Chictopia.com} \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{http://www.hcii-lab.net/data/SCUT-FBP/EN/introduce.html}{SCUT-FBP}%\tablefootnote{\url{http://www.hcii-lab.net/data/SCUT-FBP/EN/introduce.html}}
        ~\cite{xie:smc2015}}} & \makecell{2015} & 500 & \makecell[l]{Asian female face images with attractiveness ratings} & \makecell[l]{Internet} \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://esslab.jp/~ess/en/data/fashion144k_stylenet/}{Fashion144k}%\tablefootnote{\url{https://esslab.jp/~ess/en/data/fashion144k_stylenet/}}
        ~\cite{simoserra:cvpr2015}}} & 2015 & 144,169 & \makecell[l]{Each post contains text in the form of descriptions and garment\\ tags. It also consists of votes or ``likes'' for scaling popularity} & \makecell[l]{Chictopia.com}\\
    \hline
        \multirow{4}{*}{\makecell[l]{Park~\emph{et al.}\\\cite{park:cscw2016}}} & \makecell[l]{Fashion\\ Model\\ Directory} & \multirow{4}{*}{\makecell{2016}} & \multirow{4}{*}{\makecell{N/A}} & \makecell[l]{Profile of fashion models, including name, height, hip size, dress\\ size, waist size, shoes size, list of agencies, and details about all\\ runways the model walked on (year, season, and city)} & \makecell[l]{Fashionmodel-\\directory.com} \\
    \cline{2-2}\cline{5-6}
        & \makecell[l]{Instagram} &  &  & \makecell[l]{Annotated with the number of ``likes'' and comments, as well as the\\ metadata of the first 125 ``likes'' of each post} & \makecell[l]{Instagram} \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{TPIC17~\cite{SMP2017ijcai}}} & \makecell{2017} & 680,000 & \makecell[l]{With time information} & \makecell[l]{Flickr.com} \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Massip~\emph{et al.}~\cite{massip:icmew2018}}} & \makecell{2018} & 6,000 & \makecell[l]{Using textual queries with hashtags of targeted image categories\\ to collect, e.g., \#selfie, or \#friend} & \makecell[l]{Instagram} \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://github.com/HCIILAB/SCUT-FBP5500-Database-Release}{SCUT-FBP5500}%\tablefootnote{\url{https://github.com/HCIILAB/SCUT-FBP5500-Database-Release}}
        ~\cite{liang2018SCUT}}} & \makecell{2018} & 5,500 & \makecell[l]{Frontal faces with various properties (gender, race, ages) and div-\\erse labels (face landmark and beauty score)} & \makecell[l]{Internet} \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Lo~\emph{et al.}~\cite{lo2019icip}}} & \makecell{2019} & 380,000 & \makecell[l]{Within 52 different cities and the timeline was between 2008--2016} & \makecell[l]{lookbook.nu} \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{http://smp-challenge.com/dataset}{SMPD2019}%\tablefootnote{\url{http://smp-challenge.com/dataset}}
        ~\cite{Wu2019SMPCA}}} & \makecell{2019} & 486,000 & \makecell[l]{It contains rich contextual information and annotations} & \makecell[l]{Flickr.com} \\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:popularity_prediction_datasets}
    \begin{tablenotes}
      \scriptsize
      \item N/A: there is no reported information to cite.
    \end{tablenotes}
\end{table*}

%------------------------------------------

\subsubsection{Performance evaluations}
Mean Absolute Percentage Error (MAPE), Mean Absolute Error (MAE), Mean Square Error (MSE), and Spearman Ranking Correlation (SRC) are the most used metrics to evaluate the popularity prediction performance. SRC is to measure the ranking correlation between groundtruth popularity set and predicted popularity set, varying from 0 to 1.


==> ACMCSUR – Fashion/src/fffashion_detection.tex <==
\section{Fashion Detection}
\label{sec:fffashion_detection}

Fashion detection is a widely discussed technology since most fashion works need detection first. Take virtual try-on as an example~\cite{fashionon}. It needs to early detect the human body part of the input image for knowing where the clothing region is and then synthesize the clothing there. Therefore, detection is the basis for most extended works. In this section, we mainly focus on fashion detection tasks, which are split into three aspects: landmark detection, fashion parsing, and item retrieval. For each aspect, state-of-the-art methods, the benchmark datasets, and the performance comparison are rearranged.

%Fashion images consist of an overwhelming number of visual patterns generated by very diverse basic elements, such as the collar and sleeve. Therefore, the objective of fashion image understanding is to construct a structured description of clothing by analyzing an image(s). Notably, there exists a large semantic gap between clothing image representation and their interpretation by humans. In a quest to narrow the semantic gap, recent research efforts on fashion image understanding have concentrated on landmark detection, attribute prediction, and semantic segmentation.


\subsection{Landmark Detection}
\label{subsec:landmark_detection}

Fashion landmark detection %or fashion alignment 
aims to predict the positions of functional keypoints defined on the clothes, such as the corners of the neckline, hemline, and cuff. These landmarks not only indicate the functional regions of clothes, but also implicitly capture their bounding boxes, making the design, pattern, and category of the clothes can be better distinguished. Indeed, features extracted from these landmarks greatly facilitate fashion image analysis.

It is worth mentioning the difference between fashion landmark detection and human pose estimation, which aims at locating human body joints as Fig.~\ref{fig:detection_comparison}(a) shows. 
%As shown in Fig.~\ref{fig:detection_comparison}(a), fashion landmark detection is different from human pose estimation, which aims at locating human body joints such as neck and elbow.
Fashion landmark detection % in clothing images 
is a more challenging task than human pose estimation as the clothes are intrinsically more complicated than human body joints. In particular, garments undergo non-rigid deformations or scale variations, while human body joints usually have more restricted deformations. Moreover, the local regions of fashion landmarks exhibit more significant spatial and appearance variances than those of human body joints, as shown in Fig.~\ref{fig:detection_comparison}(b).

\subsubsection{State-of-the-art methods}

The concept of fashion landmark was first proposed by Liu~\emph{et al.}~\cite{liu2016deepfashion} in 2016, under the assumption that clothing bounding boxes are given as prior information in both training and testing. For learning the clothing features via simultaneously predicting the clothing attributes and landmarks, Liu~\emph{et al.} introduced FashionNet~\cite{liu2016deepfashion}, a deep model. The predicted landmarks were used to pool or gate the learned feature maps, which led to robust and discriminative representations for clothes. In the same year, Liu~\emph{et al.} also proposed a deep fashion alignment (DFA) framework~\cite{liu2016fashion}, which consisted of a three-stage deep convolutional network (CNN), where each stage subsequently refined previous predictions. Yan \emph{et al.}~\cite{yan2017unconstrained} further relaxed the clothing bounding box constraint, which is computationally expensive and inapplicable in practice. The proposed Deep LAndmark Network (DLAN) combined selective dilated convolution and recurrent spatial transformer, where bounding boxes and landmarks were jointly estimated and trained iteratively in an end-to-end manner. Both \cite{liu2016fashion} and \cite{yan2017unconstrained} are based on the regression model.

A more recent work \cite{wang2018attentive} indicated that the regression model is highly non-linear and difficult to optimize. Instead of regressing landmark positions directly, they proposed to predict a confidence map of positional distributions (\textit{i.e.}, heatmap) for each landmark. Additionally, they took into account the fashion grammar to help reason the positions of landmarks. For instance, ``\emph{left collar} $\leftrightarrow$ \emph{left waistline} $\leftrightarrow$ \emph{left hemline}'' that connecting in a human-parts kinematic chain was used as a constraint on the connected clothing parts to model the grammar topology. The human anatomical constraints were inherited in a recurrent neural network. Further, Lee~\emph{et al.}~\cite{Lee2019AGE} considered contextual knowledge of clothes and proposed a global-local embedding module for achieving more accurate landmark prediction performance. Ge~\emph{et al.}~\cite{DeepFashion2} presented a versatile benchmark Deepfashion2 for four tasks, clothes detection, pose estimation, human segmentation, and clothing retrieval, which covered most significant fashion detection works. They built a strong model Match R-CNN based on Mask R-CNN~\cite{maskrcnn2017} for solving the four tasks.

\subsubsection{Benchmark datasets}

As summarized in Table~\ref{tab:landmark_detection_datasets}, there are four benchmark datasets for fashion landmark detection, and the most used is Fashion Landmark Dataset~\cite{liu2016fashion}. These datasets differ in two major aspects: (1) standardization process of the images, and (2) pose and scale variations. 
%A comparison between the Fashion Landmark Detection Benchmark and the Unconstrained Landmark Database is shown in Fig.~\ref{fig:landmark_detection_datasetStatistics} (please refer to~\cite{yan2017unconstrained} for more details). 

%We summarize the benchmark datasets for landmark detection in Table~\ref{tab:landmark_detection_datasets} and provide the links for downloading the datasets if they are available.

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{img/detection_comparison.png}
  \caption{(a) The visual difference between landmark detection and pose estimation. (b) The visual difference between the constrained fashion landmark detection and the unconstrained fashion landmark detection~\cite{yan2017unconstrained}.}
  \label{fig:detection_comparison}
\end{figure}


%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=0.8\linewidth]{img/landmark_detection_FLDvsULD.jpg}
%  \caption{Dataset statistics of Fashion Landmark Detection (FLD)~\cite{liu2016fashion} and Unconstrained Landmark Database (ULD)~\cite{yan2017unconstrained}. `XS', `S', `M', `L', and `XL' respectively represent extreme small, small, medium, large, and extreme large variations.}
%  \label{fig:landmark_detection_datasetStatistics}
%\end{figure}

\begin{table*}[t!]
\scriptsize
    \centering
        \caption{Summary of the benchmark datasets for fashion landmark detection task.}
        \vspace{-3mm}
    \begin{tabular}{l|c|c|c|c|c}
    \Xhline{1.0pt}
      \makecell[c]{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ photos} & \makecell{\# of \\landmark\\ annotations} & Key features & Sources \\
    \hline
        \makecell[l]{\href{http://mmlab.ie.cuhk.edu.hk/projects/DeepFashion/AttributePrediction.html}{DeepFashion-C}%\tablefootnote{\url{http://mmlab.ie.cuhk.edu.hk/projects/DeepFashion/AttributePrediction.html}
        \label{refnote:deepFashionC}
        \cite{liu2016deepfashion}} & 2016 & 289,222 & 8 & \makecell[l]{Annotated with clothing bounding box, pose variation\\ type, landmark visibility, clothing type, category,\\ and attributes} & \makecell[l]{Online shopping\\ sites, Google \\Images}\\  
    \hline
        \makecell[l]{\href{http://mmlab.ie.cuhk.edu.hk/projects/DeepFashion/LandmarkDetection.html}{Fashion Landmark}\\ \href{http://mmlab.ie.cuhk.edu.hk/projects/DeepFashion/LandmarkDetection.html}{Dataset  (FLD)}%\tablefootnote{\url{http://mmlab.ie.cuhk.edu.hk/projects/DeepFashion/LandmarkDetection.html}}
        ~\cite{liu2016fashion}} & 2016 & 123,016 & 8 & \makecell[l]{Annotated with clothing type, pose variation type, \\landmark visibility, clothing bounding box, and \\human body joint} & \makecell[l]{DeepFashion \\\cite{liu2016deepfashion}}\\
    \hline
        \makecell[l]{Unconstrained Land-\\mark Database~\cite{yan2017unconstrained}} & 2017 & 30,000 & 6 & \makecell[l]{The unconstrained datasets are often with cluttered \\background and deviate from image center.\\The visual comparison between constrained and\\ unconstrained dataset is presented in Fig.~\ref{fig:detection_comparison}(b)} & \makecell[l]{Fashion blogs\\ forums,  Deep-\\Fashion~\cite{liu2016deepfashion}}\\
    \hline
        \makecell[l]{\href{https://github.com/switchablenorms/DeepFashion2}{DeepFashion2}%\tablefootnote{\url{https://github.com/switchablenorms/DeepFashion2}}
        ~\cite{DeepFashion2}} & 2019 & 491,000 & \makecell{over 3.5x\\ of ~\cite{liu2016deepfashion}} & \makecell[l]{A versatile benchmark of four tasks including clothes\\ detection, pose estimation, segmentation, and  retrieval} & \makecell[l]{ Deep-Fashion \\\cite{liu2016deepfashion}, Online \\shopping sites}\\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:landmark_detection_datasets}
%    \begin{tablenotes}
%      \scriptsize
%      \item N/A: there is no reported information to cite.
%    \end{tablenotes}
\end{table*}

\subsubsection{Performance evaluations}

\begin{table*}[t!]
%\footnotesize
\notsotiny
%\renewcommand{\arraystretch}{1.2} %extend the table hight
\center
\caption{Performance comparisons of fashion landmark detection methods in terms of normalized error (NE).}
\vspace{-3mm}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
  \Xhline{1.0pt}
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  Dataset & Method & L. Collar & R. Collar & L. Sleeve & R. Sleeve & L. Waistline & R. Waistline & L. Hem & R. Hem & Avg. \\
  \hline
  \multirow{4}{*}{\makecell[l]{DeepFashion\\-C~\cite{liu2016deepfashion}}}% & FashionNet~\cite{liu2016deepfashion} &0.0854 & 0.0902 & 0.0973 & 0.0935 & 0.0854 & 0.0845 & 0.0812 & 0.0823 &0.0872 \\
%  \cline{2-11}
  & \makecell[l]{DFA~\cite{liu2016fashion}} & 0.0628 & 0.0637 & 0.0658 & 0.0621 & 0.0726 & 0.0702 & 0.0658 & 0.0663 & 0.0660 \\
  \cline{2-11}
  & \makecell[l]{DLAN~\cite{yan2017unconstrained}} & 0.0570 & 0.0611 & 0.0672 & 0.0647 & 0.0703 & 0.0694 & 0.0624 & 0.0627 & 0.0643 \\
  \cline{2-11}
  & \makecell[l]{AttentiveNet~\cite{wang2018attentive}} & 0.0415 & 0.0404 & 0.0496 & 0.0449 & 0.0502 & 0.0523 & 0.0537 & 0.0551 & 0.0484 \\
  \cline{2-11}
  & \makecell[l]{Global-Local~\cite{Lee2019AGE}} & \textbf{0.0312} & \textbf{0.0324} & \textbf{0.0427} & \textbf{0.0434} & \textbf{0.0361} & \textbf{0.0373} & \textbf{0.0442} & \textbf{0.0475} & \textbf{0.0393} \\
  \hline
  \hline
  \multirow{4}{*}{\makecell[l]{FLD~\cite{liu2016fashion}}} %& FashionNet~\cite{liu2016deepfashion} &0.0784 & 0.0803 & 0.0975 & 0.0923 & 0.0874 & 0.0821 & 0.0802 & 0.0893 &0.0859 \\
%  \cline{2-11}
  & \makecell[l]{DFA~\cite{liu2016fashion}} & 0.0480 & 0.0480 & 0.0910 & 0.0890 & -- & -- & 0.0710 & 0.0720 & 0.0680 \\
  \cline{2-11}
  & \makecell[l]{DLAN~\cite{yan2017unconstrained}} & 0.0531 & 0.0547 & 0.0705 & 0.0735 & 0.0752 & 0.0748 & 0.0693 & 0.0675 & 0.0672 \\
  \cline{2-11}
  & \makecell[l]{AttentiveNet~\cite{wang2018attentive}} & 0.0463 & 0.0471 & \textbf{0.0627} & \textbf{0.0614} & 0.0635 & 0.0692 & 0.0635 & \textbf{0.0527} & 0.0583 \\
  \cline{2-11}
  & \makecell[l]{Global-Local~\cite{Lee2019AGE}} & \textbf{0.0386} & \textbf{0.0391} & 0.0675 & 0.0672 & \textbf{0.0576} & \textbf{0.0605} & \textbf{0.0615} & 0.0621 & \textbf{0.0568} \\
  \Xhline{1.0pt}
\end{tabular}
\label{table:landmark_detection_result}
    \begin{tablenotes}
      \scriptsize
      \item `L. Collar' represents left collar, while `R. Collar' represents right collar.
      \item ``--'' represents detailed results are not available.
    \end{tablenotes}
\end{table*}

Fashion landmark detection algorithms output the landmark (\textit{i.e.}, functional key point) locations in the clothing images. %The accuracy is evaluated by comparing the detected landmark locations to the ground truth landmark locations.
The normalized error (NE), which is defined as the $\ell_2$ distance between detected and the ground truth landmarks in the normalized coordinate space, is the most popular evaluation metric used in fashion landmark detection benchmarks.  %~\cite{liu2016deepfashion, liu2016fashion, wang2018attentive, yan2017unconstrained, Lee2019AGE}. Besides NE,~\cite{liu2016fashion, yan2017unconstrained} employed the percentage of detected landmarks (PDL), which %is adopted from human pose estimation~\cite{toshev2014deeppose}. PDL
%refers to the percentage of detected landmarks under certain overlapping criterion. Typically, smaller values of NE or higher values of PDL indicate better results.
Typically, smaller values of NE indicates better results. 

We list the performance comparisons of leading methods on the benchmark datasets in Table~\ref{table:landmark_detection_result}. %Lower values are better, and the best are marked in bold. From this comparison, we can observe that contextual knowledge of clothes is crucial for accurate landmark detection, which leads model~\cite{Lee2019AGE} achieved state-of-the-art results on several benchmarks. 
Moreover, the performances of the same method are different across datasets, but the rank is generally consistent.


\subsection{Fashion Parsing}

Fashion parsing, human parsing with clothes classes, is a specific form of semantic segmentation, where the labels are based on the clothing items, such as dress or pants. Example of fashion parsing is shown in Fig.~\ref{fig:fashion_parsing_example}. Fashion parsing task distinguishes itself from general object or scene segmentation problems in that fine-grained clothing categorization requires higher-level judgment based on the semantics of clothing, the deforming structure within an image, and the potentially large number of classes.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{img/FashionParsingExample_IJCAI18.png}
  \caption{Examples of semantic segmentation for fashion images~\cite{ji:ijcai2018}.}
  \label{fig:fashion_parsing_example}
\end{figure}

\subsubsection{State-of-the-art methods}

The early work in fashion parsing was conducted by  %Hasan~\emph{et al.}~\cite{hasan:bmvc2010}. They built a prior shape model by a Markov Random Field (MRF) learning based on pixel-level labels. However, this model can only parse upper-body clothing items (\textit{i.e.}, shirt, jacket, and tie) of an individual whose face is detected. Later, 
Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}. They exploited the relationship between clothing parsing and human pose estimation by refining two problems mutually. % -- predicting a clothing parsing based on estimates of pose, and predicting pose via estimates of clothes parsing. 
Specifically, clothing labels for every image segment were predicted with respect to body parts in a Conditional Random Field %(CRF) 
model. Then the predictions of clothing were incorporated as additional features for pose estimation. Their work, however, mainly focused on constrained parsing problem, where test images were parsed given user-provided tags indicating depicted clothing items. To overcome this limitation,~\cite{KYamaguchi2013, yamaguchi:tpami2014} proposed clothes parsing with a retrieval-based approach. For a given image, similar images from a parsed dataset were first retrieved, and then the nearest-neighbor parsings were transferred to the final result via dense matching. 
%Wu and Boulanger~\cite{wu:tomm2016} later explored the superiority of %Markov Random Fields 
%MRFs over %Conditional Random Fields 
%CRFs for real-time fashion parsing tasks. They applied a modification of MRFs, named reweighted MRF (RW-MRF), to incorporate background prior, occlusion prior, and a reweighted pairwise term. 
Since pixel-level labels required for model training were time-consuming, Liu \emph{et al.}~\cite{SLiu2014TMM} introduced  %an approach to achieve 
the fashion parsing task with weak supervision from the color-category tags instead of pixel-level tags. They combined the human pose estimation module %, the Markov Random Field 
%MRF-based color and category inference module, 
and (super)pixel-level category classifier learning module to generate category classifiers. They then applied the category tags to complete the parsing task.

%-----------This paragraph seems not that related to fashion parsing------------
%For the clothing extraction works, Wu~\emph{et al.}~\cite{wu:mmm2013} proposed extracting clothing region by utilizing coarse region localization based on human proportions and fine foreground/background estimation according to the color distributions. The clothing extraction work was guided by the face detection. A similar idea was proposed in~\cite{zhao:tmm2016}. In particular, Zhao~\emph{et al.}~\cite{zhao:tmm2016} considered the upper body detection along with saliency region detection instead of face detection as in~\cite{wu:mmm2013} to estimate the potential clothing regions.

Different from the abovementioned works %~\cite{hasan:bmvc2010, SLiu2014TMM, KYamaguchi2012CVPR, KYamaguchi2013, yamaguchi:tpami2014, wu:tomm2016, wu:mmm2013, zhao:tmm2016} 
that tended to consider the human pose first, which might lead to sub-optimal results due to the inconsistent targets between pose estimation and clothing parsing, recent research studies mainly attempted to relax this constraint. Dong~\emph{et al.}~\cite{dong2013deformable} proposed to use Parselets, a group of semantic image segments obtained from a low-level over-segmentation algorithm, as the essential elements. A Deformable Mixture Parsing Model (DMPM) based on the ``And-Or'' structure of sub-trees was built to jointly learn and infer the best configuration for both appearance and structure.  Next,~\cite{yang:cvpr2014, XLiang2016TMM} exploited contexts of clothing configuration, \textit{e.g.}, spatial locations and mutual relations of clothes items, to jointly parse a batch of clothing images given the image-level clothing tags. The proposed Clothes Co-Parsing (CCP) framework consists of two phases of inference: (1) image co-segmentation for extracting distinguishable clothes regions by applying exemplar-SVM classifiers, and (2) region co-labeling for recognizing garment items by optimizing a multi-image graphical model. Hidayati~\emph{et al.}~\cite{hidayati:mipr2019} integrated local features and possible body positions from each superpixel as the instances of the price-collecting Steiner tree problem.

In particular, the %aforementioned 
clothing parsing approaches %\cite{hasan:bmvc2010, KYamaguchi2012CVPR, KYamaguchi2013, yamaguchi:tpami2014, dong2013deformable, yang:cvpr2014, XLiang2016TMM, SLiu2014TMM, wu:mmm2013, hidayati:mipr2019, wu:tomm2016} 
based on hand-crafted processing steps need to be designed carefully to capture the complex correlations between clothing appearance and structure fully. To tackle this challenge, %a number of 
some CNN-based approaches have been explored. %Hara~\emph{et al.}~\cite{hara:wacv2015} utilized a deep CNN to generate a set of object proposals in the form of bounding boxes, then applied SVM classifiers to determine if the patch belongs to a particular class. By considering the correlation between the locations of fashion items and the locations of body joints, they incorporated the probability outputs from SVM and pose information to improve the detection performance.
Liang~\emph{et al.}~\cite{liang:tpami2015} developed a framework based on active template regression to locate the mask of each semantic label, rather than assigning a label to each pixel. Two separate convolutional neural networks were utilized to build the end-to-end relation between the input image and the parsing result%, \textit{i.e.}, active template network with max-pooling to predict the template coefficients for each label mask, and active shape network without max-pooling to preserve position sensitiveness for predicting the active shape parameters
. Following~\cite{liang:tpami2015}, Liang~\emph{et al.} later built a Contextualized %Convolutional Neural Network 
CNN (Co-CNN) architecture~\cite{XLiang2015ICCV} to simultaneously capture the cross-layer context, global image-level context, and local super-pixel contexts to improve the accuracy of parsing results.

%The utilization of video contexts to facilitate fashion parsing was proposed by Liu~\emph{et al.}~\cite{liu:mm2014}. The work in \cite{SLiu2015TMM} further improved the performance of \cite{liu:mm2014} by applying an active learning approach that incorporated human guidance to refine the parser. The proposed framework consisted of two components: contextual video parsing to parse all the frames in each unlabelled fashion video simultaneously, and non-parametric human parsing to transfer the parsing labels of the parsed gallery to the test image. A transfer learning approach to address the problem of automatic clothing parsing in the surveillance video was presented in~\cite{zheng:iccasp2017}. The method captured clothing information by training the fashion dataset and applied it to the surveillance domain via multiple-instance transfer learning with weak labels.

%, dong:cvpr2014
To address the issues of parametric and non-parametric human parsing methods that relied on the hand-designed pipelines composed of multiple sequential components, such as in~\cite{KYamaguchi2012CVPR, KYamaguchi2013, dong2013deformable, SLiu2014TMM}, Liu~\emph{et al.} presented a quasi-parametric human parsing framework~\cite{liu:cvpr2015}. The model inherited the merits of both parametric models and non-parametric models by the proposed Matching Convolutional Neural Network (M-CNN), which estimated the matching semantic region between the input image and KNN image. %A cross-domain human parsing problem by exploiting the commonalities across domains was explored by Liu~\emph{et al.}~\cite{liu:aaai2018}. They introduced an adversarial feature and structured label adaptation method to minimize the feature differences between two domains and maximize the label map commonalities. Ji~\emph{et al.}~\cite{ji:ijcai2018} proposed a deformable network for semantic locality-aware segmentation model, which adaptively attached an original clothing image with a semantically similar auxiliary exemplar by search. 
The works~\cite{Gong2017CVPR, liang:tpami2019} proposed self-supervised structure-sensitive learning approaches to explicitly enforce the consistency between the parsing results and the human joint structures. In this way, there is no need for specifically labeling human joints in model training.% Moreover, in the absence of a standard representative collection of images and annotations that could serve as a benchmark for the human parsing task, they presented ``Look into Person (LIP)'' dataset and a public evaluation server.

Unlike previous approaches that only focused on single-person parsing task%~\cite{KYamaguchi2012CVPR, KYamaguchi2013, yamaguchi:tpami2014, dong2013deformable, yang:cvpr2014, XLiang2016TMM, SLiu2014TMM, liang:tpami2015, SLiu2015TMM, liu:cvpr2015, XLiang2015ICCV, Gong2017CVPR, liu:aaai2018, ji:ijcai2018, liang:tpami2019, wu:mmm2013, hidayati:mipr2019, wu:tomm2016, zheng:iccasp2017}, Zhao~\emph{et al.}~\cite{Zhao2018MHP2}, Gong~\emph{et al.}~\cite{gong:eccv2018}, and Ruan~\emph{et al.}~\cite{CE2P2019} 
,~\cite{Zhao2018MHP2, gong:eccv2018, CE2P2019} presented different methods for solving multi-person human parsing. Zhao~\emph{et al.}~\cite{Zhao2018MHP2} presented a deep Nested Adversarial Network\footnote{\url{https://github.com/ZhaoJ9014/Multi-Human-Parsing}} which contained three Generative Adversarial Network (GAN)-like sub-nets for semantic saliency prediction, instance-agnostic parsing, and instance-aware clustering respectively. These three sub-nets jointly learned in an end-to-end training way. Gong~\emph{et al.}~\cite{gong:eccv2018} designed a detection-free Part Grouping Network (PGN) to deal with multi-person human parsing in an image in a single pass. The proposed PGN integrates two twinned subtasks that can be mutually refined under a unified network, \textit{i.e.}, semantic part segmentation, and instance-aware edge detection. Further, Ruan~\emph{et al.}~\cite{CE2P2019} proposed CE2P framework\footnote{\url{https://github.com/liutinglt/CE2P}} containing three key modules, high resolution embedding module, global context embedding module, and edge perceiving module, for single human parsing. This work won the 1$^{st}$ place within all three human parsing tracks in the 2$^{nd}$ Look Into Person (LIP) Challenge\footnote{\url{https://vuhcs.github.io/vuhcs-2018/index.html}}. For multi-person parsing, they designed a global to local prediction process based on CE2P cooperating with Mask R-CNN to form M-CE2P framework and achieved the multi-person parsing goal.

In 2019, hierarchical graph was considered for human parsing tasks~\cite{3wayparsing2019, grapho2019}. Wang~\emph{et al.}~\cite{3wayparsing2019} defined the human body as a hierarchy of multi-level semantic parts and employed three processes (direct, top-down, and bottom-up) to capture the human parsing information for better parsing performance. For tackling human parsing in various domain via a single model without retraining on various datasets, Gong~\emph{et al.}~\cite{grapho2019} comprised hierarchical graph transfer learning based on the conventional parsing network to constitute a general human parsing model, Graphonomy\footnote{\url{https://github.com/Gaoyiminggithub/Graphonomy}}, which consisted of two processes. It first learned and propagated compact high-level graph representation among the labels within one dataset, and then transferred semantic information across multiple datasets. 

%\begin{figure}[t!]
%  \centering
%  \subfigure
%  {\includegraphics[width=0.33\linewidth]{img/fashion_parsing_chictopia01.png}}~~~~
%  \subfigure
%  {\includegraphics[width=0.33\linewidth]{img/fashion_parsing_chictopia02.png}}
%  \vspace{-2mm}
%  \caption{An example of two Chictopia posts.}
%  \label{fig:fashion_parsing_chictopia}
%\end{figure}

%\begin{figure}[t!]
%  \centering
%  \subfigure[The number of images on 19 semantic part labels.]
%  {\includegraphics[width=0.48\linewidth]{img/fashion_parsing_LIP_1.png}}~~~~
%  \subfigure[The number of images that show diverse visibilities.]
%  {\includegraphics[width=0.52\linewidth]{img/fashion_parsing_LIP_2.png}}
%  \vspace{-2mm}
%  \caption{Statistics of the LIP dataset~\cite{Gong2017CVPR, liang:tpami2019}.}
%  \label{fig:fashion_parsing_LIPstatistics}
%\end{figure}

\subsubsection{Benchmark Datasets}

There are multiple datasets for fashion parsing, most of which are collected from Chictopia\footnote{\url{http://chictopia.com}}, a social networking website for fashion bloggers.  %Fig.~\ref{fig:fashion_parsing_chictopia} shows an example of picture and metadata from Chictopia. 
%liu:mm2014, SLiu2015TMM,
%There are some studies~\cite{liang:tpami2015, liu:aaai2018} that combined existing datasets to form a new one that suited their needs. For example, the study in~\cite{liang:tpami2015} not only constructed the Human Parsing in the Wild dataset, but also combined three other datasets (\textit{i.e.}, the Fashionista dataset~\cite{KYamaguchi2012CVPR}, the Colorful Fashion Parsing Data dataset~\cite{SLiu2014TMM}, and the Daily Photos dataset~\cite{dong2013deformable}) to enlarge the diversity of their data used to train the deep network model. 
Table~\ref{tab:clothing_parsing_datasets} summarizes the benchmark datasets for fashion parsing in more detail. To date, the most comprehensive one is the LIP dataset~\cite{Gong2017CVPR, liang:tpami2019}, containing over 50,000 annotated images with 19 semantic part labels captured from a wider range of viewpoints, occlusions, and background complexity. 
%We present statistics of the LIP dataset in terms of the number of images per label and per visibility condition in Fig.~\ref{fig:fashion_parsing_LIPstatistics}(a) and~\ref{fig:fashion_parsing_LIPstatistics}(b), respectively. 

\begin{table*}[t!]
\renewcommand{\arraystretch}{1.1}
\notsotiny
    \centering
        \caption{Summary of the benchmark datasets for fashion parsing task.}
        \vspace{-3mm}
    \begin{tabular}{l|c|c|c|c|l|c}
    \Xhline{1.0pt}
        \multicolumn{2}{c|}{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ photos} & \makecell{\# of\\classes} & \makecell[c]{Key features} & Sources \\
    %\hline
    %    \multicolumn{2}{c|}{\makecell[l]{Hasan~\emph{et al.}~\cite{hasan:bmvc2010}}} & 2010 & 117 & 6 &  \makecell[l]{There are 42 people in total} & \makecell[l]{N/A}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{http://vision.is.tohoku.ac.jp/~kyamagu/research/clothing_parsing/}{Fashionista dataset}%\tablefootnote{\url{http://vision.is.tohoku.ac.jp/~kyamagu/research/clothing_parsing/}}
        ~\cite{KYamaguchi2012CVPR}}} & 2012 & 158,235 & 56 & \makecell[l]{Annotated with tags, comments, and links} & \makecell[l]{Chictopia.com}\\ % 50/291/6,565
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Daily Photos (DP)~\cite{dong2013deformable}}} & 2013 & 2,500 & 18 & \makecell[l]{High resolution images; Parselet definition} & \makecell[l]{Chictopia.com}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{http://vision.is.tohoku.ac.jp/~kyamagu/research/paperdoll/}{Paper Doll dataset}%\tablefootnote{\url{http://vision.is.tohoku.ac.jp/~kyamagu/research/paperdoll/}}\\
        ~\cite{KYamaguchi2013, yamaguchi:tpami2014}}} & 2013 & 339,797 & 56 & \makecell[l]{Annotated with metadata tags denoting characteris-\\tics, \emph{e.g.}, color, style, occasion, clothing type, brand} & \makecell[l]{Fashionista~\cite{KYamaguchi2012CVPR}, \\ Chictopia.com}\\
%    \hline
%       \multirow{2}{*}{\makecell[l]{Wu~\emph{et al.}\\\cite{wu:mmm2013}}} & \makecell[l]{Taobao} & \multirow{2}{*}{2013} & 1.35M & \multirow{2}{*}{2} & \multirow{2}{*}{\makecell[l]{Annotated with category labels}} & \makecell[l]{Taobao.com}\\
%    \cline{2-2}\cline{4-4}\cline{7-7}
%        & \makecell[l]{Mogujie} & & 1,000 & & & \makecell[l]{Mogujie.com}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://github.com/bearpaw/clothing-co-parsing}{Clothing Co-Parsing (CCP)}\\ \href{https://github.com/bearpaw/clothing-co-parsing}{SYSU-Clothes}%\tablefootnote{\url{https://github.com/bearpaw/clothing-co-parsing}}
        ~\cite{yang:cvpr2014, XLiang2016TMM}}} & 2014 & 2,098 & 57 & \makecell[l]{Annotated with superpixel-level or image-level tags} & \makecell[l]{Online shopping websites}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://sites.google.com/site/fashionparsing/home}{Colorful-Fashion Dataset}\\ \href{https://sites.google.com/site/fashionparsing/home}{(CFD)}%\tablefootnote{\url{https://sites.google.com/site/fashionparsing/home}}
        ~\cite{SLiu2014TMM}}} & 2014 & 2,682 & 23 & \makecell[l]{Annotated with 13 colors} & \makecell[l]{Chictopia.com}\\ %86/490/1,341
%    \hline 
%        \multirow{2}{*}{\makecell[l]{Liu~\emph{et al.}\\\cite{liu:mm2014, SLiu2015TMM}}} & \makecell[l]{Video dataset} & \multirow{2}{*}{2014} & N/A & N/A & \makecell[l]{1,500 videos with the lengths of 2 to 10 seconds} & \makecell[l]{MVs of the singers,\\dance teaching videos,\\fashion shows,\\ fashion TV dramas,\\big evening parties}\\
%    \cline{2-2}\cline{4-7} 
%        & \makecell[l]{Fashion Icon\\image dataset}  &  & 1,082 & 18 & \makecell[l]{Multiple humans; diverse poses} & \makecell[l]{Website}\\
    \hline 
        \multirow{3}{*}{\makecell[l]{ATR~\cite{liang:tpami2015}}} & \makecell[l]{Benchmark} & \multirow{3}{*}{2015} & 5,867 & \multirow{3}{*}{18} & \makecell[l]{Standing people in frontal/near-frontal view with good\\ visibilities of all body parts} & \makecell[l]{Fashionista~\cite{KYamaguchi2012CVPR}, Daily\\ Photos~\cite{dong2013deformable}, CFD~\cite{SLiu2014TMM}}\\
    \cline{2-2}\cline{4-4}\cline{6-7} 
        & \makecell[l]{Human Parsing\\ in the Wild}  &  & 1,833 &  & \makecell[l]{Annotated with pixel-level labels} & \makecell[l]{N/A}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Chictopia10k~\cite{XLiang2015ICCV}}} & 2015 & 10,000 & 18 & \makecell[l]{ It contains real-world images with arbitrary postures,\\ views and backgrounds} & \makecell[l]{Chictopia.com}\\
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{Clothing CoSegmentation\\ dataset (CCS)~\cite{zhao:tmm2016}}} & 2016 & 1,000 & N/A & \makecell[l]{ It includes 304 groups, and each group has 2$\sim$7\\ images with fashion models wearing the same clothing} & \makecell[l]{Taobao.com}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{http://hcp.sysu.edu.cn/li}{LIP}%\tablefootnote{\url{http://hcp.sysu.edu.cn/li}}
        ~\cite{Gong2017CVPR, liang:tpami2019}}} & 2017 & 50,462 & 20 & \makecell[l]{Annotated with pixel-wise and body joints} & \makecell[l]{Microsoft COCO~\cite{lin:eccv2014}}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://sukixia.github.io/paper.html}{PASCAL-Person-Part}%\tablefootnote{\url{https://sukixia.github.io/paper.html}}
        ~\cite{Pascal2017}}} & 2017 & 3,533 & 14 & \makecell[l]{It contains multiple humans per image in uncon-\\strained poses and occlusions} & \makecell[l]{N/A}\\
    \hline 
        \multirow{2}{*}{\makecell[l]{\href{https://lv-mhp.github.io/dataset}{MHP}%\tablefootnote{\url{https://lv-mhp.github.io/dataset}}
        }} & \makecell[l]{v1.0~\cite{li2017MHP1}} & 2017 & 4,980 & 18 & \makecell[l]{There are 7 body parts and 11 clothes and accessory\\ categories} & \makecell[l]{N/A}\\
    \cline{2-7} 
        & \makecell[l]{v2.0~\cite{Zhao2018MHP2}}  & 2018 & 25,403 & 58 & \makecell[l]{There are 11 body parts and 47 clothes and accessory\\ categories} & \makecell[l]{N/A}\\  
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{http://sysu-hcp.net/lip/overview.php}{Crowd Instance-level Human}\\\href{http://sysu-hcp.net/lip/overview.php}{Parsing (CIHP)}%\tablefootnote{\url{http://sysu-hcp.net/lip/overview.php}}
        ~\cite{gong:eccv2018}}} & 2018 & 38,280 & 19 & \makecell[l]{Multiple-person images; pixel-wise annotations in\\ instance-level} & \makecell[l]{Google, Bing}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://github.com/eBay/modanet}{ModaNet}%\tablefootnote{\url{https://github.com/eBay/modanet}}
        ~\cite{zheng:mm2018}}} & 2018 & 55,176 & 13 & \makecell[l]{Annotated with pixel-level labels, bounding boxes,\\ and polygons} & \makecell[l]{PaperDoll~\cite{KYamaguchi2013}}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://github.com/switchablenorms/DeepFashion2}{DeepFashion2}%\tablefootnote{\url{https://github.com/switchablenorms/DeepFashion2}}
        ~\cite{DeepFashion2}}} & 2019 & 491,000 & 13 & \makecell[l]{A versatile benchmark of four tasks including clothes\\ detection, pose estimation, segmentation, and  retrieval.} & \makecell[l]{ DeepFashion~\cite{liu2016deepfashion},\\ Online shopping websites}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://fashionpedia.github.io/home/}{Fashionpedia}%\tablefootnote{\url{https://fashionpedia.github.io/home/}}
        ~\cite{fashionpedia2020eccv}}} & 2020 & 48,000 & 46 & \makecell[l]{There are 294 fine-grained attributes. It contains high\\ resolution with 1710 $\times$ 2151 to maintain more details} & \makecell[l]{Flickr, Free license\\ photo websites}\\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:clothing_parsing_datasets}
    \begin{tablenotes}
      \scriptsize
      \item N/A: there is no reported information to cite
    \end{tablenotes}
\end{table*}

\subsubsection{Performance Evaluations}

There are multiple metrics for evaluating fashion parsing methods: %(1) Balanced-Accuracy for the correct labelling compared to the ground-truth segmentations; 
(1) average Pixel Accuracy (aPA) as the proportion of correctly labeled pixels in the whole image, (2) mean Average Garment Recall (mAGR), (3) Intersection over Union (IoU) as the ratio of the overlapping area of the ground truth and predicted area to the total area, (4) mean accuracy, (5) average precision, (6) average recall, (7) average F-1 score over pixels, and (8) foreground accuracy as the number of true pixels on the body over the number of actual pixels on the body.
%

% mAGR is measured by computing the average labeling performance (recall) of the garment items present in an image and then the mean is computed across all images
% average Pixel Accuracy (aPA), which is defined as the proportion of correctly labeled pixels in the whole image




%\begin{table*}[t!]
%\footnotesize
%    \centering
%        \caption{Evaluation metrics used for fashion parsing task.}
%        \vspace{-3mm}
%    \begin{tabular}{l|c|c|c|c|c|c|c|c}
%    \Xhline{1.0pt}
%         Method & %\makecell{Balanced-\\Accuracy} & 
%         \makecell{aPA} & \makecell{mAGR} & \makecell{IoU} & \makecell{mean\\accuracy} & \makecell{Average\\precision} & \makecell{Average\\recall} & \makecell{Avg. F-1\\ over pixels} & \makecell{Foreground\\accuracy} \\
    %\hline
        %Hasan~\emph{et al.}~
    %    \cite{hasan:bmvc2010} & \checkmark &  &  &  &  &  &  &  &  \\
%    \hline
        %Yamaguchi~\emph{et al.}~
%        \cite{KYamaguchi2012CVPR, wu:tomm2016, yang:cvpr2014, XLiang2016TMM} & \checkmark & \checkmark &  &  &  &  &  &  \\
%    \hline
        %Dong~\emph{et al.}~
%        \cite{dong2013deformable,dong:cvpr2014, liang:tpami2019, Gong2017CVPR, ji:ijcai2018} & \checkmark &  & \checkmark &  &  &  &  &    \\
%    \hline
        %Liang~\emph{et al.}~
%        \cite{CE2P2019} & \checkmark &  & \checkmark & \checkmark &  &  &  &  \\
%    \hline
        %Liang~\emph{et al.}~
%        \cite{3wayparsing2019} & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
%    \hline
%        \cite{SLiu2014TMM, zheng:iccasp2017, Pascal2017} &  &  & \checkmark &  &  &  &  &  \\
%    \hline
        %Gong~\emph{et al.}~
%        \cite{Zhao2018MHP2} &  &  & \checkmark &  &  \checkmark &  &  &  \\
%    \hline
        %Gong~\emph{et al.}~
%        \cite{gong:eccv2018} &  &  & \checkmark &  &  \checkmark &  &  &   \\
%    \hline
        %Gong~\emph{et al.}~
%        \cite{grapho2019} &  &  & \checkmark & \checkmark &   &  & \checkmark &   \\
%    \hline
        %Wu~\emph{et al.}~
%        \cite{wu:mmm2013, zhao:tmm2016} &  &  &  & \checkmark &  &  &  &  \\
%    \hline
        %Liang~\emph{et al.}~
%        \cite{liang:tpami2015, liu:cvpr2015} &  &  &  & \checkmark & \checkmark & \checkmark & \checkmark &  \\
%    \hline
        %Liang~\emph{et al.}~
%        \cite{XLiang2015ICCV, SLiu2015TMM, liu:aaai2018,KYamaguchi2013, liu:mm2014, yamaguchi:tpami2014} &  &  &  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark\\
%    \hline
        %Hara~\emph{et al.}~
%        \cite{DeepFashion2} &  &  &  &  & \checkmark &  &  &  \\    
    %\hline
        %Hara~\emph{et al.}~
        %\cite{hara:wacv2015} &  &  &  &  & \checkmark & \checkmark &  &  \\
%    \hline
        %Hidayati~\emph{et al.}~
%        \cite{hidayati:mipr2019} &  &  &  &  &  \checkmark & \checkmark & \checkmark &  \\
%    \Xhline{1.0pt}
%    \end{tabular}
%    \label{tab:clothing_parsing_evaluation_metrics}
%\end{table*}

In particular, most of the parsing methods %introduced above 
are evaluated on Fashionista dataset~\cite{KYamaguchi2012CVPR} in terms of accuracy, average precision, average recall, and average F-1 score over pixels. We %list the evaluation metrics used by each work in Table~\ref{tab:clothing_parsing_evaluation_metrics} and 
report the performance comparisons in Table 1 of Supplementary Material.

\begin{comment}
\begin{table*}[t!]
\renewcommand{\arraystretch}{1.1}
\scriptsize
    \centering
        \caption{Performance comparisons of fashion parsing methods (in \%).}
        \vspace{-3mm}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \Xhline{1.0pt}
        \multirow{2}{*}{\makecell{Evaluation\\protocol}} & \multirow{2}{*}{\makecell[l]{Dataset}} & \multirow{2}{*}{\makecell{Method}} & \multicolumn{8}{c}{\makecell{Evaluation metric}}\\
     \cline{4-11}   
        & & & \makecell{mIOU} & \makecell[l]{aPA} & \makecell[l]{mAGR} & \makecell[l]{Acc.} & \makecell[l]{Fg. acc.} & \makecell[l]{Avg. prec.} & \makecell[l]{Avg. recall} & \makecell[l]{Avg. F-1}\\
%    \hline\hline
%        \multirow{4}{*}{\makecell[l]{\cite{dong2013deformable}}} & \multirow{2}{*}{\makecell[l]{Fashionista}} & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & 29.90 & 77.60 & -- & -- & -- & -- & -- & -- & --\\
%    \cline{3-12}
%         &  & \makecell[l]{DMPM~\cite{dong2013deformable}} & \textbf{51.70} & \textbf{83.10} & -- & -- & -- & -- & -- & -- & --\\
%    \cline{2-12}
%         & \multirow{2}{*}{\makecell[l]{Daily Photos}} & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & 24.60 & 76.60 & -- & -- & -- & -- & -- & -- & --\\
%    \cline{3-12}
%         &  & \makecell[l]{DMPM~\cite{dong2013deformable}} & \textbf{53.00} & \textbf{84.60} & -- & -- & -- & -- & -- & -- & --\\
%    \hline\hline
%        \multirow{2}{*}{\makecell[l]{\cite{SLiu2014TMM}}} & \multirow{2}{*}{\makecell[l]{CFD}} & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & 38.20 & -- & -- & -- & -- & -- & -- & --\\
%    \cline{3-12}
%        &  & \makecell[l]{Liu~\emph{et al.}~\cite{SLiu2014TMM}} & -- & \textbf{42.10} & -- & -- & -- & -- & -- & -- & --\\
%    \hline\hline
%        \multirow{2}{*}{\makecell[l]{\cite{wu:tomm2016}}} & \multirow{2}{*}{\makecell[l]{Fashionista}} & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}}  & -- & 85.10 & 57.20 & -- & -- & -- & -- & --\\
%    \cline{3-11}
%        &  & \makecell[l]{RW-MRF~\cite{wu:tomm2016}} & --  & \textbf{90.50} & \textbf{63.00} & -- & -- & -- & -- & --\\
    \hline\hline
        \multirow{4}{*}{\makecell[l]{\cite{yang:cvpr2014, XLiang2016TMM}}} & \multirow{2}{*}{\makecell[l]{SYSU-clothes}} & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & 85.97 & 51.25 & -- & -- & -- & -- & --\\
    \cline{3-11}
         &  & \makecell[l]{CCP~\cite{yang:cvpr2014, XLiang2016TMM}} & -- & 88.23 & 63.89 & -- & -- & -- & -- & --\\
    \cline{2-11}
         & \multirow{2}{*}{\makecell[l]{Fashionista}} & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & 89.00 & 64.37 & -- & -- & -- & -- & --\\
    \cline{3-11}
         &  & \makecell[l]{CCP~\cite{yang:cvpr2014, XLiang2016TMM}} & -- & \textbf{90.29} & \textbf{65.52} & -- & -- & -- & -- & --\\
%    \hline\hline
%        \multirow{2}{*}{\makecell[l]{\cite{KYamaguchi2013, yamaguchi:tpami2014}}} & \multirow{2}{*}{\makecell[l]{Paper Doll}} & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & -- & -- & 77.45 & 23.11 & 10.53 & \textbf{17.20} & 10.35\\
%    \cline{3-11}
%        &  & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2013, yamaguchi:tpami2014}} & -- & -- & -- & \textbf{84.68} & \textbf{40.20} & \textbf{33.34} & 15.34 & \textbf{14.87}\\
%    \hline\hline
%        \multirow{4}{*}{\makecell[l]{\cite{SLiu2015TMM}}} & \multirow{2}{*}{\makecell[l]{CFD}}& \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2013, yamaguchi:tpami2014}} & -- & -- & -- & 85.69 & 52.09 & 41.74 & \textbf{45.15} & 37.43\\
%    \cline{3-11}
%        &  & \makecell[l]{Liu~\emph{et al.}~\cite{SLiu2015TMM}} & -- & -- & -- & \textbf{88.92} & \textbf{58.68} & \textbf{57.68} & 43.57 & \textbf{44.90}\\
%    \cline{2-11}
%        & \multirow{2}{*}{\makecell[l]{Fashionista}}& \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2013, yamaguchi:tpami2014}} & -- & -- & -- & 82.79 & 44.08 & \textbf{49.20} & 32.00 & 32.66\\
%    \cline{3-11}
%        &  & \makecell[l]{Liu~\emph{et al.}~\cite{SLiu2015TMM}} & -- & -- & -- & \textbf{85.97} & \textbf{54.66} & 43.90 & \textbf{42.42} & \textbf{41.35}\\
    \hline\hline
        \multirow{6}{*}{\makecell[l]{\cite{XLiang2015ICCV}}} & \multirow{3}{*}{\makecell[l]{ATR}} & %\makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & -- & -- & 84.38 & 55.59 & 37.54 & 51.05 & 41.80\\
%    \cline{3-11}
%         &  & 
         \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2013, yamaguchi:tpami2014}} & -- & -- & -- & 88.96 & 62.18 & 52.75 & 49.43 & 44.76\\
%    \cline{3-11}
%         &  & \makecell[l]{Liu~\emph{et al.}~\cite{liu:cvpr2015}} & -- & -- & -- & 89.57 & 73.98 & 64.56 & 65.17 & 62.81\\
    \cline{3-11}
         &  & \makecell[l]{Liang~\emph{et al.}~\cite{liang:tpami2015}} & -- & -- & -- & 91.11 & 71.04 & 71.69 & 60.25 & 64.38\\
    \cline{3-11}
         &  & \makecell[l]{Co-CNN~\cite{XLiang2015ICCV}} & -- & -- & -- & \textbf{96.02} & \textbf{83.57} & \textbf{84.95} & \textbf{77.66} & \textbf{80.14}\\
    \cline{2-11}
         & \multirow{3}{*}{\makecell[l]{Fashionista}} & %\makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & -- & -- & 87.87 & 58.85 & 51.04 & 48.05 & 42.87\\
%    \cline{3-11}
%         &  & 
        \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2013, yamaguchi:tpami2014}} & -- & -- & -- & 89.98 & 65.66 & 54.87 & 51.16 & 46.80 \\
    \cline{3-11}
         &  & \makecell[l]{Liang~\emph{et al.}~\cite{liang:tpami2015}} & -- & -- & -- & 92.33 & 76.54 & 73.93 & 66.49 & 69.30\\
    \cline{3-11}
         &  & \makecell[l]{Co-CNN~\cite{XLiang2015ICCV}} & -- & -- & -- & \textbf{97.06} & \textbf{89.15} & \textbf{87.83} & \textbf{81.73} & \textbf{83.78}\\
    \hline\hline
        \multirow{12}{*}{\makecell[l]{\cite{3wayparsing2019}}} & \multirow{3}{*}{\makecell[l]{LIP}} & %\makecell[l]{FCN-8s~\cite{long2015fully}} & 28.29 & 76.06 & -- & 36.75 & -- & -- & -- &  --\\
%    \cline{3-11}
%         &  & 
%        \makecell[l]{SSL~\cite{Gong2017CVPR}} & 44.73 & 84.36 & -- & 54.94 & -- & -- & -- & --\\
%    \cline{3-11}
%         &  & 
        \makecell[l]{MuLA~\cite{nie2018mula}} & 49.30 & \textbf{88.50} & -- & 60.50 & -- & -- & -- & --\\
    \cline{3-11}
         &  & \makecell[l]{CE2P~\cite{CE2P2019}} & 53.10 & 87.37 & -- & 63.20 & -- & -- & -- & --\\
    \cline{3-11}
         &  & \makecell[l]{Wang~\emph{et al.}\cite{3wayparsing2019}} & \textbf{57.74} & 88.03 & -- & \textbf{68.80} & -- & -- & -- & --\\
    \cline{2-11}
         & \multirow{3}{*}{\makecell[l]{PASCAL-\\Person-Part}} & %\makecell[l]{SSL~\cite{Gong2017CVPR}} & 59.36 & -- & -- & -- & -- & -- & -- & --\\
%    \cline{3-11}
%         &  & 
         \makecell[l]{MuLA~\cite{nie2018mula}} & 65.10 & -- & -- & -- & -- & -- & -- & --\\
%    \cline{3-11}
%         &  & \makecell[l]{WSHP~\cite{WSHP2018cvpr}} & 67.60 & -- & -- & -- & -- & -- & -- & --\\
    \cline{3-11}
         &  & \makecell[l]{PGN~\cite{gong:eccv2018}} & 68.40 & -- & -- & -- & -- & -- & -- & --\\
    \cline{3-11}
         &  & \makecell[l]{Wang~\emph{et al.}~\cite{3wayparsing2019}} & \textbf{70.76} & -- & -- & -- & -- & -- & -- & --\\
    \cline{2-11}
         & \multirow{3}{*}{\makecell[l]{ATR}} & %\makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & 84.38 & -- & -- & 55.59 & 37.54 & 51.05 & 41.80\\
%    \cline{3-11}
%         &  & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2013}} & -- & 88.96 & -- & -- & 62.18 & 52.75 & 49.43 & 44.76\\
%    \cline{3-11}
%         &  & 
         \makecell[l]{Co-CNN~\cite{XLiang2015ICCV}} & -- & 96.02 & -- & -- & 83.57 & \textbf{84.95} & 77.66 & 80.14\\
    \cline{3-11}
         &  & \makecell[l]{TGPNet~\cite{TGPNet2018mm}} & -- & \textbf{96.45} & -- & -- & \textbf{87.91} & 83.36 & 80.22 & 81.76\\
    \cline{3-11}
         &  & \makecell[l]{Wang~\emph{et al.}~\cite{3wayparsing2019}} & -- & 96.26 & -- & -- & \textbf{87.91} & 84.62 & \textbf{86.41} & \textbf{85.51}\\
    \cline{2-11}
         & \multirow{3}{*}{\makecell[l]{CFD +\\Fashionista +\\CCP}} & %\makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & 81.32 & -- & -- & 32.24 & 23.74 & 23.68 & 22.67\\
%    \cline{3-11}
%         &  & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2013}} & -- & 87.17 & -- & -- & 50.59 & 45.80 & 34.20 & 35.13\\
%    \cline{3-11}
%         &  & 
        \makecell[l]{Deeplab~\cite{chen2018deeplab}} & -- & 87.68 & -- & -- & 56.08 & 35.35 & 39.00 & 37.09\\
     \cline{3-11}
         &  & \makecell[l]{TGPNet~\cite{TGPNet2018mm}} & -- & 91.25 & -- & -- & 66.37 & 50.71 & 53.18 & 51.92\\
    \cline{3-11}
         &  & \makecell[l]{Wang~\emph{et al.}\cite{3wayparsing2019}} & -- & \textbf{92.20} & -- & -- & \textbf{68.59} & \textbf{56.84} & \textbf{59.47} & \textbf{58.12}\\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:fashion_parsing_results}
    \begin{tablenotes}
      \scriptsize
      \item ``--'' represents detailed results are not available.
    \end{tablenotes}
\end{table*}
\end{comment}

%\subsubsection{Body Shape Under Clothing.}
%reorganize for this subsubsection
%Estimating the body shape of a dressed human is a highly under-constrained problem. To cope with this problem, most existing methods exploited statistical 3D body models, like SCAPE~\cite{anguelov:tog2005} or its variants. In \cite{wuhrer:cviu2014}, Wuhrer~\emph{et al.} introduced a posture-invariant shape space to model body shape variation combined with a skeleton-based deformation to model posture variation. Neophytou and Hilton~\cite{neophytou:ic3v2014} proposed to use a layered model of cloth and estimate the body shape by detecting areas where clothing fits closely to the body. Yang~\emph{et al.}~\cite{yang:eccv2016} formulated an optimization problem that models body shape variations and posture variations as linear factors in a shape space. More recently, Zhang~\emph{et al.}~\cite{zhang:cvpr2017} considered temporal information in a sequence to provide constraints on the underlying body shape by fusing all clothed registrations into a single frame.

\subsection{Item Retrieval}
\label{subsec:item_retrieval}

As fashion e-commerce has grown over the years, there has been a high demand for innovative solutions to help customers find preferred fashion items with ease.
Though many fashion online shopping sites support keyword-based searches, there are many visual traits of fashion items that are not easily translated into words. It thus attracts tremendous attention from many research communities to develop cross-scenario image-based fashion retrieval tasks for matching the real-world fashion items to the online shopping image. Given a fashion image query, the goal of image-based fashion item retrieval is to find similar or identical items from the gallery. 


\subsubsection{State-of-the-art methods}

The notable early work on automatic image-based clothing retrieval was presented by Wang and Zhang~\cite{wang2011clothes}. To date, extensive research studies have been devoted to addressing the problem of cross-scenario clothing retrieval since there is a large domain discrepancy between daily human photo captured in general environment and clothing images taken in ideal conditions (\textit{i.e.}, embellished photos used in online clothing shops). %The illustration of cross-scenario clothing retrieval is presented in Fig.~\ref{fig:clothing_retrieval_street2shop}. 
Liu~\emph{et al.}~\cite{liu2012street} proposed to utilize an unsupervised transfer learning method based on part-based alignment and features derived from the sparse reconstruction.  %Fu~\emph{et al.}~\cite{fu:accv2012} proposed a semantic-preserving visual phrases (SPVP) representation, which encoded the regions of human parts refined with sparse background reconstruction into the vocabulary tree under the bag-of-visual-word (BOW) framework. 
Kalantidis~\emph{et al.}~\cite{kalantidis:icmr2013} presented clothing retrieval from the perspective of human parsing. A prior probability map of the human body was obtained through pose estimation to guide clothing segmentation, and then the segments were classified through locality-sensitive hashing. The visually similar items were retrieved by summing up the overlap similarities. Notably,~\cite{wang2011clothes, liu2012street, kalantidis:icmr2013} are based on hand-crafted features.
%, chi:mtap2016, fu:accv2012


%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=0.45\linewidth]{img/clothing_retrieval_street2shop.png}
%  \caption{\textcolor{red}{An illustration of cross-scenario clothing retrieval model.}}
%  \label{fig:clothing_retrieval_street2shop}
%\end{figure}

%Early works on image-based clothing retrieval are mostly based on hand designed features~\cite{wang2011clothes, liu2012street, fu:accv2012, kalantidis:icmr2013, kovashka:cvpr2012, kovashka:ijcv2015, li:viscomput2016}.

With the advances of deep learning, there has been a trend of building deep neural network architectures to solve the clothing retrieval task. %Huang~\emph{et al.}~\cite{huang:mm2014} developed an attribute-aware clothing retrieval system using a holistic tree-structure convolutional neural network that integrated multiple clothing attributes simultaneously. Later, Huang further published~\cite{huang2015cross} for proposing a Dual Attribute-aware Ranking Network (DARN) %, two sub-networks with similar structure, one for each domain,
Huang~\emph{et al.}~\cite{huang2015cross} developed a Dual Attribute-aware Ranking Network (DARN) to represent in-depth features using attribute-guided learning. DARN simultaneously embedded semantic attributes and visual similarity constraints into the feature learning stage, while at the same time modeling the discrepancy between domains. %Liang~\emph{et al.}~\cite{XLiang2016TMM} incorporated clothing parsing into clothing retrieval. Given a query clothing image, they first parsed it into fine-grained semantic regions by the proposed clothes co-parsing framework formulated as a probabilistic model, then retrieved clothing items from online shopping images. 
Li~\emph{et al.}~\cite{li:icpr2016} presented a hierarchical super-pixel fusion algorithm for obtaining the intact query clothing item and used sparse coding for improving accuracy. More explicitly, an over-segmentation hierarchical fusion algorithm with human pose estimation was utilized to get query clothing items and to retrieve similar images from the product clothing dataset. % To improve the accuracy of the classifiers and the adaptability of the dictionary for recognizing clothing styles in different scenarios, the intermediate domain dictionaries between product clothing dataset and daily clothing dataset were learned sequentially during the recognition phase. 

% chi:mtap2016, sanchez-riera:mmm2017
The abovementioned studies %~\cite{wang2011clothes, liu2012street, fu:accv2012, kalantidis:icmr2013, huang:mm2014, huang2015cross, li:icpr2016} 
are designed for similar fashion item retrieval. But more often, people desire to find the same fashion item, as illustrated in Fig.~\ref{fig:_retrieval_attribute_example}(a). The first attempt on this task was achieved %in 2015 
by Kiapour~\emph{et al.}~\cite{kiapour:iccv2015}, who developed three different methods for retrieving the same fashion item in the real-world image from the online shop, the street-to-shop retrieval task. The three methods contained two deep learning baseline methods, and one method aimed to learn the similarity between two different domains, street and shop domains. %Also, they collected a large scale dataset, \textit{Exact Street2Shop Dataset}, including 404,683 shop photos. 
For the same goal of learning the deep feature representation, Wang~\emph{et al.}~\cite{wang:icmr2016} adopted a Siamese network that contained two copies of the Inception-6 network with shared weights. Also, they introduced a \textit{robust contrastive loss} to alleviate over-fitting caused by some positive pairs (containing the same product) that were visually different, and used one multi-task fine-tuning approach to learn a better feature representation by tuning the parameters of the siamese network with product images and general images from ImageNet~\cite{imagenet2009}. Further, Jiang~\emph{et al.} ~\cite{jiang:mm2016} extended the one-way problem, street-to-shop retrieval task, to the bi-directional problem, street-to-shop and shop-to-street clothing retrieval task. They proposed a deep bi-directional cross-triplet embedding algorithm to model the similarity between cross-domain photos, and further expanded the utilization of this approach to retrieve a series of representative and complementary accessories %(\textit{e.g.}, bags, shoes) 
to pair with the shop item~\cite{jiang:tomm2018}. %For considering the influence of different view angles on clothing retrieval tasks, Liu~\emph{et al.}~\cite{liu:icmr2016} collected a Multi-View Clothing Dataset containing 161,638 clothing images, and most of them had four different viewpoints.
Moreover, Cheng~\emph{et al.}~\cite{ZQCheng2017CVPR} increased the difficulty of image-based %street-to-shop retrieval tasks 
to video-based street-to-shop retrieval tasks%. For the video-based task, it 
, which was more challenging because of the diverse viewpoint or motion blur%, which would cause significant visual discrepancy
. They introduced three networks: %to solve the video2shop task, 
Image Feature Network, Video Feature Network, and Similarity Network. They first did clothing detection and tracking for generating clothing trajectories. Then, Image Feature Network extracted deep visual features which would be fed into the %Long Short-Term Memory 
LSTM framework for capturing the temporal dynamics in the Video Feature Network, and finally went to Similarity Network for pair-wise matching. %To focus the video domain on popular film and TV show, Garcia~\emph{et al.}\cite{garcia:iccvw2017} proposed a framework based on frame retrieval and fast indexing algorithm.
For improving the existing algorithms for retrieval tasks, which only considered global feature vectors,~\cite{FashionRV2019} proposed a Graph Reasoning Network to build the similarity pyramid, which represented the similarity between a query and a gallery clothing by considering both global and local representation. %Besides, they built a new benchmark dataset, FindFashion Dataset, by revisiting \textit{Street2Shop}~\cite{kiapour:iccv2015} and \textit{DeepFashion}~\cite{liu2016deepfashion}. 


%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=0.5\linewidth]{img/clothing_retrieval_exactRetrieval.png}
%  \caption{An illustration of exact clothing retrieval~\cite{kiapour:iccv2015}.}
%  \label{fig:clothing_retrieval_exactRetrieval}
%\end{figure}

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{img/Example_ItemRetrieval_AttributeRecognition.png}
  \caption{(a) An illustration of exact clothing retrieval~\cite{kiapour:iccv2015}. (b) An example for clothing attributes recognition.}
  \label{fig:_retrieval_attribute_example}
\end{figure}

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{img/clothing_retrieval_interactiveSearch.png}
  \caption{An example of interactive fashion item retrieval~\cite{kovashka:cvpr2012}.}
  \label{fig:clothing_retrieval_interactiveSearch}
\end{figure}

In the clothing retrieval methods described above, the retrieval is only based on query images that reflect users' needs, without considering that users may want to provide extra keywords to describe the desired attributes that are absent in the query image. Towards this goal, Kovashka~\emph{et al.} developed the WhittleSearch~\cite{kovashka:cvpr2012} %, kovashka:ijcv2015}
that allows the user to upload a query image and provide additional relative attribute description as feedback for iteratively refining the image retrieval results (see Fig.~\ref{fig:clothing_retrieval_interactiveSearch}). Besides, for advancing the retrieval task with attribute manipulation, given a query image with attribute manipulation request, such as ``\textit{I want to buy a jacket %that looks 
like this query image, but with %blue color instead of pink and 
plush collar instead of round collar},'' the memory-augmented Attribute Manipulation Network (AMNet)~\cite{zhao:cvpr2017} updated the query representation encoding the unwanted attributes and replacing them to the desired ones. %The manipulated representation was then used to retrieve images with desired attributes from the gallery. 
Later, Ak~\emph{et al.}%~\cite{ak:wacv2018, ak:cvpr2018} explored the localization aspect of attribute representations to facilitate region-specific attribute manipulation requests. In particular, \cite{ak:wacv2018} estimated clothing item parts using an unsupervised segmentation method and applied CNN with part-based triplet ranking constraint as an attention mechanism.
~\cite{ak:cvpr2018} presented the FashionSearchNet to learn regions and region-specific attribute representations by exploiting the attribute activation maps %(AAMs)
generated by the global average pooling %(GAP)
layer. %In~\cite{laenen:wsdm2018}, Laenen~\emph{et al.} built a multimodal retrieval model that used a combination of an image and text as a query and ranked the image results based on their semantic similarity to the query text and their visual similarity to the query image. 
%, ak:wacv2018
Different from~\cite{zhao:cvpr2017, ak:cvpr2018} that %used neural networks to 
constructed visual representation of searched item by manipulating the visual representation of query image with the textual attributes in query text, \cite{laenen:wsdm2018} %used neural network to 
inferred the semantic relationship between visual and textual attributes in a joint multimodal embedding space. To help facilitate the reasoning of search results and user intent, Liao~\emph{et al.}~\cite{liao:mm2018} built EI (Exclusive and Independent) tree, that captured hierarchical structures of the fashion concepts%. The EI Tree 
, which was generated by incorporating product hierarchies of online shopping websites and domain knowledge of fashion experts. %The generated EI tree 
It was then applied to guide the end-to-end deep learning procedure, mapping the deep implicit features to explicit fashion concepts.

As the fashion industry attracts much attention %in recent years
recently, there comes a multimedia grand challenge ``AI meets beauty''~\footnote{\url{https://challenge2020.perfectcorp.com/}}, which aimed for competing for the top fashion item recognition methods, held in ACM Multimedia yearly from 2018. Perfect Corp.% , the leading beauty app developer, in collaborating with 
, CyberLink Corp., and National Chiao Tung University in Taiwan held this grand challenge and provided a large-scale image dataset %of over half a million images 
of beauty and personal care products, namely the Perfect-500K dataset~\cite{perfect500k}. Lin~\emph{et al.}~\cite{MMGC2019} received the top performance in the challenge %of ACM Multimedia2019
in 2019. They presented an unsupervised embedding learning to train a CNN model and combined the existing retrieval methods trained on different datasets to finetune the retrieval results.

%\footnote{\url{https://challenge2018.perfectcorp.com/}}

%----------Glasses Retrieval-------
%gu:icmr2015 -> glasses retrieval
%gu:sigir2016 -> glasses recommendation
%兩個都先不要，因為兩個感覺要一起講，但他跨retrieval跟recommendation
%Different problem is tackled in the fashion retrieval literature. Gu~\emph{et al.}~\cite{gu:icmr2015} presented a cross-scenario eyeglasses retrieval system, namely Fashion Glasses Search System (FGSS). They introduced a keypoint-based scheme called \textit{EyeGlass keYPoinT} (EGYPT) to describe the appearances of glasses, making FGSS free from segmentation problems. In the EGYPT, hybrid feature descriptors that combine shape, color, and texture features extracted from the detected keypoints are exploited to form a representative feature vector. Gu~\emph{et al.} later developed iGlasses~\cite{gu:sigir2016}, a recommendation for best-fits glasses that exploits the implicit matching rules between human faces and eyeglasses. Given a frontal face photo as the input, the iGlasses captures the correlation among the fine-grained attributes of human faces and frames of glasses, and then returns a ranked list of candidate eyeglasses. It further produces a synthesized image for the input face to demonstrate the visual effect when wearing the recommended glasses. 

%--------------------上面已經有retrieve bag的paper了，特別為非clothes開一個段落有點奇怪----------------------------
%The studies in~\cite{wang:icip2014, wang:tmm2016, wang:tmm2015} dealt with handbag recognition problems. In particular, Wang~\emph{et al.}~\cite{wang:icip2014} introduced a complementary feature obtained by extracting low-level features from a structure enhanced handbag image to compensate the missing details of the feature, called original feature, extracted directly from the original handbag image. The complementary feature is then fused with the original feature for the recognition. \cite{wang:tmm2016} further extended~\cite{wang:icip2014} by utilizing color model based on dominant color naming features. A CNN-based model for end-to-end framework to recognize the handbag models is presented in~\cite{wang:tmm2015}. It proposed feature selective joint classification regression CNN (FSCR-CNN) classification model, which consists of Feature Selective CNN and joint Classification-Regression CNN, to attenuate the illumination changes and inter-class similarity among handbags. The scores from FSCR-CNN classification model and CNN detection model are further eventually combined by a conditional probability model to recognize the handbag. 

%vittayakorn:wacv2015 -> from runway to realway (published in unknown rank conference but it has 76 citation; however, it works for matching the runway clothing image to the real-world clothing image (on human) -> it is not like runway to real store image, I can't find its value so ignore first 
%Other than fashion image retrieval studies mentioned above, Vittayakorn \emph{et al.}~\cite{vittayakorn:wacv2015} learned human based judgments of outfit similarity. They employed a linear SVM for pairwise comparison of clothing outfits based on a learned combination of features computed over parsed clothing regions. In \cite{semertzidis:tist2016}, Semertzidis~\emph{et al.} designed and evaluated a crowd-powered system for visual fashion similarity search based on user-defined criteria. Different kinds of crowds, ranges from click workers for tedious tasks, such as cleaning content, to mobile fashion crowds, are integrated for this purpose.

%\begin{figure}
%  \centering
%  \subfigure[Wang and Zhang~\cite{wang2011clothes}.]
%  {\includegraphics[width=1\linewidth]{img/clothing_retrieval_wangMM2011.png}}

%  \subfigure[Deep Search~\cite{huang:mm2014}.]
%  {\includegraphics[width=0.9\linewidth]{img/clothing_retrieval_huangMM2014.png}}
  
%  \subfigure[FashionSearchNet~\cite{ak:cvpr2018}.]
%  {\includegraphics[width=1\linewidth]{img/clothing_retrieval_akCVPR2018.png}}

%  \subfigure[EI Tree~\cite{liao:mm2018}.]
%  {\includegraphics[width=1\linewidth]{img/clothing_retrieval_liaoMM2018.png}}
  %\vspace{-2mm}
%  \caption{Pipelines of state-of-the-art clothing retrieval methods.}
%  \label{fig:clothing_retrieval_pipelines}
%\end{figure}

\subsubsection{Benchmark datasets}

The existing clothing retrieval studies mainly focused on a cross-domain scenario. Therefore, most of the benchmark datasets were collected from daily photos and online clothing shopping websites. Table~\ref{tab:clothing_retrieval_datasets} gives a summary and link of the download page (if publicly available) of the benchmark datasets.% used to evaluate the fashion retrieval studies.


\begin{table*}[t]
\renewcommand{\arraystretch}{1.1}
%\footnotesize
\notsotiny
    \centering
        \caption{Summary of the benchmark datasets for fashion retrieval task.}
        \vspace{-3mm}
    \begin{tabular}{l|c|c|c|l|c}
    \Xhline{1.0pt}
        \multicolumn{2}{c|}{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ photos\\ (videos)}  & \makecell{Key features} & Sources \\
    %\hline
    %    \multicolumn{2}{c|}{\makecell[l]{The Gallagher Collection\\ Person\tablefootnote{\url{http://chenlab.ece.cornell.edu/people/Andy/projectpage_clothing.html}}~\cite{gallagher:cvpr2008}}} & 2008 & 589 & \makecell[l]{Annotated 1008 faces with 32 identities} & \makecell[l]{N/A}\\ 
%    \hline
%        \multirow{2}{*}{\makecell[l]{Liu~\emph{et al.}\\\cite{liu2012street}}} & \makecell[l]{Online Shopping} & \multirow{2}{*}{2012} & 16,636 & \multirow{2}{*}{\makecell[l]{Each image consists of either upper- or lower-wear,\\ annotated with clothing-specific attributes}} & \makecell[l]{Online shopping sites}\\ 
%        \cline{2-2}\cline{4-4}\cline{6-6}
%        & \makecell[l]{Daily Photo} &  & 8,389 & & \makecell[l]{Flickr.com }\\ 
%    \hline
%        \multirow{2}{*}{\makecell[l]{Fu~\emph{et al.}\\\cite{fu:accv2012}}} & \makecell[l]{Online Shopping} & \multirow{2}{*}{2012} & $\sim$110,000 & \multirow{2}{*}{\makecell[l]{Each image consists of either upper- or lower-wear,\\ annotated with clothing-specific attributes}} & \makecell[l]{Amazon.com, eBay.com,\\ vancl.com, taobao.com}\\ 
%        \cline{2-2}\cline{4-4}\cline{6-6}
%        & \makecell[l]{Daily Photo} &  & \makecell{2,000} & & \makecell[l]{Flickr.com }\\ 
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{Women's Fashion Coat~\cite{WFC2013}}} & 2013 & 2,092 & \makecell[l]{Each image is labeled as one of 12 coat/jacket categories%:\\ blazer, cape, jean, military, motorcycle, parka, peacoat,\\ poncho, puffer, raincoat, trench, vest\\ Each category includes a minimum of 44 images} & \makecell[l]{eBay.com}\\
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{Fashion-focused Creative\\ Commons Social\tablefootnote{\url{http://skuld.cs.umass.edu/traces/mmsys/2013/fashion/}}~\cite{loni:mmsys2013}}} & 2013 & 4,810 & \makecell[l]{Annotated with 154 fashion-focused categories%(perform-\\ed by crowdsourcing workers and trusted annotators), user-pro-\\vided metadata, tags, favorites, comments, context, and note} & \makecell[l]{Flickr.com}\\ 
    %\hline
    %    \multicolumn{2}{c|}{\makecell[l]{Chi~\emph{et al.}~\cite{chi:mtap2016}}} & 2016 & 23,854  & \makecell[l]{Annotated with 5 categories} & \makecell[l]{Amazon.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{http://skuld.cs.umass.edu/traces/mmsys/2014/user05.tar}{Fashion 10000}%\tablefootnote{\url{http://skuld.cs.umass.edu/traces/mmsys/2014/user05.tar}}
        ~\cite{loni:mmsys2014}}} & 2014 &  32,398 & \makecell[l]{Annotated with 470 fashion categories%, associated meta-\\data, ground truth labels
        } & \makecell[l]{Flickr.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Deep Search~\cite{huang:mm2014}}} & 2014 & 206,235 & \makecell[l]{With template matching, 7 attributes and type are extract-\\ed from the descriptions, i.e. pattern, sleeve, button panel,\\ collar, style, and color } & \makecell[l]{Taobao.com,\\ Tsmall.com,\\ Amazon.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{DARN~\cite{huang2015cross}}} & 2015 & 545,373 & \makecell[l]{Online-offline upper-clothing image pair, annotated with\\ clothing attribute categories} & \makecell[l]{Online-shopping sites\\ and corresponding\\ customer review pages}\\ 
    \hline
        \multirow{2}{*}{\makecell[l]{\href{http://www.tamaraberg.com/street2shop}{Exact Street-}\\\href{http://www.tamaraberg.com/street2shop}{2Shop}%\tablefootnote{\url{http://www.tamaraberg.com/street2shop}}
        ~\cite{kiapour:iccv2015}}} & \makecell[l]{Street photos} & \multirow{2}{*}{2015} & \makecell{20,357} & \multirow{2}{*}{\makecell[l]{39,479 pairs of exactly matching items worn in street\\ photos and shown in shop photos}} & \makecell[l]{ModCloth.com}\\ 
    \cline{2-2}\cline{4-4}\cline{6-6}
         & \makecell[l]{Shop photos} & & 404,683 & & \makecell[l]{Online clothing retailers}\\ 
    \hline 
        \multicolumn{2}{c|}{\makecell[l]{\href{http://mvc-datasets.github.io/MVC/}{MVC}
        %\tablefootnote{\url{http://mvc-datasets.github.io/MVC/}}
        ~\cite{liu:icmr2016}}} & 2016 & 161,638 & Annotated with 264 attribute labels & \makecell[l]{Online shopping sites}\\
    \hline
        \multirow{2}{*}{\makecell[l]{Li~\emph{et al.}~\cite{li:icpr2016}}} & \makecell[l]{Product Clothing} & \multirow{2}{*}{2016} & 15,690 & \multirow{2}{*}{\makecell[l]{Annotated with clothing categories}} & \makecell[l]{Online shopping sites}\\ 
        \cline{2-2}\cline{4-4}\cline{6-6}
        & \makecell[l]{Daily Clothing} &  & \makecell{4,206} & & \makecell[l]{Flickr.com}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{http://mmlab.ie.cuhk.edu.hk/projects/DeepFashion/InShopRetrieval.html}{DeepFashion (In-shop Clothes}\\ \href{http://mmlab.ie.cuhk.edu.hk/projects/DeepFashion/InShopRetrieval.html}{Retrieval Benchmark)}%\tablefootnote{\url{http://mmlab.ie.cuhk.edu.hk/projects/DeepFashion/InShopRetrieval.html}}
        ~\cite{liu2016deepfashion}}} & 2016 & 52,712 & \makecell[l]{The resolution of images is 256$\times$256} & \makecell[l]{Online shopping sites\\ (Forever21 and Mogujie),\\ Google Images}\\
    \hline
        \multirow{2}{*}{\makecell[l]{Video2Shop\\\cite{ZQCheng2017CVPR}}} & \makecell[l]{Videos} & \multirow{2}{*}{2017} & \makecell{26,352\\(526)} & \multirow{2}{*}{\makecell[l]{39,479 exact matching pairs annotated with 14 categories\\ of clothes}} & \makecell[l]{Tmall MagicBox}\\ 
    \cline{2-2}\cline{4-4}\cline{6-6}
         & \makecell[l]{Online shopping} & & 85,677 & & \makecell[l]{Tmall.com, Taobao.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Dress like a star~\cite{garcia:iccvw2017}}} & 2017 & \makecell{7,000,000\\(40)} & \makecell[l]{It contains different movie genres such as animation, \\fantasy, adventure, comedy or drama} & \makecell[l]{YouTube.com}\\      
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{Shopping100k~\cite{ak:wacv2018}}} & 2018 & 101,021 & \makecell[l]{Annotated with 12 fashion attributes} & \makecell[l]{Online shopping sites}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Amazon~\cite{liao:mm2018}}} & 2018 & 489,000 & \makecell[l]{Annotated with 200 clothing categories} & \makecell[l]{Amazon.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Perfect-500K~\cite{perfect500k}}} & 2018 & 500,000 & \makecell[l]{It is vast in scale, rich and diverse in content in order to\\ collect as many as possible beauty and personal care items} & \makecell[l]{e-commerce websites}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://github.com/switchablenorms/DeepFashion2}{DeepFashion2}%\tablefootnote{\url{https://github.com/switchablenorms/DeepFashion2}}
        ~\cite{DeepFashion2}}} & 2019 & 491,000 & \makecell[l]{a  versatile benchmark of four tasks including clothes\\ detection, pose estimation, segmentation, and  retrieval} & \makecell[l]{ DeepFashion~\cite{liu2016deepfashion},\\ Online shopping websites}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{FindFashion~\cite{FashionRV2019}}} & 2019 & 565,041 & \makecell[l]{Merge two existing datasets, Street2Shop and Deep-\\Fashion, and label three attributes of the most affected} & \makecell[l]{Street2Shop~\cite{kiapour:iccv2015},\\DeepFashion~\cite{liu2016deepfashion}}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://github.com/Maryeon/asen}{Ma~\emph{et al.}}%\tablefootnote{\url{https://github.com/Maryeon/asen}}
        ~\cite{ma2020aaai}}} & 2020 & 180,000 & \makecell[l]{Since dataset for attribute-specific fashion retrieval is\\ lacking, this dataset rebuild three fashion dataset with\\ attribute annotations} & \makecell[l]{DARN~\cite{huang2015cross},\\FashionAI~\cite{Zou2019cvprw},\\DeepFashion~\cite{liu2016deepfashion}}\\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:clothing_retrieval_datasets}
    %\begin{tablenotes}
    %  \scriptsize
      %\item N/A: there is no reported information to cite.
    %\end{tablenotes}
\end{table*}


\subsubsection{Performance evaluations}
\label{sec:item_retrieval_PE}
%(2) , sanchez-riera:mmm2017
%(3), sanchez-riera:mmm2017
There are some evaluation metrics used to assess the performance of clothing retrieval methods. The different evaluation metrics used are as follows: (1) %\cite{fu:accv2012, liu2012street, huang2015cross, kiapour:iccv2015, wang:icmr2016, ZQCheng2017CVPR, jiang:mm2016, XLiang2016TMM, liao:mm2018, huang:mm2014, zhao:cvpr2017, ak:wacv2018, ak:cvpr2018, liu:icmr2016, jiang:tomm2018, FashionRV2019} use 
Top-\textit{k} retrieval accuracy, the ratio of queries with at least one matching item retrieved within the top-\textit{k} returned results, %This metric is used in \cite{fu:accv2012, liu2012street, huang2015cross, kiapour:iccv2015, wang:icmr2016, ZQCheng2017CVPR, jiang:mm2016, XLiang2016TMM, liao:mm2018, huang:mm2014, zhao:cvpr2017, ak:wacv2018, ak:cvpr2018, liu:icmr2016, jiang:tomm2018, FashionRV2019}. 
(2) %\cite{wang2011clothes, liu2012street, fu:accv2012, kalantidis:icmr2013, li:icpr2016, laenen:wsdm2018} apply 
Precision@\textit{k}, the ratio of items in the top-\textit{k} returned results that are matched with the queries, %This metric is used in \cite{wang2011clothes, liu2012street, fu:accv2012, kalantidis:icmr2013, li:icpr2016, laenen:wsdm2018}. 
(3) %\cite{wang2011clothes} employs 
Recall@\textit{k}, the ratio of matching items that are covered in the top-\textit{k} returned results, %This metric is used in \cite{wang2011clothes}. 
(4) %\cite{huang2015cross, zhao:cvpr2017} utilize 
Normalized Discounted Cumulative Gain (NDCG@\textit{k}), the relative orders among matching and non-matching items within the top-\textit{k} returned results, and %This metric is used in \cite{huang2015cross, zhao:cvpr2017}. 
(5) Mean Average Precision (MAP), which measures the precision of returned results at every position in the ranked sequence of returned results across all queries. %This metric evaluates the ranking performance of \cite{laenen:wsdm2018, MMGC2019}. 


%It is defined as
%\begin{equation}
%NDCG@k = \frac{1}{N}\sum_{i}^k \frac{2^{r(i)}-1}{log(i+1)},
%\label{equ:ndcg_at_k}
%\end{equation}
%the proportion of relevant documents in the top k positions.
%where $r(i)$ is the ground truth relevance indicated the matched attributes between the query image and the $i$-th ranked image, $N$ is a constant for normalization. 

%(6) The area under the precision recall curve (AUC), which is used to evaluate the model performance of \cite{vittayakorn:wacv2015}.(7) The ultimate percentile rank assigned to the query image, which measures the ratio of database images ranked below the matched items. (8) The correlation between the full ranking, which is computed by the method's relevance scoring function and a ground truth ranking. Both evaluation metrics (7) and (8) are used in \cite{kovashka:cvpr2012, kovashka:ijcv2015}.

Table 2 of the Supplementary Material presents the performance comparisons of some retrieval methods reviewed in this survey. We are unable to give comparisons for all different retrieval methods because the benchmarks they used are not consistent.

\begin{comment}
\begin{table}[t!]
\footnotesize
    \centering
        \caption{Performance comparisons of some clothing retrieval methods by different evaluation protocols.}
        \vspace{-3mm}
    \begin{tabular}{c|c|c|c|c}
    \Xhline{1.0pt}
        \makecell{Protocol} & \makecell{Evaluation metric} & \makecell{Dataset} & \makecell{Method} & \makecell{Result}\\
    \hline
        \makecell{\cite{ZQCheng2017CVPR}} & \makecell{Top-20 accuracy} & \makecell{Video2Shop} & \makecell{Kiapour~\emph{et al.}~\cite{kiapour:iccv2015} / Wang~\emph{et al.}~\cite{wang:icmr2016} / AsymNet~\cite{ZQCheng2017CVPR}} & \makecell{23.47 / 28.73 / \textbf{36.63}}\\
    \hline
        \makecell{\cite{jiang:mm2016}} & \makecell{Top-20 accuracy} & \makecell{Exact Street2Shop} & \makecell{Jiang~\emph{et al.}~\cite{jiang:mm2016} / Kiapour~\emph{et al.}~\cite{kiapour:iccv2015}} & \makecell{20.35 / \textbf{30.59}}\\
    \hline
        \multirow{2}{*}{\makecell[l]{\cite{ak:cvpr2018}}} & \multirow{2}{*}{\makecell{Top-30 accuracy}} & \makecell{Deep Fashion} & \makecell{AMNet~\cite{zhao:cvpr2017} / FashionSearchNet~\cite{ak:cvpr2018}} & \makecell{24.60 / \textbf{37.60}} \\
    \cline{3-5}
         &  & \makecell{Shopping 100k} & \makecell{AMNet~\cite{zhao:cvpr2017} / FashionSearchNet~\cite{ak:cvpr2018}} & \makecell {40.60 / \textbf{56.60}} \\


    \hline
        \multirow{2}{*}{\makecell[l]{\cite{liao:mm2018}}} & \multirow{2}{*}{\makecell{Recall@20}} & \makecell{Amazon} & \makecell{AMNet~\cite{zhao:cvpr2017} / EI Tree~\cite{liao:mm2018}} & \makecell{31.20 / \textbf{63.60}} \\
    \cline{3-5}
         &  & \makecell{DARN} & \makecell{AMNet~\cite{zhao:cvpr2017} / EI Tree~\cite{liao:mm2018}} & \makecell {60.50 / \textbf{71.40}} \\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:clothing_retrieval_results}
    \begin{tablenotes}
      \scriptsize
      \item The best results are highlighted in bold font.
    \end{tablenotes}
\end{table}
\end{comment}

%\begin{table}[htbp]
%\footnotesize
%    \centering
%        \caption{Performance comparisons of some clothing retrieval methods.}
%        \vspace{-3mm}
%    \begin{tabular}{c|c|c|c|c}
%    \Xhline{1.0pt}
%        \makecell{Evaluation protocol} & \makecell{Evaluation metric} & \makecell{Dataset} & \makecell{Method} & \makecell{Result}\\
%    \hline
%        \multirow{3}{*}{\makecell[l]{\cite{ZQCheng2017CVPR}}} & \multirow{3}{*}{\makecell{Top-20 accuracy}} & \multirow{3}{*}{\makecell[l]{Video2Shop}} & %\makecell[l]{Deep Search~\cite{huang:mm2014}} & 21.44 \\ 
%    \cline{4-5}
%        &  &  & 
%        \makecell[l]{Kiapour~\emph{et al.}~\cite{kiapour:iccv2015}} & 23.47 \\ 
%    \cline{4-5}
%        &  &  & \makecell[l]{Wang~\emph{et al.}~\cite{wang:icmr2016}} & 28.73 \\
%    \cline{4-5}
%        &  &  & \makecell[l]{AsymNet~\cite{ZQCheng2017CVPR}} & \textbf{36.63} \\
%    \hline\hline
%        \multirow{2}{*}{\makecell[l]{\cite{jiang:mm2016}}} & \multirow{2}{*}{\makecell{Top-20 accuracy}} & \multirow{2}{*}{\makecell[l]{Exact Street2Shop}}  & \makecell[l]{Jiang~\emph{et al.}~\cite{jiang:mm2016}} & 20.35 \\
%    \cline{4-5}
%         &  &  & \makecell[l]{Kiapour~\emph{et al.}~\cite{kiapour:iccv2015}} & \textbf{30.59} \\
%    \hline\hline
%        \multirow{4}{*}{\makecell[l]{\cite{ak:cvpr2018}}} & \multirow{4}{*}{\makecell{Top-30 accuracy}} & \multirow{2}{*}{\makecell[l]{Deep Fashion}}  & \makecell[l]{AMNet~\cite{zhao:cvpr2017}} & 24.60 \\
%    \cline{4-5}
%         &  &  & \makecell[l]{FashionSearchNet~\cite{ak:cvpr2018}} & \textbf{37.60} \\
%    \cline{3-5}
%         &  & \multirow{2}{*}{\makecell[l]{Shopping 100k}} & \makecell[l]{AMNet~\cite{zhao:cvpr2017}} & 40.60 \\
%    \cline{4-5}
%         &  &  & \makecell[l]{FashionSearchNet~\cite{ak:cvpr2018}} & \textbf{56.60} \\
%    \hline\hline
%        \multirow{4}{*}{\makecell[l]{\cite{liao:mm2018}}} & \multirow{4}{*}{Recall@20} & \multirow{2}{*}{\makecell[l]{Amazon}}  & \makecell[l]{AMNet~\cite{zhao:cvpr2017}} & 31.20 \\
%    \cline{4-5}
%         &  &  & \makecell[l]{EI Tree~\cite{liao:mm2018}} & \textbf{63.60} \\
%    \cline{3-5}
%         &  & \multirow{2}{*}{\makecell[l]{DARN}} & \makecell[l]{AMNet~\cite{zhao:cvpr2017}} & 60.50 \\
%    \cline{4-5}
%         &  &  & \makecell[l]{EI Tree~\cite{liao:mm2018}} & \textbf{71.40} \\
%    \Xhline{1.0pt}
%    \end{tabular}
%    \label{tab:clothing_retrieval_results}
%    \begin{tablenotes}
%      \scriptsize
%      \item The best results are highlighted in bold font.
%    \end{tablenotes}
%\end{table}

%However, we are unable to give comparisons for all different retrieval methods due to the inconsistent benchmarks.

%--++--++

==> ACMCSUR – Fashion/src/fffashion_recommendation.tex <==
\section{Fashion Recommendation}
\label{sec:fffashion_recommendation}

%Being well dressed and knowing how to dress well is extremely important. Dressing well will make everyone look and feel confident and energetic. What is more, Tom Ford, a fashion expert and a film director, once even said, ``Dressing well is a form of good manners.'' 
\textit{``Dressing well is a form of good manners.''} --- Tom Ford \textit{(1961-)}% However,
, while not everyone is a natural-born fashion stylist. In support of this need, fashion recommendation has attracted increasing attention, given its ready applications to online shopping for fashion products. Relevant literature on the research progress of fashion recommendation falls into three main tasks: fashion compatibility, outfit matching, and hairstyle suggestion.
%there have been several attempts to develop intelligent fashion style recommendations, with focused on classifying styles according to occasion, location, body shape, or social circle.

%four main categories, \textit{i.e.}, outfit matching, fashion item retrieval, style classification, and hairstyle suggestion.


\subsection{Fashion Compatibility}
Fashion recommendation works based on fashion compatibility, which performs how well items of different types can collaborate to form fashionable outfits. Also, it is worth mentioning that the main difference between fashion item retrieval (Sec.~\ref{subsec:item_retrieval}) and fashion recommendation (Sec.~\ref{sec:fffashion_recommendation}) is that the former learns the visual similarity between the same clothing type. In contrast, the latter learns both visual similarity and visual compatibility between different clothing types.

\subsubsection{State-of-the-art methods} 

%For answering the questions like ''What outfit goes well with this pair of shoes?'' Veit~\emph{et al.}~\cite{veit:iccv2015} utilized the co-purchase data from Amazon.com to train a Siamese Convolutional Neural Network (CNN) to learn style compatibility across categories. 
Veit~\emph{et al.} introduced Conditional Similarity Networks (CSNs) \cite{AVeit2017CVPR}, which learned non-linear feature embeddings that incorporated various notions of similarity within a shared embedding using a shared feature extractor. The CSNs addressed the issue of a standard triplet embedding that treated all triplets equally and ignored the sources of similarity. Song~\emph{et al.}~\cite{song2017neurostylist} integrated visual and contextual modalities of fashion items by employing the autoencoder neural model to seek the non-linear latent compatibility space. Following ~\cite{song2017neurostylist}, Song~\emph{et al.}~\cite{song:sigir2018} integrated fashion domain knowledge to the neural networks to boost the %compatibility modeling 
performance. Vasileva~\emph{et al.}~\cite{vasileva:eccv2018} presented %an approach 
to learn an image embedding that respected item type. They first learned a single, shared embedding space to measure item similarity, then projected from that shared embedding to subspaces identified by type. For learning the compatibility between clothing styles and body shapes, Hidayati~\emph{et al.}~\cite{hidayati:mm2018,hidatayi2020tmm} exploited human body measurements and images of stylish celebrities. They presented a body shape calculator to determine the type of body shape based on a set of body measurements, and a style propagation mechanism to model the correlation between body shapes and clothing styles by constructing graphs of images based on the body shape information and the visual appearance of clothing items, respectively. For using category complementary relations to model compatibility, Yang~\emph{et al.}~\cite{Yang2018aaai} proposed a translation-based neural fashion compatibility model which contained three parts: (1) first mapped each item into a latent space via two CNN for visual and textual modality, (2) encoded the category complementary relations into the latent space, and (3) minimized a margin-based ranking criterion to optimize both item embeddings and relation vectors jointly. 

For making the fashion compatibility task more user-friendly, Wang~\emph{et al.}~\cite{wang2019acmmm} introduced a diagonal process for giving information about which item made the outfit incompatible. They presented an end-to-end multi-layered comparison network to predict the compatibility between different items at different layers and use the backpropagation gradient for diagnosis. Hsiao~\emph{et al.}~\cite{hsiao2019fashionplus} proposed Fashion++ to make minimal adjustments to a full-body clothing outfit that have a maximal impact on its fashionability. Besides, Song~\emph{et al.}~\cite{Song2019GPBPR} took user preferences into account to present a personalized compatibility modeling scheme GP-BPR. It utilized two components, general compatibility modeling and personal preference modeling, for evaluating the item-item and user-item interactions, respectively.

\subsubsection{Benchmark datasets}
The most used source for fashion compatibility datasets is the Polyvore fashion website. It is an online shopping website, where the fashion items contain rich annotations, e.g., clothing color, text description, and multi-view outfit images. We list the benchmark datasets for fashion compatibility in Table~\ref{tab:fashion_compatibility_datasets}. 

\begin{table*}[htbp]
\scriptsize
    \centering
        \caption{Summary of the benchmark datasets for fashion compatibility task.}
        \vspace{-3mm}
    \begin{tabular}{c|c|c|c|c|c|c}
    \Xhline{1.0pt}
      \multicolumn{2}{c|}{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ outfits} & \makecell{\# of item\\ categories} & Key features & Sources \\
    \hline 
        \multicolumn{2}{c|}{\makecell[l]{FashionVC~\cite{song2017neurostylist}}} & 2017 & 20,726 & 2 & \makecell[l]{Annotated with title, category, and description} & \makecell[l]{Polyvore.com} \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{\href{https://github.com/mvasil/fashion-compatibility}{Vasileva~\emph{et al.}}%\tablefootnote{\url{https://github.com/mvasil/fashion-compatibility}}
        ~\cite{vasileva:eccv2018}}} & 2018 & 68,306 & 19 & \makecell[l]{Annotated with outfit and item ID, fine-grained\\ item type, title, and text descriptions} & \makecell[l]{Polyvore.com} \\
    \hline
        \multirow{6}{*}{\makecell[l]{\href{http://bit.ly/Style4BodyShape}{Style}\\ \href{http://bit.ly/Style4BodyShape}{for} \\\href{http://bit.ly/Style4BodyShape}{Body}\\\href{http://bit.ly/Style4BodyShape}{Shape}%\tablefootnote{\url{ http://bit.ly/Style4BodyShape}}
        \\\cite{hidayati:mm2018}}} & \makecell[l]{Stylish Celeb-\\rity Names} & \multirow{6}{*}{2018} & \multirow{3}{*}{N/A} & \multirow{6}{*}{N/A} & \makecell[l]{270 names of the top stylish female celebrities} & \makecell[l]{Ranker.com,\\ fashion magazine sites}\\
    \cline{2-2}\cline{6-7}
         & \makecell[l]{Body\\Measurements} &  &  & & \makecell[l]{Body measurements of 3,150 female celebrities} & \makecell[l]{Bodymeasurements.org}\\
    \cline{2-2}\cline{4-4}\cline{6-7}
         & \makecell[l]{Stylish Celeb-\\rity Images} &  & 347,948 & & \makecell[l]{Annotated with clothing categories and celebrity\\ names} & \makecell[l]{Google Image Search}\\
    \hline
        % # of item 83,691
        \multicolumn{2}{c|}{\makecell[l]{\href{https://github.com/WangXin93/fashion_compatibility_mcn}{PolyVore-T}%\tablefootnote{\url{https://github.com/WangXin93/fashion_compatibility_mcn}}
        ~\cite{wang2019acmmm}}} & 2019 & 19,835 & 5 & \makecell[l]{Categories includes top, bottom, shoes, bag,\\ and accessory} & \makecell[l]{Dataset collected by\\ \cite{han2017learning} from Polyvore} \\
        
    \hline
        % # of item 672,335
        \multicolumn{2}{c|}{\makecell[l]{IQON3000~\cite{Song2019GPBPR}}} & 2019 & 308,747 & 6 & \makecell[l]{Categories contains top, bottom, shoes, accesso-\\ry, dress and tunic, and coat. The outfits within\\ this dataset was created by 3,568 users} & \makecell[l]{The fashion web\\ service IQON} \\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:fashion_compatibility_datasets}
    \begin{tablenotes}
      \scriptsize
      \item N/A: there is no reported information to cite.
    \end{tablenotes}
\end{table*}

\subsubsection{Performance evaluations}
\label{sec:fashion_compatibility_PE}
For measuring the performance of fashion compatibility works, area under the receiver operating characteristic curve (AUC) is the most used metric. AUC measures the probability that the evaluated work would recommend higher compatibility for positive set than negative set. The AUC scores range between 0 and 1.
%In~\cite{hidayati:mm2018}, in addition to the subjective ratings of user satisfaction, the mean Average Precision (mAP) was computed to measure the overall ranks.

%\subsection{Clothing Recommendation}
\subsection{Outfit Matching}
Each outfit generally involves multiple complementary items, such as tops, bottoms, shoes, and accessories. A key to a stylish outfit lies in the matching fashion items, as illustrated in Fig.~\ref{fig:outfit_matching_example}. However, generating harmonious fashion matching is challenging due to three main reasons. First, %a 
the fashion concept is %often 
subtle and subjective. Second, there are a large number of attributes for describing fashion. Third, the notion of fashion item compatibility generally goes across categories and involves complex %many-to-many 
relationships. In the past several years, this problem has attracted a great deal of interest, resulting in a long list of algorithms and techniques. %In the following, we review the current state-of-the-art of recommendation method for outfit matching.


\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{img/outfit_matching_hsiaoCVPR2018.png}
  \caption{Examples of outfit matching task~\cite{hsiao2018creating}.}
  \label{fig:outfit_matching_example}
\end{figure}


\subsubsection{State-of-the-art methods}

%move from the item retrieval part
%-------chi:mtap2016-------
%Chi~\emph{et al.} introduced Visual Part-based Object Representation (VPOR) framework~\cite{chi:mtap2016} that use partial visual appearances to obtain personalized item recommendation results. Conceptually, the VPOR decomposes every item image into a set of disjoint part, with each part represents a meaningful semantic part, then discovers auxiliary features through part-based feature propagation mechanism. The feature propagation can make two items that share a similar part but are different in the rest parts become more similar for improving the relevance of recommended results.
%-------sanchez-riera:mmm2017-------


%-------------------from fashion modeling (popularity prediction)----------------------
%fan:neurocomp2016 -> manipulate the face shape (to get thinner face)
%liang:tcsvt2017 -> like facial makeup recommendation
%The studies in~\cite{fan:neurocomp2016, liang:tcsvt2017} modeled facial attractiveness under mobile computing settings, which required efficient processing. Fan~\emph{et al.}~\cite{fan:neurocomp2016} developed a mesh-based face beautifier with focused on local chin shape. They leveraged Laplacian as the constraint to remap the original chin shape to the target, then applied a triangular mesh based warping algorithm to generate a beautified face image. An averaged chin shape is used as the attractive template. Liang~\emph{et al.}~\cite{liang:tcsvt2017} proposed a mask generation method based on the edge-aware label propagation model. It adjusts the facial lighting, detail, and color adaptively by the facial masks in the corresponding facial layers, while preserves the background unchanged.


Fashion recommendation for outfit matching was initially introduced by Iwata~\emph{et al.}~\cite{iwata:ijcai2011}. They proposed a probabilistic topic model for learning information about fashion coordinates. Liu~\emph{et al.}~\cite{liu:mm2012} explored occasion-oriented clothing recommendation by considering the \textit{wearing properly} and \textit{wearing aesthetically} principles. They adopted a unified latent Support Vector Machine (SVM) to learn the recommendation model that incorporates clothing matching rules among visual features, attributes, and occasions. A similar idea of location-oriented recommendation system was proposed by Zhang~\emph{et al.}~\cite{zhang:tmm2017}%which was different from~\cite{liu:mm2012} that constrained the aesthetic matching rule to the clothing items only, 
. They considered the visual match between the foreground clothing and the background scenery %. To this aim, they 
and proposed a hybrid multi-label convolutional neural network combined with the %support vector machine 
SVM (mCNN-SVM), which captured the uneven distribution of clothing attributes and explicitly formulated the correlations between clothing attributes and location attributes. More recently, Kang~\emph{et al.}~\cite{kang:cvpr2019} introduced ``Complete the Look'' %task 
aiming at recommending fashion items that %complement (or \textit{
go well with %}) 
the given scene. %To achieve this task, 
They measured both global compatibility (\textit{i.e.}, the compatibility between the scene and product images) and local compatibility (\textit{i.e.}, the compatibility between every scene patch and product image) via Siamese networks and category-guided attention mechanisms. The comparison of the  %use-cases of 
product-based and the %``complete the look'' 
scene-based complementary recommendation is shown in Fig.~\ref{fig:outfit_matching_completeTheLook}. 

%Inspired by the advances of deep learning technique, most of the current researchers have put efforts in modeling the style compatibility based on the data-driven deep learning approaches. 
A line with metric-based works then proposed to model item-to-item compatibility based on co-purchase behavior. Veit~\emph{et al.}~\cite{veit:iccv2015} utilized the co-purchase data from Amazon.com to train a Siamese %Convolutional Neural Network (
CNN %)
to learn style compatibility across categories and used a robust nearest neighbor retrieval to generate compatible items. The study in~\cite{mcauley:sigir2015} modeled human preference to uncover the relationships between the appearances of pairs of items by Low-rank Mahalanobis Transform that mapped compatible items to embeddings close in the latent space. He and McAuley~\cite{he:aaai2016} later extended the work of~\cite{mcauley:sigir2015} by combining visual and historical user feedback data. The proposed study incorporated visual signals into Bayesian Personalized Ranking with Matrix Factorization as the underlying predictor. 
%The metric-based works~\cite{veit:iccv2015, mcauley:sigir2015, he:aaai2016} aimed to model item-to-item recommendation based on co-purchasing behaviour; 
%Furthermore, \cite{he:icdm2016} proposed to relax the identity and symmetry assumptions inherent in metric-based recommendation methods. The \textit{Mixtures of Non-Metric Embeddings for Recommendation} framework allows \cite{he:icdm2016} to learn multiple notions of relatedness to compete and interact. 
Besides, %in~\cite{hu:mm2015}, 
Hu~\emph{et al.}~\cite{hu:mm2015} addressed the personalized issue by utilizing a functional tensor factorization method to model the user-item and item-item interactions. 

%In particular, previous studies mainly focus on visual information but fail to consider the contextual factors. To bridge this gap, Song~\emph{et al.}~\cite{song2017neurostylist} integrated visual and contextual modalities of fashion items by employing the autoencoder neural model to seek the non-linear latent compatibility space. Following this work,~\cite{song:sigir2018} integrated fashion domain knowledge to the neural networks to boost the compatibility modeling performance. 

%Most previous works~\cite{iwata:ijcai2011, liu:mm2012, song:sigir2018} 
Most previous works mainly focused on top-bottom matching. However, an outfit generally includes more items, such as shoes and bags%, \emph{etc}
. To address this issue, Chen and He~\cite{chen2018dress} extended the traditional triplet neural network, which usually receives three instances, to accept multiple instances. A mixed-category metric learning method was proposed to adapt the multiple inputs. A similar idea was also employed in~\cite{shih2018compatibility}, where the %metric learning was combined with generative neural networks. The 
proposed generator, referred to as metric-regularized cGAN, was regularized by a projected compatibility distance %(PCD) 
function. It ensured the compatible items were closer in the learned space compared to the incompatible ones.

%Conditional Generative Adversarial Network (MrCGAN)

%\textcolor{red}{Given the image of a query item, the well-trained MrCGAN is able to generate an image of a compatible item.}


As for methods with the end-to-end framework, Li \emph{et al.}~\cite{YLi2017TMM} formulated the problem as a classification task, where a given outfit composition was labeled as a popular or unpopular one. They designed a multi-modal multi-instance model, that exploited images and meta-data of fashion items, and information across fashion items, to evaluate instance aesthetics and set compatibility simultaneously. %In~\cite{han2017learning}, an end-to-end model was built based on bidirectional LSTM (Bi-LSTM). Specifically, inspired by image captioning of~\cite{donahue2015long}, Han~\emph{et al.} treated an outfit as a sequence of fashion items and each item in the outfit as a time step.
Inspired by image captioning of~\cite{donahue2015long}, Han~\emph{et al.}~\cite{han2017learning} built a model based on bidirectional LSTM (Bi-LSTM) to treat an outfit as a sequence of fashion items and each item in the outfit as a time step. A Bi-LSTM model was then utilized to predict the next item conditioned on previously seen ones, where the objective was to maximize the total probability of the given positive sequence. The model was able to achieve three tasks, \emph{i.e.}, fill-in-the-blank (fashion item recommendation given an existing set), outfit generation conditioned on users' text/image inputs, and outfit compatibility prediction. Another work~\cite{hsiao2018creating} also borrowed the idea from natural language processing, which meant that an outfit was regarded as a ``document'', an inferred clothing attribute was taken to be a ``word'', and a clothing style was referred to the ``topic''. The problem of outfit matching was formulated with the topic model. The combinations similar to previously assembled outfits should have a higher probability, which can be employed as the prediction for compatibility, and then solve the outfit matching problem.

For building the bridge between fashion compatibility and personalized preference in outfit matching tasks, there are a few methods for this goal. %~\cite{sanchez-riera:mmm2017, Yu2019ICCV, dong2019acmmm, chen2019kdd, Hou2019ijcai}. 
A personalized clothing recommendation system, namely i-Stylist that retrieved clothing items through the analysis of user's images, was developed in \cite{sanchez-riera:mmm2017}. The i-Stylist organized the deep learning features and clothing properties of user's clothing items as a fully connected graph. The user's personalized graph model later derived the probability distribution of the likability of an item in shopping websites. Dong~\emph{et al.}~\cite{dong2019acmmm} took user preference and body shape into account for measuring the user-garment compatibility to deal with personalized capsule wardrobe creation task. They introduced an optimization-based  %personalized capsule wardrobe creation 
framework with dual compatibility modeling, which can both evaluate the garment-garment compatibility and user-garment compatibility. Besides, Yu~\emph{et al.}~\cite{Yu2019ICCV} worked for synthesizing new items automatically for recommendation. Given a query item, the personalized fashion design network they proposed would generate a fashion item for the specific user based on fashion compatibility and user preference. Furthermore, Chen~\emph{et al.}~\cite{chen2019kdd} presented an industrial-scale Personalized Outfit Generation (POG) model. % for personalized fashion recommendation. 
They deployed POG on platform \textit{Dida} in \textit{Alibaba} to recommend personalized fashionable outfits for users. For providing more concrete recommendation for users, Hou~\emph{et al.}~\cite{Hou2019ijcai} proposed a semantic attribute explainable recommender system to not only recommend for personalized compatible items but also explain the reason why the system recommends it.



\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{img/recommendation_comparison.png}
  \caption{A comparison between product-based and scene-based complementary recommendation~\cite{kang:cvpr2019}.}
  \label{fig:outfit_matching_completeTheLook}
\end{figure}



%a popular fashion website, where users create and upload outfit data as shown in Figure 3.

\subsubsection{Benchmark datasets}

Since different papers are under various settings and most of the datasets for outfit matching are not publicly available, almost every %paper for outfit  matching
work collected their own dataset. %The datasets were collected  from social media platforms where users can create their own outfits, such as Polyvore.com. 
We list the benchmark datasets for outfit matching in Table~\ref{tab:outfit_matching_datasets}. Note that the outfit database in~\cite{mcauley:sigir2015, he:aaai2016, hu:mm2015, YLi2017TMM, han2017learning, hsiao2018creating, kang:cvpr2019} 
%vasileva:eccv2018
comprises the images of each single item, while in~\cite{iwata:ijcai2011, liu:mm2012, chen2018dress} consists of an outfit in a single image.


\begin{table*}[t!]
\scriptsize
    \centering
        \caption{Summary of the benchmark datasets for outfit matching task.}
        \vspace{-3mm}
    \begin{tabular}{c|c|c|c|c|c}
    \Xhline{1.0pt}
      \makecell{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ outfits} & \makecell{\# of item\\categories} & Key features & Sources \\
%     \hline
%        \makecell[l]{Iwata~\emph{et al.}~\cite{iwata:ijcai2011}} & 2011 & 14,813 & 5 &   \makecell[l]{Full-body fashion model} & \makecell[l]{Magazine,\\ Chicisimo.com,\\ Weardrobe.ie}\\ %clothes, bags, shoes, cosmetics, accessories
    \hline
        \makecell[l]{What-to-Wear\\\cite{liu:mm2012}} & 2012 & 24,417 & 2 &  \makecell[l]{Occasion-oriented work; Annotated with full-body,\\ upper-body, or lower-body} & \makecell[l]{Online shopping\\ photo sharing sites}\\
    %\hline
    %    \multirow{3}{*}{\makecell[l]{What-to-Wear\\ (WoW)~\cite{liu:mm2012}}} & \makecell[l]{WOW\_Full} & \multirow{3}{*}{2012} & 9,469 & \multirow{3}{*}{\makecell{Occasion}} & \multirow{3}{*}{\makecell[l]{Annotated with 7 multi-value clothing attributes\\and 10 occasion categories via Amazon Mechan-\\ical Turk}} & \multirow{3}{*}{\makecell[l]{Online shopping \\sites, photo sharing\\ sites}} \\
    %\cline{2-2}\cline{4-4}
    %    & \makecell[l]{WoW\_Upper} & & 8,421 & & & \\
    %\cline{2-2}\cline{4-4}
    %    & \makecell[l]{WoW\_Lower} & & 6,527 & & & \\
    \hline
        \makecell[l]{Styles and\\Substitutes \cite{mcauley:sigir2015}} & 2015 & 773,465 & N/A & \makecell[l]{Annotated with 4 categories of relationship: (1) users\\ who viewed X also viewed Y, (2) users who viewed\\ X eventually bought Y, (3) users who bought X also\\ bought Y, (4) users bought X and Y simultaneously} & \makecell[l]{Amazon.com}\\
    \hline
        \makecell[l]{Hu~\emph{et al.}~\cite{hu:mm2015}} & 2015 & 28,417 & 3 & \makecell[l]{Annotated with categories, names, and descriptions} & \makecell[l]{Polyvore.com}\\
    \hline
        \makecell[l]{He~\emph{et al.}~\cite{he:aaai2016}} & 2016 & 598.353 & N/A & \makecell[l]{Annotated with users' review histories} & \makecell[l]{Amazon.com,\\ Tradesy.com}\\
    \hline
        {\makecell[l]{Journey Outfit\\\cite{zhang:tmm2017}}} & 2017 & 3,392 & N/A & \makecell[l]{Location-oriented work; Annotated with 14 travel\\ destinations} & \makecell[l]{Online travel\\ review sites}\\
    \hline
        \makecell[l]{Li~\emph{et al.}~\cite{YLi2017TMM}} & 2017 & 195,262 & 4 & \makecell[l]{Annotated with\ title, category, and number of likes} & \makecell[l]{Polyvore.com} \\
    \hline 
        \makecell[l]{Han~\emph{et al.}~\cite{han2017learning}} & 2017 & 21,889 & 8 & \makecell[l]{Each item contains a pair -- product image and a corre\\sponding text description} & \makecell[l]{Polyvore.com} \\
    \hline
        \makecell[l]{Hsiao~\emph{et al.}~\cite{hsiao2018creating}} & 2018 & 3,759 & $\geq 2$ & \makecell[l]{Annotated with meta-labels, \emph{e.g.}, season (winter, spring,\\ summer, fall), occasion (work, vacation), and function\\ (date, hike)} & \makecell[l]{Polyvore.com} \\
    \hline
        \makecell[l]{Fashion\\ Collocation\cite{chen2018dress}} & 2018 & 220,000 & 5 & \makecell[l]{Annotated with independent and ready for wearing (off-\\body module) or dependent (on-body module), or a \\bounding box} & \makecell[l]{Chictopia.com,\\ Wear.net,\\ FashionBeans.com} \\
    \hline
        \makecell[l]{\href{https://github.com/kang205/STL-Dataset}{Pinterest's Shop}\\\href{https://github.com/kang205/STL-Dataset}{The Look}%\tablefootnote{\url{https://github.com/kang205/STL-Dataset}}
        ~\cite{kang:cvpr2019}} & 2019 & 38,111 & 10 & \makecell[l]{Annotated with categories of shoes, tops, pants, hand-\\bags, coats, sunglasses, shorts, skirts, earrings, necklaces} & \makecell[l]{Pinterest.com}\\
    \hline
        \makecell[l]{\href{https://anonymousresearch.wixsite.com/pcw-dc}{bodyFashion}%\tablefootnote{\url{https://anonymousresearch.wixsite.com/pcw-dc}}
        ~\cite{dong2019acmmm}} & 2019 & 75,695 & N/A & \makecell[l]{It contains 11,784 users with his/her latest historical pur-\\chase records in total of 116,532 user-item records} & \makecell[l]{Amazon.com}\\
    \hline
        \makecell[l]{Yu~\emph{et al.}~\cite{Yu2019ICCV}} & 2019 & 208,814 & N/A & \makecell[l]{It contains 797 users with 262 outfits and each outfit with\\ 2 items, i.e., a top and a bottom} & \makecell[l]{Polyvore.com}\\
    \hline 
        \makecell[l]{\href{https://github.com/wenyuer/POG}{POG}%\tablefootnote{\url{https://github.com/wenyuer/POG}}
        ~\cite{dong2019acmmm}} & 2019 & 1.01M & 80 & \makecell[l]{It is composed of 583,000 individual items} & \makecell[l]{Taobao.com,\\iFashion}\\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:outfit_matching_datasets}
    \begin{tablenotes}
      \scriptsize
      \item N/A: there is no reported information to cite ; M means million.
    \end{tablenotes}
\end{table*}

\subsubsection{Performance evaluations}
As the evaluation protocol for fashion compatibility (Sec.~\ref{sec:fashion_compatibility_PE}), AUC is the most used metric for outfit matching methods. %~\cite{he:aaai2016, veit:iccv2015, shih2018compatibility, YLi2017TMM, han2017learning, dong2019acmmm, Hou2019ijcai}.
%, song:sigir2018, vasileva:eccv2018
While some methods are also evaluated with NDCG, \textit{i.e.}, \cite{liu:mm2012, hu:mm2015, Hou2019ijcai}, and FITB (fill in the blank) accuracy, \textit{i.e.}, \cite{han2017learning, chen2019kdd}. Unfortunately, there is no unified benchmark for outfit matching, both in datasets and evaluation metrics. Therefore, we are unable to give a comparison of different methods.

%Some methods are evaluated with Normalized Discounted Cumulative Gain (NDCG)(\textit{i.e.}, \cite{liu:mm2012, hu:mm2015}), prediction accuracy (\textit{i.e.}, \cite{iwata:ijcai2011, hsiao2018creating, mcauley:sigir2015, han2017learning, vasileva:eccv2018, kang:cvpr2019}), recall$@k$ (\textit{i.e.}, \cite{chen2018dress}), or Average Precision (\textit{i.e.}, \cite{YLi2017TMM}). Unfortunately, there is no unified benchmark for outfit matching, both in datasets and evaluation metrics. Therefore, we are unable to give a comparison of different methods.

%Zhang~\emph{et al.}~\cite{zhang:tmm2017} used three common multi-label criteria, \textit{i.e.,} Macro-F, mean Average Precision (mAP), and Area under curve (AUC), to evaluate the quality of the results. 

%~\cite{iwata:ijcai2011}: The similarity evaluation measurement, which calculated as the average similarity between the recommended clothing and the held-out paired clothing.


%related to CY's recommendation
%\subsection{Style Classification}

%\subsubsection{State-of-the-art methods}

%A location-oriented clothing recommendation is presented in \cite{zhang:tmm2017}. 

%The works in \cite{hidayati:mm2018, sattar:wacv2019} developed frameworks for learning the compatibility of clothing styles and body shapes. 

%Sattar~\emph{et al.}~\cite{sattar:wacv2019} used multiple photos of the same person to estimate the body shape, whereby the body shape model is built based on 2D positions of body joints and silhouette. A conditional distribution of clothing category given the inferred body shape is computed to predict the best fitting clothing.

%Another work~\cite{sun:mtap2018} studied social-based recommendation on fashion style. The recommendation is implemented by combining user social circle and style consistency of clothing items. With this aim, the authors integrated a Siamese CNN-based learning model employed to analyze the fashion style consistency with social factors (\emph{i.e.}, personal interest, interpersonal interest similarity, and interpersonal influence) into a Probabilistic matrix factorization (PMF) framework.


%\begin{figure}
%  \centering
%  \subfigure[Magic Closet~\cite{liu:mm2012}.]
%  {\includegraphics[width=1\linewidth]{img/style_recommendation_liuMM2012.png}}

%  \subfigure[Trip Outfits Advisor~\cite{zhang:tmm2017}.]
%  {\includegraphics[width=0.9\linewidth]{img/style_recommendation_zhangTMM2016.png}}
  
%  \subfigure[Style for Body Shape~\cite{hidayati:mm2018}.]
%  {\includegraphics[width=1\linewidth]{img/style_recommendation_hidayatiMM2018.png}}

  %\subfigure[EI Tree~\cite{liao:mm2018}]
  %{\includegraphics[width=1\linewidth]{img/clothing_retrieval_liaoMM2018.png}}
  %\vspace{-2mm}
%  \caption{Pipelines of state-of-the-art style recommendation methods.}
%  \label{fig:clothing_retrieval_pipelines}
%\end{figure}

%\subsubsection{Benchmark datasets}

%Table~\ref{tab:style_recommendation_datasets} lists and compares the benchmark datasets used in~\cite{liu:mm2012, zhang:tmm2017, sun:mtap2018, hidayati:mm2018, sattar:wacv2019}. In particular, these datasets are mainly different in terms of the tasks covered.%Worthy to note, the rich social media provide valuable clues to solve the problems of fashion recommendations.

%\begin{table*}[htbp]
%\footnotesize
%    \centering
%        \caption{Summary of the benchmark datasets for style recommendation task.}
%        \vspace{-3mm}
%    \begin{tabular}{l|c|c|c|c|l|l}
%    \Xhline{1.0pt}
%      \multicolumn{2}{c|}{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ photos} & \makecell[c]{Task oriented} & \makecell[c]{Key features} & \makecell[c]{Source} \\
%    \hline
%       \multirow{2}{*}{\makecell[l]{Sun\\\emph{et al.}~\cite{sun:mtap2018}}} & \makecell[l]{Mogujie\_1} & \multirow{2}{*}{2017} & 74,686 & \multirow{2}{*}{\makecell{Social circle}} & \makecell[l]{Consists of 37,343 pairs of clothing items (tops\\ and bottoms) shared by fashion icons} & \multirow{2}{*}{\makecell[l]{Mogujie.com}}\\
%    \cline{2-2}\cline{4-4}\cline{6-6}
%         & \makecell[l]{Mogujie\_2} & & 30,050 &  & \makecell[l]{Contains 1031 users with their relationships} & \\
    %\hline
    %    \multicolumn{2}{c|}{\makecell[l]{Fashion Takes Shape~\cite{sattar:wacv2019}}} & 2019 & 18,413 & \makecell{Body shape} & \makecell[l]{Annotated with metadata including clothing cate-\\gory, and a manual shape annotation indicating \\ the person's shape is above average or average} & \makecell[l]{Chictopia.com}\\
%    \Xhline{1.0pt}
%    \end{tabular}
%    \label{tab:style_recommendation_datasets}
%\end{table*}


%\subsubsection{Performance evaluations}

%A subjective evaluation was conducted in~\cite{liu:mm2012, sun:mtap2018, hidayati:mm2018, sattar:wacv2019} to ensure the usability and functionality of the suggested styles match with users' preferences. 

\subsection{Hairstyle Suggestion}

Hairstyle plays an essential role in physical appearance. People can look completely different with a different hairstyle. The right hairstyle can enhance the best facial features while concealing the flaws, bringing out natural beauty and style. However, choosing the right hairstyle needs a careful selection as not all hairstyles suit all facial features.

\subsubsection{State-of-the-art methods}
In recent years, many papers have been published related to hairstyles focusing on how to model and render hairstyles with computer graphics~\cite{chai:tog2016, paris:tog2004, selle:tog2008, xu:tog2014, fei:tog2017} or on how to segment hair automatically~\cite{yacoob:tpami2006, rousset:icip2008, wang:accv2010, wang:cvpr2012, qin:icme2017}. Only little studies have been devoted to finding the right hairstyle to suit one's face. In the following, we review the literature concerning hairstyle recommendation.

The pioneering work in~\cite{yang:mmm2012} suggested suitable hairstyles for a given face by learning the relationship between facial shapes and successful hairstyle examples. The proposed example-based framework consisted of two steps: the statistical learning step and the composition step. The purpose of the statistical learning step was to find the most suitable hairstyle through Bayesian inference-based model that estimated the probability distributions of hairstyles to a face image. They proposed to use the ratio of line segments as the feature vector for characterizing the shape of each face, and $\alpha$-matting-based method to indicate hair area in the image. The most suitable hairstyle obtained from the statistical learning step was further superimposed over a given face image to output the face in a suitable hairstyle.

Liu~\emph{et al.} later developed the Beauty e-Experts system~\cite{liu:tomm14} to automatically recommend the most suitable facial hairstyle and makeup, and synthesize the visual effects. They proposed to use the extracted facial and clothing features to simultaneously learn multiple tree-structured super-graphs to collaboratively model the underlying relationships among the high-level beauty attributes (\emph{e.g.}, hair length, and eye shadow color), mid-level beauty-related attributes (\emph{e.g.}, eye shape and mouth width), and low-level image features. Besides, they also proposed a facial image synthesis module to synthesize the beauty attributes recommended by the multiple tree-structured super-graphs model. %into the testing image.

%Fig.~\ref{fig:hairstyle_suggestion_pipelines} illustrates the pipeline of the Beauty e-Experts system. 


%\begin{figure}[t!]
%  \centering
%%  \includegraphics[width=1\linewidth]{img/hairstyle_suggestion_liuMM2013.png}
%  \caption{Pipeline of the Beauty e-Experts system~\cite{liu:mm2013, liu:tomm14}.}
%  \label{fig:hairstyle_suggestion_pipelines}
%\end{figure}

\subsubsection{Benchmark datasets}

Table~\ref{tab:hairstyle_suggestion_dataset} provides benchmark datasets for assessing the performance of hairstyle suggestion methods. %described above. 
It is worth mentioning that Hairstyle30k~\cite{yin2017acmmm} is by far the largest dataset for hairstyle related problems thought the proposed method is not for hairstyle suggestion.

%In particular, these datasets were collected from hairstyle experts. 

\begin{table*}[t!]
\scriptsize
    \centering
        \caption{Summary of the benchmark datasets for hairstyle suggestion task.}
        \vspace{-3mm}
    \begin{tabular}{c|c|c|c|c}
    \Xhline{1.0pt}
      Dataset name & \makecell{Publish \\ time} & \makecell{\# of \\ photos} &  Key features & Sources \\
    \hline
        \makecell[l]{Yang~\emph{et al.}~\cite{yang:mmm2012}} & 2012 & 84 & \makecell[l]{Frontal face photos} & \makecell[l]{Hair stylists from 3 salons}\\
     \hline
        \makecell[l]{Beauty e-Experts\\\cite{liu:mm2014}} & 2013 & 1,605 & \makecell[l]{It consists of 20 hair color classes, 3 different hair\\ length attributes (long, medium, or short), 3 differ-\\ent hair shape attributes (straight, curled, or wavy),\\ and 2 kinds of hair volume (dense or normal)} & \makecell[l]{Professional hairstyle and makeup\\ websites (\emph{e.g.,} Stylebistro.com)}\\
    \hline
        \makecell[l]{Hairstyle30k\\\cite{yin2017acmmm}} & 2017 & 30,000 & \makecell[l]{It contains 64 different hairstyles} & \makecell[l]{Various web search engines (\emph{e.g.,}\\ Google, Flicker, and Bing)}\\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:hairstyle_suggestion_dataset}
\end{table*}


\subsubsection{Performance evaluations}

Yang~\emph{et al.}~\cite{yang:mmm2012} conducted a user study to evaluate the effectiveness of their proposed system, while Liu~\emph{et al.}~\cite{liu:tomm14} computed the NDCG that measures how close the ranking of the top-\textit{k} recommended styles is to the optimal ranking. However, we are unable to give comparisons on different hairstyle suggestion methods due to inconsistent benchmarks for different papers.

==> ACMCSUR – Fashion/src/fffashion_synthesis.tex <==
\section{Fashion Synthesis}
\label{sec:fffashion_synthesis}

Given an image of a person, we can imagine what that person would like in a different makeup or clothing style. We can do this by synthesizing a realistic-looking image. In this section, we review the progress to address this task, including style transfer, pose transformation, and physical simulation.
%facial makeup synthesis and clothing synthesis.

\subsection{Style Transfer}
Style transfer is transferring an input image into a corresponding output image such as transferring a real-world image into a cartoon-style image, transferring a non-makeup facial image into a makeup facial image, or transferring the clothing, which is tried on the human image, from one style to another. Style transfer in image processing contains a wide range of applications, \emph{e.g.}, facial makeup and virtual try-on. 

\subsubsection{State-of-the-art methods} The most popular style transfer work is pix2pix~\cite{isola2017image}, which is a general solution for style transfer. It learns not only the mapping from the input image to output image but also a loss function to train the mapping. For specific goal, based on a texture patch, ~\cite{jiang2017fashion, xian2018cvpr}\footnote{\url{https://github.com/janesjanes/Pytorch-TextureGAN}} transferred the input image or sketch to the corresponding texture. Based on the human body silhouette, ~\cite{lassner2017generative, Han2019iccv} inpainted compatible style garments to synthesize realistic images. An interesting work~\cite{Shi2019iccv} learned to transferred the facial photo into the game character style.

%The work in~\cite{lassner2017generative} presented a generative model of people in clothing for the full body, but it is not clear how to control the appearance of the generated results.
%Another interesting work is fashion style generator~\cite{jiang2017fashion}, which generates a clothing image with the certain style. Rather than applying a global method on artistic style, the fashion style generator combines both global and patch based methods, to keep global structure and high fidelity of details at the same time.

\textbf{Facial Makeup}. %Facial makeup is a technique to beautify one's appearance with unique cosmetics, such as eyeshadow, lipstick, and foundation. 
Finding the most suitable makeup for a particular human face is challenging, given the fact that a makeup style varies from face-to-face due to the different facial features. %Different facial features of each person is also a challenge to recover the original face from makeup face. Notably, 
Studies on how to automatically synthesize the effects of with or without makeup on one's facial appearance have aroused interest recently. %in recent years. We would also like to mention that 
There is a survey on computer analysis of facial beauty provided %by Laurentini and Bottino
in~\cite{laurentini:cviu2014}. However, it is limited to the context of the perception of attractiveness.

%\subsection{Facial makeup synthesis}
%\label{subsec:makeup_synthesis}
%\subsubsection{State-of-the-art methods}
%We can classify existing studies related to facial makeup into three problem areas, namely facial makeup detection, facial makeup transfer, and facial makeup removal (\emph{cf}. Fig.~\ref{fig:facial_makeup_synthesis}). Basically, there are two ways of achieving this task, either by traditional image processing approaches or by deep learning based methods.

%\textbf{Facial Makeup Detection.} The purpose of facial makeup detection is to design a system to recognize the presence of makeup in face images. Since facial makeup alters the appearance of a person, such makeup detection applications are useful to assist and improve automated face image analysis techniques~\cite{chen:btas2012}. In particular, the studies in~\cite{chen:icb2013,hu:icassp2013,guo:casvt2014,liu:icip2015, kose:fg2015} designed facial makeup detection frameworks based on low-level features. Chen~\emph{et al.}~\cite{chen:icb2013} extracted a feature vector that captures the shape, texture, and color information of the face image. Hu~\emph{et al.}~\cite{hu:icassp2013} and Guo~\emph{et al.}~\cite{guo:casvt2014} explored correlation mapping between the makeup and non-makeup faces. Instead of learning a correlation of global faces between makeup and non-makeup as in~\cite{hu:icassp2013}, \cite{guo:casvt2014} proposed to use features extracted from local patches. Liu~\emph{et al.}~\cite{liu:icip2015} extracted feature vector from the facial entropy information and further adopted a feature selection procedure to reduce redundant information on the extracted feature vector.~\cite{chen:icb2013,hu:icassp2013,guo:casvt2014, liu:icip2015} employed the Support Vector Machine (SVM) as the classifier. In~\cite{kose:fg2015}, Kose~\emph{et al.} utilized shape and texture features extracted from the entire face and employed two types of classifiers, \emph{i.e.,} SVM and Alligator. Their study suggested that Alligator classifier performed better than the SVM classifier.

%Attribute-based methods have shown promising potential to solve facial makeup detection problem and have recently been receiving much attention~\cite{wen:jcvip2013, zheng:icip2016, zheng:fg2017}. In~\cite{wen:jcvip2013}, Wen and Guo used the shared attributes to measure the similarity between a pair of makeup and non-makeup faces for matching, rather than a direct match, with low-level features. Zheng and Guo~\cite{zheng:icip2016} proposed to incorporate the low-level and mid-level features into a joint optimization framework. The low-level features are extracted from raw pixels with PCA for dimensionality reduction, whereas the mid-level features are composed of facial attributes measured by the distance from the SVM hyperplane. Transformations are learned to maximize between-class dissimilarity and minimize within-class dissimilarity. Later, Zheng and Kambhamettu introduced a hierarchical feature learning framework~\cite{zheng:fg2017} that combines both feature-augmentation and feature-transformation strategies. The feature-augmentation aims to form a feature representation by integrating mid-level and low-level features, while the feature-transformation is to learn transformations on feature representations at different levels.


%\textbf{Facial Makeup Transfer.} 
Facial makeup transfer refers to translate the makeup from a given face to another one while preserving the identity as Fig.~\ref{fig:style_transfer}(a). It provides an efficient way for virtual makeup try-on and helps users select the most suitable makeup style. The early work achieved this task by image processing methods~\cite{CLi2015CVPR}, 
%~\cite{guo2009digital, xu:icip2013, CLi2015CVPR}
which decomposed images into multiple layers and transferred information from each layer after warping the reference face image to a corresponding layer of the non-makeup one. One major disadvantage of this method was that it required warping the reference face image to the non-makeup face image, which was very challenging and inclined to generate artifacts in many cases. Liu~\emph{et al.}~\cite{liu:ijcai2016} first adopted a deep learning framework for makeup transfer. They employed several independent networks to transfer each cosmetic on the corresponding facial part. The simple combination of several components applied in this framework, however, leads to unnatural artifacts in the output image. To address this issue, Alashkar~\emph{et al.}~\cite{alashkar:aaai2017} trained a deep neural network based makeup recommendation model from examples and knowledge base rules jointly. The suggested makeup style was then synthesized on the subject face. %\cite{alashkar:fg2017} further built upon the previous study \cite{alashkar:aaai2017} by taking into account the makeup trends for different occasions or events.


\begin{figure}[t!]
  \centering
  %\subfigure [Facial makeup transfer]
  %{\includegraphics[width=0.3\textwidth]{img/makeup_transfer.png}}~~~~~~~~
  %\subfigure [Facial makeup detection and removal~\cite{AWang2016AAAI}]
  %{\includegraphics[width=0.3\textwidth]{img/makeup_detection_removal.png}}
  %\subfigure [Comparison of VITON~\cite{han2018viton} and CP-VTON~\cite{wang2018toward}]
  %{\includegraphics[width=0.35\textwidth]{img/virtual_try_on2.png}}
  \includegraphics[width=\linewidth]{img/style_transfer_example.png}
  \vspace{-5mm}
  \caption{(a) Facial makeup transfer~\cite{chen:cvpr2019}. (b) Facial makeup detection and removal~\cite{AWang2016AAAI}. (c) Comparison of VITON~\cite{han2018viton} and CP-VTON~\cite{wang2018toward}.}
  %\caption{Examples of style transfer.}
  \label{fig:style_transfer}
  %\label{fig:facial_makeup_synthesis}
\end{figure}

%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=0.4\linewidth]{img/makeup_transfer_2.pdf}
%  \vspace{-3mm}
%  \caption{\textcolor{red}{Examples of makeup transfer with PairedCycleGAN~\cite{HChang2018CVPR}.}}
%  \label{fig:makeup_transfer}
%\end{figure}

%\textbf{Facial Makeup Removal.} 
Different makeup styles result in significant facial appearance changes, which brings challenges to many practical applications, such as face recognition. Therefore, researchers also devoted themselves to makeup removal as Fig.~\ref{fig:style_transfer}(b), which is an ill-posed problem. Wang and Fu~\cite{AWang2016AAAI} proposed a makeup detector and remover framework based on locality-constrained dictionary learning. Li \emph{et al.}~\cite{YLi2018AAAI} later introduced a bi-level adversarial network %(BLAN) 
architecture, where the first adversarial scheme was to reconstruct face images, and the second was to maintain face identity.

%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=0.4\linewidth]{img/makeup_synthesis_wangAAAI2016.png}
%  \vspace{-3mm}
%  \caption{\textcolor{red}{Examples of facial makeup removal~\cite{AWang2016AAAI}.}}
%  \label{fig:makeup_removal}
%\end{figure}

%\textbf{Facial Makeup Transfer and Removal.} 
Unlike the aforementioned facial makeup synthesis methods that treat makeup transfer and removal as separate problems,~\cite{HChang2018CVPR, li2018beautygan, chen:cvpr2019, LADN2019iccv} performed makeup transfer and makeup removal simultaneously. Inspired by CycleGAN architecture~\cite{zhu2017unpaired}, Chang~\emph{et al.}~\cite{HChang2018CVPR} introduced the idea of asymmetric style transfer and a framework for training both the makeup transfer and removal networks together, each one strengthening the other. Li~\emph{et al.}~\cite{li2018beautygan} proposed a dual input/output generative adversarial network called BeautyGAN for instance-level facial makeup transfer. More recent work by Chen~\emph{et al.}~\cite{chen:cvpr2019} presented BeautyGlow that decomposed the latent vectors of face images derived from the Glow model into makeup and non-makeup latent vectors. For achieving better makeup and de-makeup performance, Gu~\emph{et al.}~\cite{LADN2019iccv} focused on local facial details transfer and designed a local adversarial disentangling network which contained multiple and overlapping local adversarial discriminators.

\textbf{Virtual Try-On}. Data-driven clothing image synthesis is a relatively new research topic that is gaining more and more attention. In the following, we review existing methods and datasets for addressing the problem of generating images of people in clothing by focusing on the styles. 
%Mirror Mirror~\cite{saakes:chi2016} is a virtual fitting room mirror that allows a designer to create their own shirt prints on top of their bodies... %But this approach requires expensive devices.
%Product-human transfer refers to generate a clothed person image conditioned on a product. Yoo \emph{et al.}~\cite{yoo2016pixel} regarded product-human transfer as a domain adaptation problem. Besides a generator and a real/fake discriminator, a domain discriminator was designed to train the semantic relation between the product images and human images. The drawbacks of~\cite{yoo2016pixel} was that the model can only deal with images in the resolution of $64\times64$, and the generated results were far from satisfactory. Nevertheless, it was a milestone work that first applied GANs to product-human transfer.
%To improve the transfer results, 
Han \emph{et al.}~\cite{han2018viton} utilized a coarse-to-fine strategy. Their framework, VIrtual Try-On Network (VITON), focused on trying an in-shop clothing image on a person image. It first generated a coarse tried-on result and predicted the mask for the clothing item. Based on the mask and coarse result, a refinement network for the clothing region was employed to synthesize a more detailed result. However,~\cite{han2018viton} fails to handle large deformation, especially with more texture details, due to the imperfect shape-context matching for aligning clothes and body shape. Therefore, a new model called Characteristic-Preserving Image-based Virtual Try-On Network (CP-VTON)~\cite{wang2018toward} was proposed. The spatial deformation can be better handled by a Geometric Matching Module, which explicitly aligned the input clothing with the body shape. The comparisons of VITON and CP-VTON are given in Fig.~\ref{fig:style_transfer}(c). There were several improved works~\cite{LAVITON2019iccv, Ayush2019iccv, VTNFP2019iccv, adaptive2020CVPR} based on CP-VTON. Different from the previous works which needed the in-shop clothing image for virtual try-on, FashionGAN~\cite{zhu2017your} and M2E-TON~\cite{M2E2019acmmm} presented target try-on clothing image based on text description and model image respectively. Given an input image and a sentence describing a different outfit, FashionGAN was able to ``redress'' the person. A segmentation map was first generated with a GAN according to the description. Then, the output image was rendered with another GAN guided by the segmentation map. M2E-TON was able to try on clothing from human$_A$ image to human$_B$ image, and two people can perform in different poses. Considering the runtime efficacy, Issenhuth \emph{et al.}~\cite{parsingfree2020eccv} proposed a parser free virtual try-on network. It designs a teacher-student architecture to free the parsing process during the inference time for improving efficiency.

Viewing the try-on performance from different views is also essential for virtual try-on task, Fit-Me~\cite{fitme2019icip} was the first work to do virtual try-on with arbitrary poses in 2019. They designed a coarse-to-fine architecture for both pose transformation and virtual try-on. Further, FashionOn~\cite{fashionon} applied the semantic segmentation for detailed part-level learning and focused on refining the facial part and clothing region to present more realistic results. They succeeded in preserving detailed facial and clothing information, perform dramatic posture, and also resolve the human limb occlusion problem in CP-VTON. Similar architecture to CP-VTON for virtual try-on with arbitrary poses was presented by~\cite{virtually2019acmmm}. They further made body shape mask prediction at the beginning of the first stage for pose transformation, and, in the second stage, they presented an attentive bidirectional GAN to synthesize the final result. For pose-guided virtual try-on, Dong~\emph{et al.}~\cite{Dong:iccv2019} further improved VITON and CP-VTON, which tackled the virtual try-on for different poses. Han~\emph{et al.}~\cite{clothflow2019iccv} proposed ClothFlow to focus on the clothing regions and model the appearance flow between source and target for transferring the appearance naturally and synthesizing novel result. Beyond the abovementioned image-based virtual try-on works, Dong~\emph{et al.}~\cite{FWGAN2019iccv} presented a video virtual try-on system, FWGAN, which learned to synthesize a video of virtual try-on results based on a person image, a target try-on clothing image and a series of target poses.
Increasing the image resolution of virtual try-on, \cite{unpaired2020cvpr,highRes2019iccvw} further design novel architectures for achieving multi-layer virtual try-on.

\subsubsection{Benchmark datasets}
Style transfer for fashion contains two hot tasks, facial makeup and virtual try-on. Existing makeup datasets applied for studying facial makeup synthesis typically assemble pairs of images for one subject: non-makeup image and makeup image pair. As for virtual try-on, since it is a highly diverse topic, there are several datasets for different tasks and settings. We summarize the datasets for style transfer in Table~\ref{tab:style_transfer_dataset}.

\begin{table*}[t!]
\notsotiny
\center
\caption{Summary of the benchmark datasets for style transfer task.}
\vspace{-3mm}
\begin{tabular}{l||c|c|c|c|c}
  \Xhline{1.0pt}
  \hline
  \makecell{Task} & Dataset name & \makecell{Publish\\time} & \makecell{\# of\\ photos} & Key features & Sources\\
  \hline
  \multirow{17}{*}{\makecell[l]{Facial\\ Makeup}} &
%    \makecell[l]{YouTube\\Makeup \cite{chen:btas2012}} & 2012 & 604 & \makecell[l]{151 Caucasian female subjects with 2 non-makeup images and 2\\ makeup images for each subject} & \makecell[l]{YouTube makeup\\ tutorial videos} \\ 
%  \cline{2-6}
%    & \makecell[l]{Makeup in the \\Wild \tablefootnote{\url{http://www.antitza.com/makeup-datasets.html}}\cite{chen:icb2013}} & 2013 & 154 & \makecell[l]{77 non-makeup images and 77 makeup images} & \makecell[l]{The Internet} \\
%  \cline{2-6}
%    & \makecell[l]{FAM~\cite{hu:icassp2013}} & 2013 & 1,038 & \makecell[l]{519 subjects (222 males and 297 females), where each subject\\ has a pair of photos being with and without makeup} & \makecell[l]{N/A} \\ 
%  \cline{2-6}
%    & \makecell[l]{FCD\tablefootnote{\url{http://fcd.eurecom.fr/}}~\cite{eckert:mmsp2013}} & 2013 & 385 & \makecell[l]{50 reference images and 335 makeup serie images} & \makecell[l]{N/A} \\ 
%  \cline{2-6}
%    & \makecell[l]{Guo~\emph{et al.}~\cite{guo:casvt2014}} & 2014 & 1,002 & \makecell[l]{501 female subjects, where each subject has a pair of photos being\\ with and without makeup} & \makecell[l]{The Internet} \\
%  \cline{2-6}
%    & 
    \makecell[l]{Liu~\emph{et al.}~\cite{liu:ijcai2016}} & 2016 & 2,000 & \makecell[l]{1000 non-makeup faces and 1000 reference faces} & \makecell[l]{N/A} \\
  \cline{2-6}
    & \makecell[l]{Stepwise \\Makeup \cite{AWang2016AAAI}} & 2016 & 1,275 & \makecell[l]{Images in 3 sub-regions (%540 
    eye%images, 235 
    , mouth%images
    , and % 500 
    skin%\\ images
    );\\ labeled with procedures of makeup} & \makecell[l]{N/A} \\
  \cline{2-6}
    & \makecell[l]{Beauty~\cite{zheng:fg2017}} & 2017 & 2,002 & \makecell[l]{1,001 subjects, where each subject has a pair of photos being with\\ and without makeup} & \makecell[l]{The Internet} \\
  \cline{2-6}
    & \makecell[l]{Before-After \\Makeup\cite{alashkar:aaai2017}} & 2017 & 1,922 & \makecell[l]{961 different females (224 Caucasian, 187 Asian, 300 African, and\\ 250 Hispanic) where one with clean face and another after pro-\\fessional makeup; annotated with facial attributes%; frontal face with no occlusion
    } & \makecell[l]{N/A}\\
  \cline{2-6}
    & \makecell[l]{Chang~\emph{et al.}\\\cite{HChang2018CVPR}} & 2018 & 2,192 & \makecell[l]{1,148 non-makeup images and 1,044 makeup images} & \makecell[l]{Youtube makeup\\ tutorial videos}\\
  \cline{2-6}
    & \makecell[l]{Makeup\\Transfer~\cite{li2018beautygan}} & 2018 & 3,834 & \makecell[l]{1,115 non-makeup images and 2,719 makeup images; assembled\\ with 5 different makeup styles (smoky-eyes, flashy, Retro, Ko-\\rean, and Japanese makeup styles), varying from subtle to heavy} & \makecell[l]{N/A}\\
  \cline{2-6}
    & \makecell[l]{\href{https://georgegu1997.github.io/LADN-project-page/}{LADN}%\tablefootnote{\url{https://georgegu1997.github.io/LADN-project-page/}}
    ~\cite{LADN2019iccv}} & 2019 & 635 & \makecell[l]{333 non-makeup images and 302 makeup images} & \makecell[l]{The Internet}\\
 \cline{2-6}
    & \makecell[l]{\href{https://github.com/wtjiang98/PSGAN}{Makeup-Wild}~\cite{PSGAN2020cvpr}} & 2020 & 772 & \makecell[l]{369 non-makeup images and 403 makeup images} & \makecell[l]{The Internet}\\
  \hline\hline    
    \multirow{13}{*}{\makecell[l]{Virtual\\Try-On}} & \makecell[l]{\href{http://mmlab.ie.cuhk.edu.hk/projects/FashionGAN/}{LookBook}%\tablefootnote{\url{http://mmlab.ie.cuhk.edu.hk/projects/FashionGAN/}}
    \\~\cite{yoo2016pixel}} & 2016 & 84,748 & \makecell[l]{The 9,732 top product images are associated with 75,016 fashion\\ model images} & \makecell[l]{Bongjashop, Jogunshop,\\ Stylenanda, SmallMan,\\ WonderPlace}\\
  \cline{2-6}
    & \makecell[l]{\href{http://mmlab.ie.cuhk.edu.hk/projects/DeepFashion/FashionSynthesis.html}{DeepFashion}%\tablefootnote{\url{http://mmlab.ie.cuhk.edu.hk/projects/DeepFashion/FashionSynthesis.html}}
    \\\cite{liu2016deepfashion}} & 2016 & 78,979 & \makecell[l]{The corresponding upper-body images, sentence descriptions, and\\ human body segmentation maps} & \makecell[l]{Forever21} \\
  \cline{2-6}  
    & \makecell[l]{CAGAN~\cite{CAGAN2017iccvw}} & 2017 & 15,000 & \makecell[l]{Frontal view human images and paired upper-body garments\\ (pullovers and hoodies)} & \makecell[l]{Zalando.com} \\
  \cline{2-6}  
    & \makecell[l]{\href{https://github.com/xthan/VITON}{VITON}%\tablefootnote{\url{https://github.com/xthan/VITON}}
    ~\cite{han2018viton}} & 2018 & 32,506 & \makecell[l]{Pairs of frontal-view women and top clothing images} & \makecell[l]{N/A} \\
  \cline{2-6}  
    & \makecell[l]{\href{https://fashiontryon.wixsite.com/fashiontryon}{FashionTryOn}%\tablefootnote{\url{https://fashiontryon.wixsite.com/fashiontryon}}
    \\\cite{virtually2019acmmm}} & 2019 & 28,714 & \makecell[l]{Pairs of same person with same clothing in 2 different poses and\\ one corresponding clothing image} & \makecell[l]{Zalando.com} \\
  \cline{2-6}  
    & \makecell[l]{FashionOn~\cite{fashionon}} & 2019 & 22,566 & \makecell[l]{Pairs of same person with same clothing in 2 different poses and\\ one corresponding clothing image} & \makecell[l]{The Internet,\\DeepFashion~\cite{liu2016deepfashion}} \\
  \cline{2-6}  
    & \makecell[l]{Video Virtual\\ Try-on \cite{FWGAN2019iccv}} & 2019 & \makecell{791\\videos} & \makecell[l]{Each video contains 250--300 frame numbers} & \makecell[l]{fashion model catwalk} \\
  \hline
  %\hline
  \Xhline{1.0pt}
\end{tabular}
\label{tab:style_transfer_dataset}
    \begin{tablenotes}
      \scriptsize
      \item N/A: there is no reported information to cite.
    \end{tablenotes}
\end{table*}

\subsubsection{Performance evaluations}
\label{sec:virtual_try_on_PE}
%Studies on facial makeup detection primarily use accuracy to assess performance. Accuracy calculates the proportion of correctly classified instances. Meanwhile, 
The evaluation for 
%facial makeup transfer and removal 
style transfer is generally based on subjective assessment or user study. That is, the participants rate the results into some certain degrees, such as ``Very bad'', ``Bad'', ``Fine'', ``Good'', and ``Very good''. The percentages of each degree are then calculated to quantify the quality of results. % Besides, in~\cite{AWang2016AAAI}, the makeup detector is evaluated in the context of face verification. The performance is reported using Receiver Operating Characteristic (ROC) curve, where the true positive rate is plotted as a function of the false positive rate. 
%We show performance comparisons of different facial makeup detection methods on three benchmark datasets in Table~\ref{table:makeup_detection_results}. 
Besides, there are objective comparisons for virtual try-on, in terms of inception score (IS) or structural similarity (SSIM). IS is used to evaluate the synthesis quality of images quantitatively. The score will be higher if the model can produce visually diverse and semantically meaningful images. On the other hand, SSIM is utilized to measure the similarity between the reference image and the generated image ranging from zero (dissimilar) to one (similar).

%\begin{table}[t!]
%\small
%\center
%\caption{Performance comparisons of facial makeup detection methods in terms of accuracy (\%).}
%\vspace{-3mm}
%\begin{tabular}{c|c|c|c}
%  \Xhline{1.0pt}
%   \multirow{2}{*}{Method} & \multicolumn{3}{c}{Dataset}\\
%   \cline{2-4}
%   & FAM~\cite{hu:icassp2013} & Beauty~\cite{zheng:fg2017} & Guo~\emph{et al.}~\cite{guo:casvt2014}\\
%   \hline
%   \makecell[l]{Dual-Attribute~\cite{wen:jcvip2013}} & $69.02\pm0.92$ & $70.39\pm2.95$ & 71.00 \\
%   \hline
%   \makecell[l]{CCA~\cite{guo:casvt2014}} & $69.83\pm3.01$ & $71.10\pm1.90$ & 72.50\\
%   \hline
%   \makecell[l]{PLS~\cite{guo:casvt2014}} & $74.28\pm3.24$ & $77.85\pm3.14$ & 80.50\\
%   \hline
%   \makecell[l]{Zheng~\emph{et al.}~\cite{zheng:icip2016}} & -- & -- & \textbf{82.50}\\
%   \hline
%   \makecell[l]{Zheng and Kambhamettu~\cite{zheng:fg2017}} & $\textbf{76.68}\pm\textbf{5.88}$ & $\textbf{81.11}\pm\textbf{2.09}$ & --\\
%  \Xhline{1.0pt}
%\end{tabular}
%    \begin{tablenotes}
%      \scriptsize
%      \item ``--'' represents detailed results are not available ; The best result for each dataset is highlighted in bold font.
%    \end{tablenotes}
%\label{table:makeup_detection_results}
%\end{table}



\subsection{Pose Transformation}
Given a reference image and a target pose only with keypoints, the goal of pose transformation is to synthesize pose-guided person image in different posture while keeping personal information. A few examples of pose transformation are shown in Fig.~\ref{fig:pose_transformation_example}. Pose transformation, in particular, is a challenging task since the input and output are not spatially aligned.

%Given a reference image and a target pose, the goal of pose-guided person image generation is to change the pose of a given person image to another while keeping human information. A few examples of pose-guided person image generation are shown in Fig.~\ref{fig:pose_transformation_example}. This in particular is a challenging task since the input and output are not spatially aligned. 

\subsubsection{State-of-the-art methods}
A two-stage adversarial network PG$^2$~\cite{ma2017pose} achieved an early attempt on this task. A coarse image under the target pose was generated in the first stage and then refined in the second stage. The intermediate results and final results are shown % in two benchmark datasets, DeepFashion and Market-1501, respectively 
in Fig.~\ref{fig:pose_transformation_example}(a)-(b) 
with two benchmark datasets. 
However, the results were highly blurred, especially for texture details. To tackle the problem, the affine transform was employed to keep textures in the generated images better%~\cite{siarohin2018deformable,balakrishnan2018synthesizing}. 
. Siarohin~\emph{et al.}~\cite{siarohin2018deformable} designed a deformable GAN, in which the key deformable skip elegantly transforms high-level features for each body part. Similarly, the work in~\cite{balakrishnan2018synthesizing} employed body part segmentation masks to guide the image generation. The proposed framework contained four modules, including source image segmentation, spatial transformation, foreground synthesis, and background synthesis that can be trained jointly. %Note that~\cite{ma2017pose,siarohin2018deformable,balakrishnan2018synthesizing} are trained with paired data.
Further, Si~\emph{et al.}~\cite{Si:cvpr2018} introduced a multistage pose-guided image synthesis framework, which divided the network into three stages for pose transform in a novel 2D view, foreground synthesis, and background synthesis. 

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{img/pose_tranformation_example.png}\\
  \caption{Examples of pose transformation~\cite{ma2017pose}.}
  \label{fig:pose_transformation_example}
\end{figure}

To break the data limitation of previous studies, Pumarola~\emph{et al.}~\cite{pumarola2018unsupervised} borrowed the idea from~\cite{zhu2017unpaired} by leveraging cycle consistency% to achieve unsupervised person image generation for arbitrary poses
. In the meantime, the works in~\cite{ma2018disentangled,esser2018variational} formulated the problem %of pose-guided image generation 
from the perspective of variational auto-encoder (VAE). %These methods~\cite{ma2018disentangled,esser2018variational} 
They can successfully model the body shape; however, their results were less faithful to the appearance of reference images since they generated results from highly compressed features sampled from the data distribution. To improve the appearance performance%for pose transformation work
, Song~\emph{et al.}~\cite{song2019pose}\footnote{\url{https://github.com/SijieSong/person_generation_spt}} designed a novel pathway to decompose the hard mapping into two accessible subtasks, semantic parsing transformation and appearance generation. Firstly, for simplifying the non-rigid deformation learning, it transformed the posture in semantic parsing maps. Then, synthesizing the semantic-aware human information to the previous synthesized semantic maps formed the realistic final results. % Since this was an unsupervised work, the training process was designed to reverse the generation process back to the source image in an end-to-end manner for advancing the two networks mutually.
Conducting the concept of optical flow, Ren~\emph{et al.}~\cite{gfla2020cvpr} proposed a differentiable global-flow local-attention framework to ensemble the features between source human, source pose, and target pose.


\subsubsection{Benchmark datasets}
The benchmark datasets for pose transformation are very limited. The most used two benchmark datasets are Market-1501~\cite{zheng2015scalable} and DeepFashion (In-shop clothes retrieval benchmark)~\cite{liu2016deepfashion}. Besides, there is one dataset collected in videos~\cite{balakrishnan2018synthesizing}. All of the three datasets are summarized in Table~\ref{table:pose_transformation_dataset}.


\begin{table*}[t!]
\scriptsize
\center
\caption{Summary of the benchmark datasets for pose transformation task.}
\vspace{-3mm}     
\begin{tabular}{c|c|c|c|c}
  \Xhline{1.0pt}
   Dataset name & \makecell{Publish\\time} & \makecell{\# of\\ photos} & Key features & Sources\\
   \hline
    \makecell[l]{\href{http://vision.imar.ro/human3.6m}{Human3.6M}%\tablefootnote{\url{http://vision.imar.ro/human3.6m}}
    ~\cite{human36m_tpami}} & 2014 & 3.6M & \makecell[l]{ It contains 32 joints for each skeleton} & \makecell[l]{self-collected}\\
  \hline 
    \makecell[l]{\href{http://www.liangzheng.com.cn/Project/project_reid.html}{Market-1501}%\tablefootnote{\url{http://www.liangzheng.com.cn/Project/project_reid.html}}
    ~\cite{zheng2015scalable}} & 2015 & 32,668 & \makecell[l]{Multiple viewpoints; the resolution of\\ images is 128$\times$64} & \makecell[l]{A supermarket in Tsinghua University}\\
  \hline
    {\makecell[l]{\href{http://mmlab.ie.cuhk.edu.hk/projects/DeepFashion/InShopRetrieval.html}{DeepFashion}%\tablefootnote{\url{http://mmlab.ie.cuhk.edu.hk/projects/DeepFashion/InShopRetrieval.html}}
    ~\cite{liu2016deepfashion}}} & 2016 & 52,712 & \makecell[l]{The resolution of images is 256$\times$256} & \makecell[l]{Online shopping sites (Forever21 and \\Mogujie), Google Images}\\
  \hline
    \makecell[l]{Balakrishnan~\emph{et al.}~\cite{balakrishnan2018synthesizing}} & 2018 & N/A & \makecell[l]{ Action classes: golf swings (136 videos),\\ yoga/workout routines (60 videos), and \\tennis actions (70 videos)} & \makecell[l]{YouTube}\\
  \Xhline{1.0pt}
\end{tabular}
    \begin{tablenotes}
      \scriptsize
      \item N/A: there is no reported information to cite. M means million.
    \end{tablenotes}
\label{table:pose_transformation_dataset}
\end{table*}

\subsubsection{Performance evaluations}
%Similar to facial makeup synthesis task, the evaluation for fashion synthesis is generally based on subjective test, \emph{e.g.}, user study. For the task of pose-guided image generation, 
There are objective comparisons for pose transformation, in terms of %inception score (IS) or structural similarity (SSIM). IS is used to quantitatively evaluate the synthesis quality of images. The score will be higher if the model can produce visually diverse and semantically meaningful images. On the other hand, SSIM is utilized to measure the similarity between the reference image and the generated image ranging from zero (dissimilar) to one (similar). 
IS and SSIM, which have been introduced in Sec.~\ref{sec:virtual_try_on_PE}. Additionally, to eliminate the effect of background, mask-IS and mask-SSIM were proposed in~\cite{ma2017pose}. %Table~\ref{table:pose_guided_generation_results} gives the comparisons of different approaches %for pose transformation
%on the DeepFashion and Market-1501. 
%A pose mask is added to both the generated and ground-truth images before computing IS and SSIM.
%The best results are marked in bold font, while the results not provided in the corresponding papers are marked using a dash. ``--'' represents the results are not provided in the corresponding papers.
%Note that these results are just indicative, as the test splits might differ between the different methods. 

%\begin{table*}[t!]
%\footnotesize
%\centering
%		\caption{Comparisons of pose transformation methods. }
%		\label{table:pose_guided_generation_results}
%		\begin{tabular}{c|c|c|c|c|c|c}
%		\Xhline{1.0pt}
%        \multirow{2}{*}{Model} &\multicolumn{2}{c|}{DeepFashion~\cite{liu2016deepfashion}} & \multicolumn{4}{c}{Market-1501~\cite{zheng2015scalable}}  \\
%        \cline{2-7}
%		 &  IS    & SSIM  & IS    & SSIM  & mask-IS & mask-SSIM \\
%        \hline
%        \makecell[l]{PG$^2$~\cite{ma2017pose}} & 3.090 & 0.762 & 3.460 & 0.253 & 3.435   & 0.792 \\
%        \hline
%        \makecell[l]{Siarohin~\emph{et al.}~\cite{siarohin2018deformable}} & \textbf{3.439} & 0.756 & 3.185 & 0.290 & \textbf{3.502} & \textbf{0.805} \\
        %\hline
        %\makecell[l]{Pumarola~\emph{et al.}~\cite{pumarola2018unsupervised}} & 2.971 & 0.747 & -- & -- & -- & -- \\
%        \hline
%        \makecell[l]{BodyROI7~\cite{ma2018disentangled}} &  3.228 & 0.614 & \textbf{3.483} & 0.099 & 3.491 & 0.614 \\
%        \hline
%        \makecell[l]{V-Unet~\cite{esser2018variational}} &  3.087 & \textbf{0.786} & 3.214 & \textbf{0.353} & -- & -- \\
%		\Xhline{1.0pt}
%		\end{tabular}
%		\begin{tablenotes}
%        \scriptsize
        %\footnotesize
%        \item The best results are marked in bold font, while ``--'' represents detailed results are not available.
        %the results not provided in the corresponding papers are marked using a dash.
%        \item Note that these results are just indicative, as the test splits might differ between the different methods. 
%        \end{tablenotes}
%\end{table*}




\subsection{Physical Simulation}
For more vivid fashion synthesis performance, physical simulation plays a crucial role. The abovementioned synthesis works are within the 2D domain, limited in the simulation of the physical deformation, e.g., shadow, pleat, or hair details. For advancing the synthesis performance with dynamic details (drape, or clothing-body interactions), there are physical simulation works based on 3D information. Take Fig.~\ref{fig:physical_simulation_example} for example. Based on a body animation sequence (a), the shape of the target garment and keyframes (marked by yellow), Wang~\emph{et al.}~\cite{wang2019acmtog} learned the intrinsic physical properties and simulated to other frames with different postures which are shown in (b).

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{img/physical_simulation.png}\\
  \caption{Examples of physical simulation~\cite{wang2019acmtog}.}
  \label{fig:physical_simulation_example}
\end{figure}

\subsubsection{State-of-the-art methods}
The traditional pipeline for designing and simulating realistic clothes is to use computer graphics to build 3D models and render the output images~\cite{wang:tog11, guan:tog2012, yang:iccv2017, pons-moll:tog2017}. 
%, kim:tog2013
For example, Wang~\emph{et al.}~\cite{wang:tog11} developed a piecewise linear elastic model for learning both stretching and bending in real cloth samples. For learning the physical properties of clothing on different human body shapes and poses, Guan~\emph{et al.}~\cite{guan:tog2012} designed a pose-dependent model to simulate clothes deformation. For simulating regular clothing on fully dressed people in motion, Pons-Moll~\emph{et al.}~\cite{pons-moll:tog2017} designed a multi-part 3D model called ClothCap. Firstly, it separated different garments from the human body for estimating the clothed body shape and pose under the clothing. Then, it tracked the 3D deformations of the clothing over time from 4D scans to help simulate the physical clothing deformations in different human posture. To enhance the realism of the garment on human body, L{\"{a}}hner~\emph{et al.}~\cite{Zorah2018DeepWrinkles} proposed a novel framework, which composed of two complementary modules: (1) A statistical model learned to align clothing templates based on 3D scans of clothed people in motion and a linear subspace model factored out the human body shape and posture. (2) A cGAN added high-resolution geometric details to normal maps and simulated the physical clothing deformations. 

For advancing the physical simulation with non-linear deformations of clothing, Santesteban~\emph{et al.}~\cite{Santesteban2019cgf} presented a two-level learning-based clothing animation method for highly efficient virtual try-on simulation. There were two fundamental processes: it first applied global body-shape-dependent deformations to the garment and then predicted dynamic wrinkle deformations based on the body shape and posture. Further, Wang~\emph{et al.}~\cite{wang2019acmtog} introduced a semi-automatic method for authoring garment animation, which first encoded essential information of the garment shape and based on the intrinsic garment representation and target body motion, it learned to reconstruct garment shape with physical properties automatically. Based only on a single-view image, Yang~\emph{et al.}~\cite{yang:iccv2017} proposed a method to recover a 3D mesh of garment with the 2D physical deformations. Given a single-view image, a human-body database, and a garment-template database as input, it first preprocessed with garment parsing, human body reconstruction, and features estimation. Then, it synthesized the initial garment registration and garment parameter identification for reconstructing body and clothing models with physical properties. Besides, Yu~\emph{et al.}~\cite{yu2019cvpr} enhanced the simulation performance with a two-step model called SimulCap, which combined the benefits of capture and physical simulation. The first step aimed to get a multi-layer avatar via double-layer reconstruction and multi-layer avatar generation. Then, it captured the human performance by body tracking and cloth tracking for simulating the physical clothing-body interactions.

%Notably, these approaches require plenty of manual labor and high computational complexity to collect necessary information for building 3D models. With the drastic advances of deep learning, there has been a growing interest in learning generative image models directly from data. 

\subsubsection{Benchmark datasets}
Datasets for physical simulation are different from other fashion tasks since the physical simulation is more related to computer graphics than computer vision. Here, we discuss the types of input data used by most physical simulation works. Physical simulation working within the fashion domain focus on clothing-body interactions, and datasets can be categorized into real data and created data. For an example of real data, for each type of clothing,% L{\"{a}}hner~\emph{et al.}
~\cite{Zorah2018DeepWrinkles} captured 4D scan sequences at 60 fps %of a subject 
in motion and dressed in a full-body suit. As for created data,% Santesteban~\emph{et al.}
~\cite{Santesteban2019cgf} was based on one garment to create dressed character animations with diverse motions and body shapes, and it can be applied to other garments.

\begin{table*}[t!]
\scriptsize
\center
\caption{Summary of the benchmark datasets for physical simulation task.}
\vspace{-3mm}     
\begin{tabular}{c|c|c|c|c}
  \Xhline{1.0pt}
   Dataset name & \makecell{Publish\\time} & \makecell{\# of\\ photos} & Key features & Sources\\
   \hline
    \makecell[l]{{DeepWrinkles}~\cite{Zorah2018DeepWrinkles}} & 2018 & 9,213 & \makecell[l]{ Each image contains a colored mesh with 200K vertices.} & \makecell[l]{N/A}\\
  \hline 
    \makecell[l]{Santesteban~\emph{et al.}~\cite{Santesteban2019cgf}} & 2019 & 7,117 & \makecell[l]{It was simulated with 17 body shapes with only one garment.} & \makecell[l]{SMPL}\\
  \hline 
    \makecell[l]{\href{https://virtualhumans.mpi-inf.mpg.de/mgn/}{MGN}~\cite{mgn2019iccv}} & 2019 & N/A & \makecell[l]{It contains 356 3D scans of people with different body shapes, poses\\ and in diverse clothing.} & \makecell[l]{SMPL+G}\\
  \hline
    {\makecell[l]{\href{https://renderpeople.com/ 3d- people.}{RenderPeople}}} & 2019 & N/A & \makecell[l]{It consists of 500 high-resolution photogrammetry scans.\\ It was used by PIFu~\cite{pifu2019iccv,pifuHD2020cvpr} and ARCH~\cite{arch2020cvpr}} & \makecell[l]{RenderPeople}\\
  \hline
    {\makecell[l]{\href{https://kv2000.github.io/2020/03/25/deepFashion3DRevisited/}{DeepFashion3D}~\cite{deepfashion3d2020eccv}}} & 2020 & N/A & \makecell[l]{It contains 2,078 3D garment models with 10 different clothing\\ categories and 563 garment instances.} & \makecell[l]{Reconstructed from\\real garments}\\
  \hline
    {\makecell[l]{\href{https://github.com/zycliao/TailorNet_dataset}{TailorNet}~\cite{tailornet2020cvpr}}} & 2020 & 55,800 & \makecell[l]{It contains 20 aligned real static garments with 1,782 different poses\\ and 9 body shapes.} & \makecell[l]{Simulated by the\\ Marvelous Designer }\\
  \hline
    {\makecell[l]{\href{https://virtualhumans.mpi-inf.mpg.de/sizer/}{Sizer}~\cite{sizer2020eccv}}} & 2020 & N/A & \makecell[l]{It includes 100 different subjects with 10 casual clothing classes in\\ various sizes in total of over 2,000 scans.} & \makecell[l]{self-collected}\\
  \Xhline{1.0pt}
\end{tabular}
    \begin{tablenotes}
      \scriptsize
      \item N/A: there is no reported information to cite. M means million.
    \end{tablenotes}
\label{table:physical simulation_dataset}
\end{table*}


\subsubsection{Performance comparison}
There are limited quantitative comparisons between physical simulation works. Most of them tend to calculate the qualitative results only within their work (e.g., per-vertex mean error% between groundtruth and generated result
) or show the vision comparison with state-of-the-art methods. Take the comparison done by% Santesteban~\emph{et al.}
~\cite{Santesteban2019cgf} for example in Fig.~\ref{fig:physical_simulation_comparsion}.

\begin{figure}[t!]
  \centering
  %\vspace{-3mm}
  \includegraphics[width=\linewidth]{img/physical_simulation_comparison_1.png}\\
  \vspace{-4mm}
  \caption{Left comparison is between DRAPE~\cite{guan:tog2012} and Santesteban~\emph{et al.}~\cite{Santesteban2019cgf}, while the right one compares between ClothCap~\cite{pons-moll:tog2017} and~\cite{Santesteban2019cgf}. Both are given a source and simulate the physical clothing deformation in different body shapes.}
  \vspace{-5mm}
  \label{fig:physical_simulation_comparsion}
\end{figure}


%-------------------------------------------------

%\textbf{Other Conditional Fashion Synthesis.}
%There are many other interesting conditional fashion synthesis, as presented in Fig.~\ref{fig:other_fashion_synthesis}, providing useful tools for further fashion applications. 


%\begin{figure}[ht]
%  \centering
%  \subfigure[Fashion generation from text (FashionGAN~\cite{zhu2017your}).]
%  {
%  \includegraphics[width=0.8\linewidth]{img/fashiongan.pdf}}
%  \subfigure[A generative model of people in clothing~\cite{lassner2017generative}.]
%  {
%  \includegraphics[width=0.45\linewidth]{img/generative_model_clothing.pdf}}
%  \subfigure[Fashion style generator~\cite{jiang2017fashion}.]
%  {
%  \includegraphics[width=0.45\linewidth]{img/fashion_style_generator.pdf}}
%  \caption{\textcolor{red}{Other conditional fashion synthesis.}}
%  \label{fig:other_fashion_synthesis}
%\end{figure}

%\begin{figure}[t!]
%  \centering
%  \subfigure[Fashion style generator~\cite{jiang2017fashion}.]
%  {\includegraphics[width=0.3\linewidth]{img/fashion_style_generator.png}}~~~~~~~~
%  \subfigure[People in clothing generator~\cite{lassner2017generative}.]
%  {\includegraphics[width=0.24\linewidth]{img/generative_model_clothing.png}}~~~~~~~~
%    \subfigure[Fashion generation from text \cite{zhu2017your}.]
%  {\includegraphics[width=0.45\linewidth]{img/fashiongan.png}}
%  \vspace{-2mm}
%  \caption{Other conditional fashion synthesis.}
%  \label{fig:other_fashion_synthesis}
%\end{figure}


%\subsubsection{Benchmark datasets}
%\subsubsection{Performance evaluations}




==> ACMCSUR – Fashion/src/introduction.tex <==
\section{Introduction}
\label{sec:intro}

Fashion is how we present ourselves to the
world. The way we dress and makeup defines our unique style and distinguishes us from other people. Fashion in modern society has become an indispensable part of who I am. Unsurprisingly, the global fashion apparel market alone has surpassed 3 trillion US dollars today, and accounts for nearly 2 percent of the world's Gross Domestic Product (GDP)\footnote{\url{https://fashionunited.com/global-fashion-industry-statistics/}}. Specifically, revenue in the Fashion segment amounts to over US \$718 billion in 2020 and is expected to present an annual growth of 8.4\%\footnote{\url{https://www.statista.com/outlook/244/100/fashion/worldwide}}.

As the revolution of computer vision with artificial intelligence (AI) is underway, AI is starting to hit the magnanimous field of fashion, whereby reshaping our fashion life with a wide range of application innovations from electronic retailing, personalized stylist, to the fashion design process. In this paper, we term the computer-vision-enabled fashion technology as intelligent fashion. Technically, intelligent fashion is a challenging task because, unlike generic objects, fashion items suffer from significant variations in style and design, and, most importantly, the long-standing semantic gap between computable low-level features %(\textit{e.g.}, visual, audio, and textual features) 
and high-level semantic concepts that they encode is huge.

There are few previous works~\cite{liu:mmmag2014, Song2018fashion} related to short fashion surveys. In 2014, Liu~\emph{et al.}~\cite{liu:mmmag2014} presented an initial literature survey focused on intelligent fashion analysis with facial beauty and clothing analysis, which introduced the representative works published during 2006--2013. However, thanks to the rapid development of computer vision, there are far more than these two domains within intelligent fashion, e.g., style transfer, physical simulation, fashion prediction. There have been a lot of related works needed to be updated. In 2018, Song and Mei~\cite{Song2018fashion} introduced the progress in fashion research with multimedia, which categorized the fashion tasks into three aspects: low-level pixel computation, mid-level fashion understanding, and high-level fashion analysis. Low-level pixel computation aims to generate pixel-level labels on the image, such as human segmentation, landmark detection, and human pose estimation. Mid-level fashion understanding aims to recognize fashion images, such as fashion items and fashion styles. High-level fashion analysis includes recommendation, fashion synthesis, and fashion trend prediction. However, there is still a lack of a systematic and comprehensive survey to paint the whole picture of intelligent fashion so as to summarize and classify state-of-the-art methods, discuss datasets and evaluation metrics, and provide insights for future research directions. 


\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{img/c3.jpg}
  \caption{Scope of the intelligent fashion research topics covered in this survey paper.}
  \setlength{\belowcaptionskip}{-80pt}
  \label{fig:overview}
\end{figure}

Current studies on intelligent fashion covers the research topics not only to detect what fashion items are presented in an image but also analyze the items, synthesize creative new ones, and finally provide personalized recommendations. Thus, in this paper, we organize the research topics accordingly, as categorized in Fig.~\ref{fig:overview}, which includes fashion image detection, analysis, synthesis, and recommendation. In addition, we also give an overview of main applications in the fashion domain, showing the power of intelligent fashion in the fashion industry. Overall, the contributions of our work can be summarized as follows:
\begin{itemize}
  \item We provide a comprehensive survey of the current state-of-the-art research progress in the fashion domain and categorize fashion research topics into four main categories: detection, analysis, synthesis, and recommendation.
  \item For each category in the intelligent fashion research, we provide an in-depth and organized review of the most significant methods and their contributions. Also, we summarize the benchmark datasets as well as the links to the corresponding online portals.
  \item We gather evaluation metrics for different problems and also give performance comparisons for different methods.
  \item We list possible future directions that would help upcoming advances and inspire the research community.
\end{itemize}

This survey is organized in the following sections. Sec.~\ref{sec:fffashion_detection} reviews the fashion detection tasks including landmark detection, fashion parsing, and item retrieval. Sec.~\ref{sec:fffashion_analysis} illustrates the works for fashion analysis containing attribute recognition, style learning, and popularity prediction. Sec.~\ref{sec:fffashion_synthesis} provides an overview of fashion synthesis tasks comprising style transfer, human pose transformation, and physical texture simulation. Sec.~\ref{sec:fffashion_recommendation} talks about works of fashion recommendation involving fashion compatibility, outfit matching, and hairstyle suggestion. Besides, Sec.~\ref{sec:application} demonstrates selected  applications and future work. Last but not least, concluding remarks are given in Sec.~\ref{sec:conclusion}.

%fffashion detection
%In Sec.~\ref{sec:understand_fashion}, we review the methods for understanding fashion images, mainly focusing on low-level approaches towards computational fashion, including landmark detection, attribute prediction, and semantic segmentation. 

%fffashion synthesis
%In Sec.~\ref{sec:fashion_synthesis}, an overview of fashion synthesis methods is given, to show how clothing design and facial beautification processes can be fueled with computer vision and multimedia technologies. 

%fffashion recommendation
%In Sec.~\ref{sec:recommendation}, fashion recommendation methods are discussed, taking a further step to practical fashion applications. 

%fffashion analysis
%Besides, Sec.~\ref{sec:fashion_analysis} illustrates the methods for fashion analysis, Sec.~\ref{sec:application} demonstrates some existing fashion applications and future work. Concluding remarks are given in Sec.~\ref{sec:conclusion}.

%Fashion related research has many open challenges awaiting to be tackled. Various attempts have already been made to unveil fashion code from various perspectives, including xxx...


==> ACMCSUR – Fashion/src/recommendation.tex <==
\section{Recommendation}
\label{sec:recommendation}

Fashion recommendation has attracted increasing attention given its ready applications to online shopping for fashion products. Relevant literature on the research progress of fashion recommendation falls into four main categories, \textit{i.e.}, outfit matching, fashion item retrieval, style classification, and hairstyle suggestion.

\subsection{Outfit Matching}

Each outfit generally involves multiple complementary items, such as tops, bottoms, shoes, and accessories. A key to a stylish outfit lies in the matching fashion items, as illustrated in Fig.~\ref{fig:outfit_matching_example}. However, generating harmonious fashion matching is challenging due to three main reasons. First, a fashion concept is often subtle and subjective. Second, there are a large number of attributes for describing fashion. Third, the notion of fashion item compatibility generally goes across categories and involves complex many-to-many relationships. In the past several years, this problem has attracted a great deal of interest, resulting in a long list of algorithms and techniques. %In the following, we review the current state-of-the-art of recommendation method for outfit matching.


\begin{figure}[t!]
  \centering
  \includegraphics[width=0.8\linewidth]{img/outfit_matching_hsiaoCVPR2018.png}
  \caption{Examples of outfit matching task~\cite{hsiao2018creating}.}
  \label{fig:outfit_matching_example}
\end{figure}


\subsubsection{State-of-the-art methods}

Fashion recommendation for outfit matching was initially introduced by Iwata~\emph{et al.}~\cite{iwata:ijcai2011}. They proposed a probabilistic topic model for learning information about fashion coordinates. Liu~\emph{et al.}~\cite{liu:mm2012} further adopted middle-level clothing attributes (\textit{e.g.}, clothing category, color, pattern) to learn the clothing recommendation model through a unified latent Support Vector Machine (SVM) framework. 

Inspired by the advances of deep learning technique, most of the current researchers have put efforts in modeling the style compatibility based on the data-driven deep learning approaches. Veit~\emph{et al.}~\cite{veit:iccv2015} utilized the co-purchase data from Amazon.com to train a Siamese Convolutional Neural Network (CNN) to learn style compatibility across categories. The study in~\cite{mcauley:sigir2015} modeled human preference to uncover the relationships between the appearances of pairs of items by Low-rank Mahalanobis Transform that mapped compatible items to embeddings close in the latent space. He and McAuley~\cite{he:aaai2016} later extended the work of~\cite{mcauley:sigir2015} by combining visual and historical user feedback data. The proposed study incorporates visual signals into Bayesian Personalized Ranking with Matrix Factorization as the underlying predictor. 

A line with~\cite{veit:iccv2015, mcauley:sigir2015, he:aaai2016} that aim to model item-to-item recommendation based on co-purchasing behaviour, \cite{he:icdm2016} proposed to relax the identity and symmetry assumptions inherent in metric-based recommendation methods \cite{veit:iccv2015, mcauley:sigir2015, he:aaai2016}. The \textit{Mixtures of Non-Metric Embeddings for Recommendation} framework allows \cite{he:icdm2016} to learn multiple notions of relatedness to compete and interact. Later, Veit~\emph{et al.} introduced Conditional Similarity Networks (CSNs) \cite{AVeit2017CVPR}, which learns nonlinear feature embeddings that incorporate multiple notions of similarity within a shared embedding using a shared feature extractor. The CSNs address the issue of a standard triplet embedding that treats all triplet equally and ignores the sources of similarity. In~\cite{hu:mm2015}, Hu~\emph{et al.} addressed the personalized issue by utilizing a functional tensor factorization method to model the user-item and item-item interactions. 

In particular, previous studies mainly focus on visual information but fail to consider the contextual factors. To bridge this gap, Song~\emph{et al.}~\cite{song2017neurostylist} integrated visual and contextual modalities of fashion items by employing the autoencoder neural model to seek the non-linear latent compatibility space. Following this work,~\cite{song:sigir2018} integrated fashion domain knowledge to the neural networks to boost the compatibility modeling performance. 

Most previous works~\cite{iwata:ijcai2011, liu:mm2012,  song2017neurostylist,song:sigir2018} mainly focused on top-bottom matching. However, an outfit generally includes more items, such as shoes, bags, \emph{etc}. To address this issue, Chen and He~\cite{chen2018dress} extent traditional triplet neural network, which usually receives three instances, to accept multiple instances. A mixed-category metric learning method is proposed to adapt the multiple inputs. The similar idea is also employed in~\cite{shih2018compatibility}, where the metric learning is combined with generative neural networks. The proposed generator, referred to as Metric-regularized Conditional Generative Adversarial Network (MrCGAN), is regularized by a projected compatibility distance (PCD) function. It ensures the compatible items are closer in the learned space compared to the incompatible ones. %\textcolor{red}{Given the image of a query item, the well-trained MrCGAN is able to generate an image of a compatible item.}

Other methods designed the end-to-end frameworks for outfit matching. Li \emph{et al.}~\cite{YLi2017TMM} formulated the problem as a classification task, where a given outfit composition is labeled as a popular or unpopular one. They designed a multi-modal multi-instance model based on convolutional neural networks that exploited images and meta-data of fashion items, and information across fashion items. In~\cite{han2017learning}, an end-to-end model is built based on bidirectional LSTM (Bi-LSTM). Specifically, inspired by image captioning of~\cite{donahue2015long}, Han~\emph{et al.} treated an outfit as a sequence of fashion items and each item in the outfit as a time step. A Bi-LSTM model is then utilized to predict the next item conditioned on previously seen ones, where the objective is to maximize the total probability of the given positive sequence. The model is able to achieve three tasks, \emph{i.e.}, fill-in-the-blank (fashion item recommendation given an existing set), outfit generation conditioned on users' text/image inputs, and outfit compatibility prediction. Another work~\cite{hsiao2018creating} also borrowed the idea from natural language processing. That is, an outfit is regarded as a ``document'', an inferred clothing attribute is regarded as a ``word'', and a clothing style is the ``topic''. The problem of outfit matching is formulated with the topic model. The combinations similar to previously assembled outfits should have a higher probability, which can be employed as the prediction for compatibility, and then solve the outfit matching problem. In~\cite{vasileva:eccv2018}, Vasileva~\emph{et al.} presented an approach to learning an image embedding that respects item type. They first learned a single, shared embedding space to measure item similarity, then projected from that shared embedding to subspaces identified by type.

More recently, Kang~\emph{et al.}~\cite{kang:cvpr2019} introduced ``Complete the Look'' task aiming at recommending fashion items that complement (or \textit{go well with}) the given scene. The comparison of the use-cases of product-based and the ``complete the look'' scene-based complementary recommendation is shown in Fig.~\ref{fig:outfit_matching_completeTheLook}. To achieve this task, \cite{kang:cvpr2019} measured both global compatibility (\textit{i.e.}, the compatibility between the scene and product images) and local compatibility (\textit{i.e.}, the compatibility between every scene patch and product image) via Siamese networks and category-guided attention mechanisms.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.85\linewidth]{img/outfit_matching_kangCVPR2019.png}
  \caption{A comparison of product-based complementary recommendation (top) and ``complete the look'' scene-based complementary recommendation (bottom).}
  \label{fig:outfit_matching_completeTheLook}
\end{figure}



%a popular fashion website, where users create and upload outfit data as shown in Figure 3.

\subsubsection{Benchmark datasets}

Since different papers are under various settings and most of the datasets for outfit matching are not publicly available, almost every paper for outfit  matching  collected their own dataset. The datasets were collected  from social media platforms where users can create their own outfits, such as Polyvore.com. We list the benchmark datasets for outfit matching in Table~\ref{tab:outfit_matching_datasets}. Note that the outfit database in~\cite{mcauley:sigir2015, he:aaai2016, hu:mm2015, song2017neurostylist, YLi2017TMM, han2017learning, hsiao2018creating, vasileva:eccv2018, kang:cvpr2019} comprises the images of each single item, while in~\cite{iwata:ijcai2011, liu:mm2012, chen2018dress}, an outfit is in a single image.

\begin{table*}[htbp]
\footnotesize
    \centering
        \caption{Summary of the benchmark datasets for outfit matching task.}
        \vspace{-3mm}
    \begin{tabular}{c|c|c|c|c|c}
    \Xhline{1.0pt}
      \makecell{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ outfits} & \makecell{\# of\\ items} & Key features & Sources \\
     \hline
        \makecell[l]{Iwata~\emph{et al.}~\cite{iwata:ijcai2011}} & 2011 & 14,813 & 5 &   \makecell[l]{Full-body fashion model} & \makecell[l]{Magazine, Chicisimo.com,\\ and Weardrobe.ie}\\ %clothes, bags, shoes, cosmetics, accessories
    \hline
        \makecell[l]{What-to-Wear~\cite{liu:mm2012}} & 2012 & 24,417 & 2 &  \makecell[l]{Annotated with full-body, upper-body, or lower-body} & \makecell[l]{Online shopping and photo\\ sharing sites}\\
    \hline
        \makecell[l]{Styles and Substitutes\\\cite{mcauley:sigir2015}} & 2015 & 773,465 & N/A & \makecell[l]{Annotated with 4 categories of relationship: (1) users who view-\\ed X also viewed Y, (2) users who viewed X eventually bought\\ Y, (3) users who bought X also bought Y, and (4) users bought\\ X and Y simultaneously} & \makecell[l]{Amazon.com}\\
    \hline
        \makecell[l]{Hu~\emph{et al.}~\cite{hu:mm2015}} & 2015 & 28,417 & 3 & \makecell[l]{Annotated with categories, names, and descriptions} & \makecell[l]{Polyvore.com}\\
    \hline
        \makecell[l]{He~\emph{et al.}~\cite{he:aaai2016}} & 2016 & 598.353 & N/A & \makecell[l]{Annotated with users' review histories} & \makecell[l]{Amazon.com, Tradesy.com}\\
    \hline 
        \makecell[l]{Song~\emph{et al.}~\cite{song2017neurostylist}} & 2017 & 20,726 & 2 & \makecell[l]{Annotated with title, category, and description} & \makecell[l]{Polyvore.com} \\
    \hline
        \makecell[l]{Li~\emph{et al.}~\cite{YLi2017TMM}} & 2017 & 195,262 & 4 & \makecell[l]{Annotated with\ title, category, and number of likes} & \makecell[l]{Polyvore.com} \\
    \hline 
        \makecell[l]{Han~\emph{et al.}~\cite{han2017learning}} & 2017 & 21,889 & 8 & \makecell[l]{Each item contains a pair -- product image and a corresponding\\ text description} & \makecell[l]{Polyvore.com} \\
    \hline
        \makecell[l]{Hsiao~\emph{et al.}~\cite{hsiao2018creating}} & 2018 & 3,759 & $\geq 2$ & \makecell[l]{Annotated with meta-labels, \emph{e.g.}, season (winter, spring, sum-\\mer, fall), occasion (work, vacation), and function (date, hike)} & \makecell[l]{Polyvore.com} \\
    \hline
        \makecell[l]{Vasileva~\emph{et al.}\tablefootnote{\url{https://github.com/mvasil/fashion-compatibility}}~\cite{vasileva:eccv2018}} & 2018 & 68,306 & 19 & \makecell[l]{Annotated with outfit and item ID, fine-grained item type,\\ title, and text descriptions} & \makecell[l]{Polyvore.com} \\
    \hline
        \makecell[l]{Fashion Collocation\\\cite{chen2018dress}} & 2018 & 220,000 & 5 & \makecell[l]{Annotated with independent and ready for wearing (off-body\\ module) or dependent (on-body module), or a bounding box} & \makecell[l]{Chictopia.com, Wear.net,\\ and FashionBeans.com} \\
    \hline
        \makecell[l]{Pinterest's Shop\\The Look~\cite{kang:cvpr2019}} & 2019 & 38,111 & 10 & \makecell[l]{Annotated with category} & \makecell[l]{Pinterest.com}\\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:outfit_matching_datasets}
    \begin{tablenotes}
      \scriptsize
      \item N/A: there is no reported information to cite.
    \end{tablenotes}
\end{table*}

\subsubsection{Performance evaluations}

Area Under the ROC curve (AUC) is the evaluation for most of outfit matching methods~\cite{he:aaai2016, veit:iccv2015, song2017neurostylist, song:sigir2018, shih2018compatibility, YLi2017TMM, han2017learning, vasileva:eccv2018}. Some methods are evaluated with Normalized Discounted Cumulative Gain (NDCG)(\textit{i.e.}, \cite{liu:mm2012, hu:mm2015}), prediction accuracy (\textit{i.e.}, \cite{iwata:ijcai2011, hsiao2018creating, mcauley:sigir2015, han2017learning, vasileva:eccv2018, kang:cvpr2019}), recall$@k$ (\textit{i.e.}, \cite{chen2018dress}), or Average Precision (\textit{i.e.}, \cite{YLi2017TMM}). Unfortunately, there is no unified benchmark for outfit matching, both in datasets and evaluation metrics. Therefore, we are unable to give a comparison of different methods.

%~\cite{iwata:ijcai2011}: The similarity evaluation measurement, which calculated as the average similarity between the recommended clothing and the held-out paired clothing.

\subsection{Fashion Image Retrieval}

As fashion e-commerce has grown over the years, there has been high demand for innovative solutions to help customers find preferred fashion items with ease. Though fashion many fashion online shopping sites support keyword-based searches, there are many visual traits of fashion items that are not easily translated into words. It thus attracts tremendous attention from many research communities to develop intelligent image-based fashion retrieval. Given a fashion image query, the goal of image-based fashion retrieval is to find  similar or identical items from the gallery. 


\subsubsection{State-of-the-art methods}

The notable early work on automatic image-based clothing retrieval was presented by Wang and Zhang~\cite{wang2011clothes}. They used dominant color patches to obtain the initial search results and then re-ranked these results using attribute information of clothes learned through least-squares posterior classifier (LSPC)~\cite{sugiyama:iecetis2010}.

To date, extensive research studies have been devoted to addressing the problem of cross-scenario clothing retrieval since there is a large domain discrepancy between daily human photo captured in general environment and clothing images taken in ideal conditions (\textit{i.e.}, embellished photos used in online clothing shops). %The illustration of cross-scenario clothing retrieval is presented in Fig.~\ref{fig:clothing_retrieval_street2shop}. 
In~\cite{liu2012street}, Liu~\emph{et al.} proposed to utilize an unsupervised transfer learning method based on part-based alignment and features derived from sparse reconstruction. Fu~\emph{et al.}~\cite{fu:accv2012} proposed a semantic-preserving visual phrases (SPVP) representation, which encodes the regions of human parts refined with sparse background reconstruction into the vocabulary tree under the bag-of-visual-word (BOW) framework. Kalantidis~\emph{et al.}~\cite{kalantidis:icmr2013} presented clothing retrieval in the perspective of human parsing. A prior probability map of the human body is obtained through pose estimation to guide clothing segmentation, and then the segments are classified through locality-sensitive hashing. The visually similar items are retrieved by summing up the overlap similarities. Chi~\emph{et al.} introduced Visual Part-based Object Representation (VPOR) framework~\cite{chi:mtap2016} that use partial visual appearances to obtain personalized item recommendation results. Conceptually, the VPOR decomposes every item image into a set of disjoint part, with each part represents a meaningful semantic part, then discovers auxiliary features through part-based feature propagation mechanism. The feature propagation can make two items that share a similar part but are different in the rest parts become more similar for improving the relevance of recommended results. Notably,~\cite{wang2011clothes, liu2012street, fu:accv2012, kalantidis:icmr2013, chi:mtap2016} are based on hand-crafted features.

%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=0.45\linewidth]{img/clothing_retrieval_street2shop.png}
%  \caption{\textcolor{red}{An illustration of cross-scenario clothing retrieval model.}}
%  \label{fig:clothing_retrieval_street2shop}
%\end{figure}

%Early works on image-based clothing retrieval are mostly based on hand designed features~\cite{wang2011clothes, liu2012street, fu:accv2012, kalantidis:icmr2013, kovashka:cvpr2012, kovashka:ijcv2015, li:viscomput2016}.

With the advances of deep learning, there has been a trend of building deep neural network architectures to solve the clothing retrieval task. Huang~\emph{et al.}~\cite{huang:mm2014} developed an attribute-aware clothing retrieval system using a holistic tree-structure convolutional neural network that integrates multiple clothing attributes simultaneously. Later, in~\cite{huang2015cross} they exploited the richness of the data obtained by mining images from customer review websites where the customers post photos of the clothing they have purchased. They introduced a Dual Attribute-aware Ranking Network (DARN), two sub-networks with similar structure, one for each domain, to represent deep features using attribute-guided learning. DARN simultaneously embeds semantic attributes and visual similarity constraints into the feature learning stage, while at the same time modeling the discrepancy between domains. Liang~\emph{et al.}~\cite{XLiang2016TMM} incorporated clothing parsing into clothing retrieval. Given a query clothing image, they first parse this query into fine-grained semantic regions by the proposed clothes co-parsing framework formulated as a probabilistic model, then retrieve clothing items from online shopping images. Li~\emph{et al.}~\cite{li:icpr2016} presented a hierarchical superpixel fusion strategy and a sparse coding-based attribute recognition. More explicitly, an over-segmentation hierarchical fusion algorithm with human pose estimation is utilized to get query clothing item and to retrieve similar images from product clothing dataset. To improve the accuracy of the classifiers and the adaptability of the dictionary for recognizing clothing styles in different scenarios, the intermediate domain dictionaries between product clothing dataset and daily clothing dataset are learned sequentially during the recognition phase. A personalized clothing recommendation system, namely i-Stylist, that retrieves clothing items through the analysis of user's own images is developed in \cite{sanchez-riera:mmm2017}. The i-Stylist organizes the visual information and semantic information (clothing properties) of user's clothing items as a fully connected graph. The user's personalized graph model later derives the probability distribution of the likability of an item in shopping website.

The studies in~\cite{wang2011clothes, liu2012street, fu:accv2012, kalantidis:icmr2013, huang:mm2014, huang2015cross, chi:mtap2016, li:icpr2016, sanchez-riera:mmm2017} are designed for similar retrieval. But more often, people desire to find exactly the same clothing item, as illustrated in Fig.~\ref{fig:clothing_retrieval_exactRetrieval}. The first attempt on this task was achieved by Kiapour~\emph{et al.}~\cite{kiapour:iccv2015} who evaluated some existing deep learning feature-based retrieval and similarity learning methods. Wang~\emph{et al.}\cite{wang:icmr2016} adopted a Siamese network that contains two copies of the Inception-6 network with shared weights. They introduced a \textit{robust contrastive loss} to alleviate over-fitting caused by some positive pairs (containing the same product) that are visually different, and a multi-task fine-tuning approach to learning feature representation with a softmax loss for improved results. Jiang~\emph{et al.} learned the discrepancy between street domain and shop domain clothing with a deep bi-directional cross-triplet embedding based on convolutional neural network \cite{jiang:mm2016}, and further expanded the utilization of this approach to retrieve a series of representative and complementary accessories (\textit{e.g.}, bags, shoes) to pair with the shop item~\cite{jiang:tomm2018}. Cheng~\emph{et al.}~\cite{ZQCheng2017CVPR} explored the exact matching clothes in videos to online shopping images. The videos and online shopping images are first encoded by a Long Short-Term Memory (LSTM) network and convolutional neural network, respectively, then are fed into the similarity network for pair-wise matching. Garcia~\emph{et al.}\cite{garcia:iccvw2017} proposed to relate clothing items and video frames in an indexed database and performed frame retrieval with temporal aggregation.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.5\linewidth]{img/clothing_retrieval_exactRetrieval.png}
  \caption{An illustration of exact clothing retrieval~\cite{kiapour:iccv2015}.}
  \label{fig:clothing_retrieval_exactRetrieval}
\end{figure}

In the clothing retrieval methods described above, the search is only based on query images that reflect users' needs, without considering that users may want to provide extra keywords to describe the desired attributes that are absent in the query image. Towards this goal, Kovashka~\emph{et al.} developed the WhittleSearch~\cite{kovashka:cvpr2012, kovashka:ijcv2015} that allows the user to upload a query image and provide additional relative attribute description as feedback for refining the image search results in an iterative manner (see Fig.~\ref{fig:clothing_retrieval_interactiveSearch}). This approach extends the class-based training procedure used in \cite{parikh:iccv2011} to incorporate image-level relative comparisons. In~\cite{li:viscomput2016}, Li~\emph{et al.} incorporated the relevant feedback approach into the optimum-path Forest classifier to enable users to search the clothing items of preferred collar design. Several traditional-based feature extraction methods are proposed to capture three kinds of collar designs -- collar spread, turnover, and front designs.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.95\linewidth]{img/clothing_retrieval_interactiveSearch.png}
  \caption{An example of interactive fashion search~\cite{kovashka:cvpr2012}.}
  \label{fig:clothing_retrieval_interactiveSearch}
\end{figure}

Unlike previous \textit{interactive fashion search} approaches that the user cannot change the attribute from one to another easily~\cite{kovashka:cvpr2012, kovashka:ijcv2015} or are designed for a specific attribute~\cite{li:viscomput2016}, the memory-augmented Attribute Manipulation Network (AMNet)~\cite{zhao:cvpr2017} is capable of manipulating image representation at the attribute level. Given a query image and attribute manipulation request, such as ``\textit{I want to buy a jacket that looks like this query image, but with blue color instead of pink and plush collar instead of round collar},'' AMNet updates the query representation encoding the unwanted attributes and replace them to the desired ones. The manipulated representation is then used to retrieve images with desired attributes from the gallery. Later, Ak~\emph{et al.}~\cite{ak:wacv2018, ak:patternrecogletter2018, ak:cvpr2018} explored the localization aspect of attribute representations to facilitate region-specific attribute manipulation requests. In particular, \cite{ak:wacv2018} estimated clothing item parts using an unsupervised segmentation method and applied CNN with part-based triplet ranking constraint as an attention mechanism.~\cite{ak:patternrecogletter2018} introduced ``Part Guided CNN'', a Convolutional Neural Network (CNN) controlled by constituent parts of clothing items, to conduct learning of the respective attributes of clothing parts. A Markov Random Field based color encoding method is adopted to generate specific color descriptions.~\cite{ak:cvpr2018} presented the FashionSearchNet to learn regions and region-specific attribute representations by exploiting the attribute activation maps (AAMs) generated by global average pooling (GAP) layer. %Fig.~\ref{fig:clothing_retrieval_pipelines}(c) presents an overview of the proposed framework in~\cite{ak:cvpr2018}.

In~\cite{laenen:wsdm2018}, Laenen~\emph{et al.} built a multimodal retrieval model that uses a combination of an image and text as a query and ranks the image results based on their semantic similarity to the query text and their visual similarity to the query image. Different from~\cite{zhao:cvpr2017, ak:wacv2018, ak:patternrecogletter2018, ak:cvpr2018} that used neural networks to construct visual representation of searched item by manipulating the visual representation of query image with the textual attributes in query text, \cite{laenen:wsdm2018} used neural network to infer the semantic relationship between visual and textual attributes in a joint multimodal embedding space. To help facilitate the reasoning of search results and user intent, Liao~\emph{et al.}~\cite{liao:mm2018} built EI (Exclusive and Independent) tree that captures hierarchical structures of the fashion concepts. The EI Tree is generated by  incorporating product hierarchies of online shopping websites and domain knowledge of fashion experts. The generated EI tree is then applied to guide the end-to-end deep learning procedure, mapping the implicit deep features to explicit fashion concepts.

Different problem is tackled in the fashion retrieval literature. Gu~\emph{et al.}~\cite{gu:icmr2015} presented a cross-scenario eyeglasses retrieval system, namely Fashion Glasses Search System (FGSS). They introduced a keypoint-based scheme called \textit{EyeGlass keYPoinT} (EGYPT) to describe the appearances of glasses, making FGSS free from segmentation problems. In the EGYPT, hybrid feature descriptors that combine shape, color, and texture features extracted from the detected keypoints are exploited to form a representative feature vector. Gu~\emph{et al.} later developed iGlasses~\cite{gu:sigir2016}, a recommendation for best-fits glasses that exploits the implicit matching rules between human faces and eyeglasses. Given a frontal face photo as the input, the iGlasses captures the correlation among the fine-grained attributes of human faces and frames of glasses, and then returns a ranked list of candidate eyeglasses. It further produces a synthesized image for the input face to demonstrate the visual effect when wearing the recommended glasses. 

The studies in~\cite{wang:icip2014, wang:tmm2016, wang:tmm2015} dealt with handbag recognition problems. In particular, Wang~\emph{et al.}~\cite{wang:icip2014} introduced a complementary feature obtained by extracting low-level features from a structure enhanced handbag image to compensate the missing details of the feature, called original feature, extracted directly from the original handbag image. The complementary feature is then fused with the original feature for the recognition. \cite{wang:tmm2016} further extended~\cite{wang:icip2014} by utilizing color model based on dominant color naming features. A CNN-based model for end-to-end framework to recognize the handbag models is presented in~\cite{wang:tmm2015}. It proposed feature selective joint classification regression CNN (FSCR-CNN) classification model, which consists of Feature Selective CNN and joint Classification-Regression CNN, to attenuate the illumination changes and inter-class similarity among handbags. The scores from FSCR-CNN classification model and CNN detection model are further eventually combined by a conditional probability model to recognize the handbag. 

Other than fashion image retrieval studies mentioned above, Vittayakorn \emph{et al.}~\cite{vittayakorn:wacv2015} learned human based judgments of outfit similarity. They employed a linear SVM for pairwise comparison of clothing outfits based on a learned combination of features computed over parsed clothing regions. In \cite{semertzidis:tist2016}, Semertzidis~\emph{et al.} designed and evaluated a crowd-powered system for visual fashion similarity search based on user-defined criteria. Different kinds of crowds, ranges from click workers for tedious tasks, such as cleaning content, to mobile fashion crowds, are integrated for this purpose.

%\begin{figure}
%  \centering
%  \subfigure[Wang and Zhang~\cite{wang2011clothes}.]
%  {\includegraphics[width=1\linewidth]{img/clothing_retrieval_wangMM2011.png}}

%  \subfigure[Deep Search~\cite{huang:mm2014}.]
%  {\includegraphics[width=0.9\linewidth]{img/clothing_retrieval_huangMM2014.png}}
  
%  \subfigure[FashionSearchNet~\cite{ak:cvpr2018}.]
%  {\includegraphics[width=1\linewidth]{img/clothing_retrieval_akCVPR2018.png}}

%  \subfigure[EI Tree~\cite{liao:mm2018}.]
%  {\includegraphics[width=1\linewidth]{img/clothing_retrieval_liaoMM2018.png}}
  %\vspace{-2mm}
%  \caption{Pipelines of state-of-the-art clothing retrieval methods.}
%  \label{fig:clothing_retrieval_pipelines}
%\end{figure}

\subsubsection{Benchmark datasets}

The existing clothing retrieval studies mainly focused on a cross-domain scenario. Therefore, most of the benchmark datasets were collected from daily photos and online clothing shopping websites. Table~\ref{tab:clothing_retrieval_datasets} gives a summary and link of the download page (if publicly available) of the benchmark datasets.% used to evaluate the fashion retrieval studies.


\begin{table*}[htbp]
\footnotesize
    \centering
        \caption{Summary of the benchmark datasets for fashion retrieval task.}
        \vspace{-3mm}
    \begin{tabular}{l|c|c|c|l|c}
    \Xhline{1.0pt}
        \multicolumn{2}{c|}{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ photos\\ (videos)}  & \makecell{Key features} & Sources \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{The Gallagher Collection Person\tablefootnote{\url{http://chenlab.ece.cornell.edu/people/Andy/projectpage_clothing.html}}~\cite{gallagher:cvpr2008}}} & 2008 & 589 & \makecell[l]{Annotated 1008 faces with 32 identities} & \makecell[l]{N/A}\\ 
    \hline
        \multirow{2}{*}{\makecell[l]{Liu~\emph{et al.}~\cite{liu2012street}}} & \makecell[l]{Online Shopping} & \multirow{2}{*}{2012} & 16,636 & \multirow{2}{*}{\makecell[l]{Each image consists of either upper- or lower-wear,\\ annotated with clothing-specific attributes}} & \makecell[l]{Online shopping sites}\\ 
        \cline{2-2}\cline{4-4}\cline{6-6}
        & \makecell[l]{Daily Photo} &  & 8,389 & & \makecell[l]{Flickr.com }\\ 
    \hline
        \multirow{2}{*}{\makecell[l]{Fu~\emph{et al.}~\cite{fu:accv2012}}} & \makecell[l]{Online Shopping} & \multirow{2}{*}{2012} & ~110,000 & \multirow{2}{*}{\makecell[l]{Each image consists of either upper- or lower-wear,\\ annotated with clothing-specific attributes}} & \makecell[l]{Amazon.com, eBay.com,\\ vancl.com, taobao.com}\\ 
        \cline{2-2}\cline{4-4}\cline{6-6}
        & \makecell[l]{Daily Photo} &  & \makecell{2,000} & & \makecell[l]{Flickr.com }\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Fashion-focused Creative Commons\\ Social\tablefootnote{\url{http://skuld.cs.umass.edu/traces/mmsys/2013/fashion/}}~\cite{loni:mmsys2013}}} & 2013 & 4,810 & \makecell[l]{Annotated with 154 fashion-focused categories (per-\\formed by crowdsourcing workers and trusted anno-\\tators), user-provided metadata, tags, favorites, com-\\ments, context, and note} & \makecell[l]{Flickr.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Chi~\emph{et al.}~\cite{chi:mtap2016}}} & 2016 & 23,854  & \makecell[l]{Annotated with 5 categories} & \makecell[l]{Amazon.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{UT-Zap50K shoe\tablefootnote{\url{http://vision.cs.utexas.edu/projects/finegrained/}}~\cite{yu:cvpr2014}}} & 2014 & 50,000  & \makecell[l]{Shoe images annotated with associated metadata\\ (shoe type, materials, manufacturer, gender, \emph{etc}.)} & \makecell[l]{Zappos.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Fashion 10000\tablefootnote{\url{http://skuld.cs.umass.edu/traces/mmsys/2014/user05.tar}}~\cite{loni:mmsys2014}}} & 2014 &  32,398 & \makecell[l]{Annotated with 470 fashion categories, associated\\ metadata, ground truth labels} & \makecell[l]{Flickr.com}\\ 
    \hline
        \multirow{2}{*}{\makecell[l]{Li~\emph{et al.}~\cite{li:icpr2016}}} & \makecell[l]{Product Clothing} & \multirow{2}{*}{2016} & 15,690 & \multirow{2}{*}{\makecell[l]{Annotated with clothing category}} & \makecell[l]{Online shopping sites}\\ 
        \cline{2-2}\cline{4-4}\cline{6-6}
        & \makecell[l]{Daily Clothing} &  & \makecell{4,206} & & \makecell[l]{Flickr.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{DARN~\cite{huang2015cross}}} & 2015 & 545,373 & \makecell[l]{Online-offline upper-clothing image pair, annotated\\ with clothing attribute categories} & \makecell[l]{Online-shopping sites\\ and corresponding customer\\ review pages}\\ 
    \hline
        \multirow{2}{*}{\makecell[l]{Exact Street2Shop\tablefootnote{http://www.tamaraberg.com/street2shop}\\\cite{kiapour:iccv2015}}} & \makecell[l]{Street photos} & \multirow{2}{*}{2015} & \makecell{20,357} & \multirow{2}{*}{\makecell[l]{39,479 pairs of exactly matching items worn in\\street photos and shown in shop photos}} & \makecell[l]{ModCloth.com}\\ 
    \cline{2-2}\cline{4-4}\cline{6-6}
         & \makecell[l]{Shop photos} & & 404,683 & & \makecell[l]{Online clothing retailers}\\ 
    \hline 
        \multicolumn{2}{c|}{\makecell[l]{MVC\tablefootnote{http://mvc-datasets.github.io/MVC/}~\cite{liu:icmr2016}}} & 2016 & 161,638 & Annotated with 264 attribute labels & \makecell[l]{Online shopping sites}\\ 
    \hline
        \multirow{2}{*}{\makecell[l]{Video2Shop\cite{ZQCheng2017CVPR}}} & \makecell[l]{Videos} & \multirow{2}{*}{2017} & \makecell{26,352\\(526)} & \multirow{2}{*}{\makecell[l]{39,479 exact matching pairs annotated with 14 cat-\\egories of clothes}} & \makecell[l]{Tmall MagicBox}\\ 
    \cline{2-2}\cline{4-4}\cline{6-6}
         & \makecell[l]{Online shopping} & & 85,677 & & \makecell[l]{Tmall.com, Taobao.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Shopping100k~\cite{ak:wacv2018}}} & 2018 & 101,021 & \makecell[l]{Annotated with 12 fashion attributes} & \makecell[l]{Online shopping sites}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Amazon~\cite{liao:mm2018}}} & 2018 & 489,000 & Annotated with 200 clothing categories & \makecell[l]{Amazon.com}\\ 
    \hline
        \multirow{3}{*}{\makecell[l]{iGlasses~\cite{gu:sigir2016}}} & \makecell[l]{Face Photo} & \multirow{3}{*}{2016} & 3,039 & \multirow{3}{*}{\makecell[l]{Annotated with both facial attributes and frame\\ attributes}} & \makecell[l]{Search engines and photo\\ sharing site}\\ 
    \cline{2-2}\cline{4-4}\cline{6-6}
         & \makecell[l]{Eyeglasses\\ Product} &  & 2,035 &  & \makecell[l]{Online eyeglasses stores}\\ 
    \hline
        \multirow{2}{*}{\makecell[l]{BrandBag~\cite{wang:icip2014}}} & \makecell[l]{BrandBag-I}  & \multirow{2}{*}{2014} & 5,545  & \makecell[l]{220 Louis Vuitton  handbag models, annotated with\\ associated style name} & \multirow{4}{*}{\makecell[l]{Google and Flickr image\\ search}}\\
        \cline{2-2}\cline{4-5}
        & \makecell[l]{BrandBag-II} &  & 4,000 & \makecell[l]{181 Coach handbag models, annotated with associ-\\ated style name} & \\ 
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:clothing_retrieval_datasets}
    \begin{tablenotes}
      \scriptsize
      \item N/A: there is no reported information to cite.
    \end{tablenotes}
\end{table*}


\subsubsection{Performance evaluations}

There are some evaluation metrics used to assess the performance of clothing retrieval methods. The different evaluation metrics used are as follows. (1) Top-\textit{k} retrieval accuracy, which is the ratio of queries with at least one matching item retrieved within the top-\textit{k} returned results. This metric is used in \cite{huang2015cross, kiapour:iccv2015, wang:icmr2016, ZQCheng2017CVPR, garcia:iccvw2017, jiang:mm2016, XLiang2016TMM, liao:mm2018, huang:mm2014, zhao:cvpr2017, ak:wacv2018, ak:patternrecogletter2018, ak:cvpr2018, wang:icip2014, wang:tmm2015, wang:tmm2016}. (2) Precision@\textit{k}, which measures the ratio of items in the top-\textit{k} returned results that are matched with the queries. This metric is used in \cite{wang2011clothes, liu2012street, fu:accv2012, kalantidis:icmr2013, li:icpr2016, sanchez-riera:mmm2017, laenen:wsdm2018}. (3) Recall@\textit{k}, which measures the ratio of matching items that are covered in the top-\textit{k} returned results. This metric is used in \cite{wang2011clothes, sanchez-riera:mmm2017}. (4) Normalized Discounted Cumulative Gain (NDCG@\textit{k}), which is the relative orders among matching and non-matching items within the top-\textit{k} returned results. %It is defined as
%\begin{equation}
%NDCG@k = \frac{1}{N}\sum_{i}^k \frac{2^{r(i)}-1}{log(i+1)},
%\label{equ:ndcg_at_k}
%\end{equation}
%the proportion of relevant documents in the top k positions.
%where $r(i)$ is the ground truth relevance indicated the matched attributes between the query image and the $i$-th ranked image, $N$ is a constant for normalization. 
This metric is used in \cite{huang2015cross, zhao:cvpr2017, gu:icmr2015, gu:sigir2016}. (5) Mean Average Precision (MAP), which measures the precision of returned results at every position in the ranked sequence of returned results across all queries. This metric evaluates the ranking performance of \cite{laenen:wsdm2018}. (6) The area under the precision recall curve (AUC), which is used to evaluate the model performance of \cite{vittayakorn:wacv2015}. (7) The ultimate percentile rank assigned to the query image, which measures the ratio of database images ranked below the matched items. (8) The correlation between the full ranking, which is computed by the method's relevance scoring function and a ground truth ranking. Both evaluation metrics (7) and (8) are used in \cite{kovashka:cvpr2012, kovashka:ijcv2015}.

Table~\ref{tab:clothing_retrieval_results} presents the performance comparisons of some retrieval methods reviewed in this survey. The best results are highlighted in bold font. We are unable to give comparisons for all different retrieval methods because the benchmarks they used are not consistent.


\begin{table}[htbp]
\footnotesize
    \centering
        \caption{Performance comparisons of some clothing retrieval methods.}
        \vspace{-3mm}
    \begin{tabular}{c|c|c|c|c}
    \Xhline{1.0pt}
        \makecell{Evaluation protocol} & \makecell{Evaluation metric} & \makecell{Dataset} & \makecell{Method} & \makecell{Result}\\
    \hline
        \multirow{4}{*}{\makecell[l]{\cite{ZQCheng2017CVPR}}} & \multirow{4}{*}{\makecell{Top-20 accuracy}} & \multirow{4}{*}{\makecell[l]{Video2Shop}} & \makecell[l]{Deep Search~\cite{huang:mm2014}} & 21.44 \\ 
    \cline{4-5}
        &  &  & \makecell[l]{Kiapour~\emph{et al.}~\cite{kiapour:iccv2015}} & 23.47 \\ 
    \cline{4-5}
        &  &  & \makecell[l]{Wang~\emph{et al.}~\cite{wang:icmr2016}} & 28.73 \\
    \cline{4-5}
        &  &  & \makecell[l]{AsymNet~\cite{ZQCheng2017CVPR}} & \textbf{36.63} \\
    \hline\hline
        \multirow{2}{*}{\makecell[l]{\cite{jiang:mm2016}}} & \multirow{2}{*}{\makecell{Top-20 accuracy}} & \multirow{2}{*}{\makecell[l]{Exact Street2Shop}}  & \makecell[l]{Kiapour~\emph{et al.}~\cite{kiapour:iccv2015}} & \textbf{30.59} \\
    \cline{4-5}
         &  &  & \makecell[l]{Jiang~\emph{et al.}~\cite{jiang:mm2016}} & 20.35 \\
    \hline\hline
        \multirow{4}{*}{\makecell[l]{\cite{ak:cvpr2018}}} & \multirow{4}{*}{\makecell{Top-30 accuracy}} & \multirow{2}{*}{\makecell[l]{Deep Fashion}}  & \makecell[l]{AMNet~\cite{zhao:cvpr2017}} & 24.60 \\
    \cline{4-5}
         &  &  & \makecell[l]{FashionSearchNet~\cite{ak:cvpr2018}} & \textbf{37.60} \\
    \cline{3-5}
         &  & \multirow{2}{*}{\makecell[l]{Shopping 100k}} & \makecell[l]{AMNet~\cite{zhao:cvpr2017}} & 40.60 \\
    \cline{4-5}
         &  &  & \makecell[l]{FashionSearchNet~\cite{ak:cvpr2018}} & \textbf{56.60} \\
    \hline\hline
        \multirow{4}{*}{\makecell[l]{\cite{liao:mm2018}}} & \multirow{4}{*}{Recall@20} & \multirow{2}{*}{\makecell[l]{Amazon}}  & \makecell[l]{AMNet~\cite{zhao:cvpr2017}} & 31.20 \\
    \cline{4-5}
         &  &  & \makecell[l]{EI Tree~\cite{liao:mm2018}} & \textbf{63.60} \\
    \cline{3-5}
         &  & \multirow{2}{*}{\makecell[l]{DARN}} & \makecell[l]{AMNet~\cite{zhao:cvpr2017}} & 60.50 \\
    \cline{4-5}
         &  &  & \makecell[l]{EI Tree~\cite{liao:mm2018}} & \textbf{71.40} \\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:clothing_retrieval_results}
\end{table}

%However, we are unable to give comparisons for all different retrieval methods due to the inconsistent benchmarks.

%--++--++

\subsection{Style Classification}

Being well dressed and knowing how to dress well is extremely important. Dressing well will make everyone look and feel confident and energetic. What is more, Tom Ford, a fashion expert and a film director, once even said, ``Dressing well is a form of good manners.'' However, not everyone is a natural-born fashion stylist. In support of this need, there have been several attempts to develop intelligent fashion style recommendations, with focused on classifying styles according to occasion, location, body shape, or social circle.


\subsubsection{State-of-the-art methods}

Liu~\emph{et al.}~\cite{liu:mm2012} explored occasion-oriented clothing recommendation by considering the \textit{wearing properly} and \textit{wearing aesthetically} principles. They adopted a unified latent Support Vector Machine (SVM) to learn the recommendation model that incorporates clothing matching rules among visual feature, attribute, and occasion. 

A location-oriented clothing recommendation is presented in \cite{zhang:tmm2017}. Different from \cite{liu:mm2012} that constrained the aesthetic matching rule to the clothing items only, Zhang~\emph{et al.}~\cite{zhang:tmm2017} considered the visual match between the foreground clothing and the background scenery. To this aim, they proposed a hybrid multi-label convolutional neural network combined with the support vector machine (mCNN-SVM), which captures the uneven distribution of clothing attributes and explicitly formulates the correlations between clothing attributes and location attributes. 

The works in \cite{hidayati:mm2018, sattar:wacv2019} developed frameworks for learning the compatibility of clothing styles and body shapes. Hidayati~\emph{et al.}~\cite{hidayati:mm2018} exploited human body measurements and images of stylish celebrities. They presented a body shape calculator to determine the type of body shape based on a set of body measurements, and a style propagation mechanism to model the correlation between body shapes and clothing styles by constructing graphs of images by the visual appearance of clothing items and body shape information respectively. Sattar~\emph{et al.}~\cite{sattar:wacv2019} used multiple photos of the same person to estimate the body shape, whereby the body shape model is built based on 2D positions of body joints and silhouette. A conditional distribution of clothing category given the inferred body shape is computed to predict the best fitting clothing.

Another work~\cite{sun:mtap2018} studied social-based recommendation on fashion style. The recommendation is implemented by combining user social circle and style consistency of clothing items. With this aim, the authors integrated a Siamese CNN-based learning model employed to analyze the fashion style consistency with social factors (\emph{i.e.}, personal interest, interpersonal interest similarity, and interpersonal influence) into a Probabilistic matrix factorization (PMF) framework.


%\begin{figure}
%  \centering
%  \subfigure[Magic Closet~\cite{liu:mm2012}.]
%  {\includegraphics[width=1\linewidth]{img/style_recommendation_liuMM2012.png}}

%  \subfigure[Trip Outfits Advisor~\cite{zhang:tmm2017}.]
%  {\includegraphics[width=0.9\linewidth]{img/style_recommendation_zhangTMM2016.png}}
  
%  \subfigure[Style for Body Shape~\cite{hidayati:mm2018}.]
%  {\includegraphics[width=1\linewidth]{img/style_recommendation_hidayatiMM2018.png}}

  %\subfigure[EI Tree~\cite{liao:mm2018}]
  %{\includegraphics[width=1\linewidth]{img/clothing_retrieval_liaoMM2018.png}}
  %\vspace{-2mm}
%  \caption{Pipelines of state-of-the-art style recommendation methods.}
%  \label{fig:clothing_retrieval_pipelines}
%\end{figure}

\subsubsection{Benchmark datasets}

Table~\ref{tab:style_recommendation_datasets} lists and compares the benchmark datasets used in~\cite{liu:mm2012, zhang:tmm2017, sun:mtap2018, hidayati:mm2018, sattar:wacv2019}. In particular, these datasets are mainly different in terms of the tasks covered.%Worthy to note, the rich social media provide valuable clues to solve the problems of fashion recommendations.

\begin{table*}[htbp]
\footnotesize
    \centering
        \caption{Summary of the benchmark datasets for style recommendation task.}
        \vspace{-3mm}
    \begin{tabular}{l|c|c|c|c|l|l}
    \Xhline{1.0pt}
      \multicolumn{2}{c|}{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ photos} & \makecell[c]{Task oriented} & \makecell[c]{Key features} & \makecell[c]{Source} \\
    \hline
        \multirow{3}{*}{\makecell[l]{What-to-Wear\\ (WoW)~\cite{liu:mm2012}}} & \makecell[l]{WOW\_Full} & \multirow{3}{*}{2012} & 9,469 & \multirow{3}{*}{\makecell{Occasion}} & \multirow{3}{*}{\makecell[l]{Annotated with 7 multi-value clothing attributes\\and 10 occasion categories via Amazon Mechan-\\ical Turk}} & \multirow{3}{*}{\makecell[l]{Online shopping \\sites, photo sharing\\ sites}} \\
    \cline{2-2}\cline{4-4}
        & \makecell[l]{WoW\_Upper} & & 8,421 & & & \\
    \cline{2-2}\cline{4-4}
        & \makecell[l]{WoW\_Lower} & & 6,527 & & & \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Journey Outfit~\cite{zhang:tmm2017}}} & 2017 & 3,392 & \makecell{Location} & \makecell[l]{Annotated with 14 travel destinations} & \makecell[l]{Online travel review\\ sites}\\
    \hline
        \multirow{2}{*}{\makecell[l]{Sun\\\emph{et al.}~\cite{sun:mtap2018}}} & \makecell[l]{Mogujie\_1} & \multirow{2}{*}{2017} & 74,686 & \multirow{2}{*}{\makecell{Social circle}} & \makecell[l]{Consists of 37,343 pairs of clothing items (tops\\ and bottoms) shared by fashion icons} & \multirow{2}{*}{\makecell[l]{Mogujie.com}}\\
    \cline{2-2}\cline{4-4}\cline{6-6}
         & \makecell[l]{Mogujie\_2} & & 30,050 &  & \makecell[l]{Contains 1031 users with their relationships} & \\
    \hline
        \multirow{6}{*}{\makecell[l]{Style for \\Body Shape\tablefootnote{\url{ http://bit.ly/Style4BodyShape}}\\\cite{hidayati:mm2018}}} & \makecell[l]{Stylish Celeb-\\rity Names} & \multirow{6}{*}{2018} & -- & \multirow{6}{*}{\makecell{Body shape}} & \makecell[l]{270 names of the top stylish female celebrities} & \makecell[l]{Ranker.com, fashion\\ magazine sites}\\
    \cline{2-2}\cline{4-4}\cline{6-7}
         & \makecell[l]{Body Measure-\\ments} &  & -- & & \makecell[l]{Body measurements of 3,150 female celebrities} & \makecell[l]{Bodymeasurements.org}\\
    \cline{2-2}\cline{4-4}\cline{6-7}
         & \makecell[l]{Stylish Celeb-\\rity Images} &  & 347,948 & & \makecell[l]{Annotated with clothing categories and celebrity\\names} & \makecell[l]{Google Image Search}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Fashion Takes Shape~\cite{sattar:wacv2019}}} & 2019 & 18,413 & \makecell{Body shape} & \makecell[l]{Annotated with metadata including clothing cate-\\gory, and a manual shape annotation indicating \\ the person's shape is above average or average} & \makecell[l]{Chictopia.com}\\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:style_recommendation_datasets}
\end{table*}


\subsubsection{Performance evaluations}

A subjective evaluation was conducted in~\cite{liu:mm2012, sun:mtap2018, hidayati:mm2018, sattar:wacv2019} to ensure the usability and functionality of the suggested styles match with users' preferences. Zhang~\emph{et al.}~\cite{zhang:tmm2017} used three common multi-label criteria, \textit{i.e.,} Macro-F, mean Average Precision (mAP), and Area under curve (AUC), to evaluate the quality of the results. In~\cite{hidayati:mm2018}, in addition to the subjective ratings of user satisfaction, the mean Average Precision (mAP) was computed to measure the overall ranks.



\subsection{Hairstyle Suggestion}

Hairstyle plays an important role in physical appearance. People can look completely different with a different hairstyle. The right hairstyle can enhance the best facial features while concealing the flaws, bringing out natural beauty and style. However, choosing the right hairstyle needs a careful selection as not all hairstyles suit all facial features.

In recent years, a lot of papers have been published related to hairstyles focusing on how to model and render hairstyles with computer graphics~\cite{chai:tog2016, paris:tog2004, selle:tog2008, xu:tog2014, fei:tog2017} or on how to segment hair automatically~\cite{yacoob:tpami2006, rousset:icip2008, wang:accv2010, wang:cvpr2012, qin:icme2017}. Only little studies have been devoted to finding the right hairstyle to suit one's face. In the following, we will review the literature concerning hairstyle recommendation.

\subsubsection{State-of-the-art methods}

The pioneer work in~\cite{yang:mmm2012} suggested suitable hairstyles for a given face by learning the relationship between facial shapes and successful hairstyle examples. The proposed example-based framework consists of two steps: the statistical learning step and the composition step. The purpose of statistical learning step is to find the most suitable hairstyle through Bayesian inference-based model that estimates the probability distributions of hairstyles to a face image. They proposed to use the ratio of line segments as the feature vector for characterizing the shape of each face, and $\alpha$-matting-based method to indicate hair area in the image. The most suitable hairstyle obtained from the statistical learning step is further superimposed over a given face image to output the face in a suitable hairstyle.

Liu~\emph{et al.} later developed the Beauty e-Experts system~\cite{liu:mm2013, liu:tomm14} to automatically recommend the most suitable facial hairstyle and makeup, and produces the synthesized visual effects. They proposed to use the extracted facial and clothing features to simultaneously learn multiple tree-structured super-graphs to collaboratively model the underlying relationships among the high-level beauty attributes (\emph{e.g.}, hair length, eye shadow color), mid-level beauty-related attributes (\emph{e.g.}, eye shape and mouth width), and low-level image features. Besides, they also proposed a facial image synthesis module that synthesis the beauty attributes recommended by the multiple tree-structured super-graphs model into the testing image. %Fig.~\ref{fig:hairstyle_suggestion_pipelines} illustrates the pipeline of the Beauty e-Experts system. 


%\begin{figure}[t!]
%  \centering
%%  \includegraphics[width=1\linewidth]{img/hairstyle_suggestion_liuMM2013.png}
%  \caption{Pipeline of the Beauty e-Experts system~\cite{liu:mm2013, liu:tomm14}.}
%  \label{fig:hairstyle_suggestion_pipelines}
%\end{figure}

\subsubsection{Benchmark datasets}

Table~\ref{tab:hairstyle_suggestion_dataset} provides benchmark datasets for assessing the performance of hairstyle suggestion methods described above. In particular, these datasets were collected from hairstyle experts. 

\begin{table*}[t!]
\footnotesize
    \centering
        \caption{Summary of the benchmark datasets for hairstyle suggestion task.}
        \vspace{-3mm}
    \begin{tabular}{c|c|c|c|c}
    \Xhline{1.0pt}
      Dataset name & \makecell{Publish \\ time} & \makecell{\# of \\ photos} &  Key features & Sources \\
    \hline
        \makecell[l]{Yang~\emph{et al.}~\cite{yang:mmm2012}} & 2012 & 84 & \makecell[l]{Frontal face photos} & \makecell[l]{Hair stylists from 3 salons}\\
     \hline
        \makecell[l]{Beauty e-Experts\\\cite{liu:mm2013}} & 2013 & 1,605 & \makecell[l]{1,505 face images with makeup and 100 face images with short/bound\\ hair and no/light makeup, annotated with 87 key points of facial land-\\mark and high-level beauty attributes} & \makecell[l]{Professional hairstyle and makeup\\ websites (\emph{e.g.,} Stylebistro.com)}\\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:hairstyle_suggestion_dataset}
\end{table*}


\subsubsection{Performance evaluations}

Yang~\emph{et al.}~\cite{yang:mmm2012} conducted a user study to evaluate the effectiveness of their proposed system, while Liu~\emph{et al.}~\cite{liu:mm2013, liu:tomm14} computed the normalized discounted cumulative gain (NDCG) that measures how close the ranking of the top-\textit{k} recommended styles is to the optimal ranking. However, we are unable to give comparisons on different hairstyle suggestion methods due to inconsistent benchmarks for different papers.

==> ACMCSUR – Fashion/src/supplementary_materials.tex <==
\section{Supplementary Materials}
\label{sec:supplementary_materials}

\begin{table*}[h]
\renewcommand{\arraystretch}{1.1}
\tiny
    \centering
        \caption{Performance comparisons of fashion parsing methods (in \%).}
        \vspace{-3mm}
    \begin{tabular}{l|l|c|c|c|c|c|c|c|c|c}
    \Xhline{1.0pt}
        \multirow{2}{*}{\makecell{Evaluation\\protocol}} & \multirow{2}{*}{\makecell[l]{Dataset}} & \multirow{2}{*}{\makecell{Method}} & \multicolumn{8}{c}{\makecell{Evaluation metric}}\\
     \cline{4-11}   
        & & & \makecell{mIOU} & \makecell[l]{aPA} & \makecell[l]{mAGR} & \makecell[l]{Acc.} & \makecell[l]{Fg. acc.} & \makecell[l]{Avg. prec.} & \makecell[l]{Avg. recall} & \makecell[l]{Avg. F-1}\\
%    \hline\hline
%        \multirow{4}{*}{\makecell[l]{\cite{dong2013deformable}}} & \multirow{2}{*}{\makecell[l]{Fashionista}} & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & 29.90 & 77.60 & -- & -- & -- & -- & -- & -- & --\\
%    \cline{3-12}
%         &  & \makecell[l]{DMPM~\cite{dong2013deformable}} & \textbf{51.70} & \textbf{83.10} & -- & -- & -- & -- & -- & -- & --\\
%    \cline{2-12}
%         & \multirow{2}{*}{\makecell[l]{Daily Photos}} & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & 24.60 & 76.60 & -- & -- & -- & -- & -- & -- & --\\
%    \cline{3-12}
%         &  & \makecell[l]{DMPM~\cite{dong2013deformable}} & \textbf{53.00} & \textbf{84.60} & -- & -- & -- & -- & -- & -- & --\\
%    \hline\hline
%        \multirow{2}{*}{\makecell[l]{\cite{SLiu2014TMM}}} & \multirow{2}{*}{\makecell[l]{CFD}} & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & 38.20 & -- & -- & -- & -- & -- & -- & --\\
%    \cline{3-12}
%        &  & \makecell[l]{Liu~\emph{et al.}~\cite{SLiu2014TMM}} & -- & \textbf{42.10} & -- & -- & -- & -- & -- & -- & --\\
%    \hline\hline
%        \multirow{2}{*}{\makecell[l]{\cite{wu:tomm2016}}} & \multirow{2}{*}{\makecell[l]{Fashionista}} & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}}  & -- & 85.10 & 57.20 & -- & -- & -- & -- & --\\
%    \cline{3-11}
%        &  & \makecell[l]{RW-MRF~\cite{wu:tomm2016}} & --  & \textbf{90.50} & \textbf{63.00} & -- & -- & -- & -- & --\\
    \hline\hline
        \multirow{4}{*}{\makecell[l]{\cite{yang:cvpr2014, XLiang2016TMM}}} & \multirow{2}{*}{\makecell[l]{SYSU-clothes}} & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & 85.97 & 51.25 & -- & -- & -- & -- & --\\
    \cline{3-11}
         &  & \makecell[l]{CCP~\cite{yang:cvpr2014, XLiang2016TMM}} & -- & 88.23 & 63.89 & -- & -- & -- & -- & --\\
    \cline{2-11}
         & \multirow{2}{*}{\makecell[l]{Fashionista}} & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & 89.00 & 64.37 & -- & -- & -- & -- & --\\
    \cline{3-11}
         &  & \makecell[l]{CCP~\cite{yang:cvpr2014, XLiang2016TMM}} & -- & \textbf{90.29} & \textbf{65.52} & -- & -- & -- & -- & --\\
%    \hline\hline
%        \multirow{2}{*}{\makecell[l]{\cite{KYamaguchi2013, yamaguchi:tpami2014}}} & \multirow{2}{*}{\makecell[l]{Paper Doll}} & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & -- & -- & 77.45 & 23.11 & 10.53 & \textbf{17.20} & 10.35\\
%    \cline{3-11}
%        &  & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2013, yamaguchi:tpami2014}} & -- & -- & -- & \textbf{84.68} & \textbf{40.20} & \textbf{33.34} & 15.34 & \textbf{14.87}\\
%    \hline\hline
%        \multirow{4}{*}{\makecell[l]{\cite{SLiu2015TMM}}} & \multirow{2}{*}{\makecell[l]{CFD}}& \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2013, yamaguchi:tpami2014}} & -- & -- & -- & 85.69 & 52.09 & 41.74 & \textbf{45.15} & 37.43\\
%    \cline{3-11}
%        &  & \makecell[l]{Liu~\emph{et al.}~\cite{SLiu2015TMM}} & -- & -- & -- & \textbf{88.92} & \textbf{58.68} & \textbf{57.68} & 43.57 & \textbf{44.90}\\
%    \cline{2-11}
%        & \multirow{2}{*}{\makecell[l]{Fashionista}}& \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2013, yamaguchi:tpami2014}} & -- & -- & -- & 82.79 & 44.08 & \textbf{49.20} & 32.00 & 32.66\\
%    \cline{3-11}
%        &  & \makecell[l]{Liu~\emph{et al.}~\cite{SLiu2015TMM}} & -- & -- & -- & \textbf{85.97} & \textbf{54.66} & 43.90 & \textbf{42.42} & \textbf{41.35}\\
    \hline\hline
        \multirow{6}{*}{\makecell[l]{\cite{XLiang2015ICCV}}} & \multirow{3}{*}{\makecell[l]{ATR}} & %\makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & -- & -- & 84.38 & 55.59 & 37.54 & 51.05 & 41.80\\
%    \cline{3-11}
%         &  & 
         \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2013, yamaguchi:tpami2014}} & -- & -- & -- & 88.96 & 62.18 & 52.75 & 49.43 & 44.76\\
%    \cline{3-11}
%         &  & \makecell[l]{Liu~\emph{et al.}~\cite{liu:cvpr2015}} & -- & -- & -- & 89.57 & 73.98 & 64.56 & 65.17 & 62.81\\
    \cline{3-11}
         &  & \makecell[l]{Liang~\emph{et al.}~\cite{liang:tpami2015}} & -- & -- & -- & 91.11 & 71.04 & 71.69 & 60.25 & 64.38\\
    \cline{3-11}
         &  & \makecell[l]{Co-CNN~\cite{XLiang2015ICCV}} & -- & -- & -- & \textbf{96.02} & \textbf{83.57} & \textbf{84.95} & \textbf{77.66} & \textbf{80.14}\\
    \cline{2-11}
         & \multirow{3}{*}{\makecell[l]{Fashionista}} & %\makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & -- & -- & 87.87 & 58.85 & 51.04 & 48.05 & 42.87\\
%    \cline{3-11}
%         &  & 
        \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2013, yamaguchi:tpami2014}} & -- & -- & -- & 89.98 & 65.66 & 54.87 & 51.16 & 46.80 \\
    \cline{3-11}
         &  & \makecell[l]{Liang~\emph{et al.}~\cite{liang:tpami2015}} & -- & -- & -- & 92.33 & 76.54 & 73.93 & 66.49 & 69.30\\
    \cline{3-11}
         &  & \makecell[l]{Co-CNN~\cite{XLiang2015ICCV}} & -- & -- & -- & \textbf{97.06} & \textbf{89.15} & \textbf{87.83} & \textbf{81.73} & \textbf{83.78}\\
    \hline\hline
        \multirow{12}{*}{\makecell[l]{\cite{3wayparsing2019}}} & \multirow{3}{*}{\makecell[l]{LIP}} & %\makecell[l]{FCN-8s~\cite{long2015fully}} & 28.29 & 76.06 & -- & 36.75 & -- & -- & -- &  --\\
%    \cline{3-11}
%         &  & 
%        \makecell[l]{SSL~\cite{Gong2017CVPR}} & 44.73 & 84.36 & -- & 54.94 & -- & -- & -- & --\\
%    \cline{3-11}
%         &  & 
        \makecell[l]{MuLA~\cite{nie2018mula}} & 49.30 & \textbf{88.50} & -- & 60.50 & -- & -- & -- & --\\
    \cline{3-11}
         &  & \makecell[l]{CE2P~\cite{CE2P2019}} & 53.10 & 87.37 & -- & 63.20 & -- & -- & -- & --\\
    \cline{3-11}
         &  & \makecell[l]{Wang~\emph{et al.}\cite{3wayparsing2019}} & \textbf{57.74} & 88.03 & -- & \textbf{68.80} & -- & -- & -- & --\\
    \cline{2-11}
         & \multirow{3}{*}{\makecell[l]{PASCAL-\\Person-Part}} & %\makecell[l]{SSL~\cite{Gong2017CVPR}} & 59.36 & -- & -- & -- & -- & -- & -- & --\\
%    \cline{3-11}
%         &  & 
         \makecell[l]{MuLA~\cite{nie2018mula}} & 65.10 & -- & -- & -- & -- & -- & -- & --\\
%    \cline{3-11}
%         &  & \makecell[l]{WSHP~\cite{WSHP2018cvpr}} & 67.60 & -- & -- & -- & -- & -- & -- & --\\
    \cline{3-11}
         &  & \makecell[l]{PGN~\cite{gong:eccv2018}} & 68.40 & -- & -- & -- & -- & -- & -- & --\\
    \cline{3-11}
         &  & \makecell[l]{Wang~\emph{et al.}~\cite{3wayparsing2019}} & \textbf{70.76} & -- & -- & -- & -- & -- & -- & --\\
    \cline{2-11}
         & \multirow{3}{*}{\makecell[l]{ATR}} & %\makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & 84.38 & -- & -- & 55.59 & 37.54 & 51.05 & 41.80\\
%    \cline{3-11}
%         &  & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2013}} & -- & 88.96 & -- & -- & 62.18 & 52.75 & 49.43 & 44.76\\
%    \cline{3-11}
%         &  & 
         \makecell[l]{Co-CNN~\cite{XLiang2015ICCV}} & -- & 96.02 & -- & -- & 83.57 & \textbf{84.95} & 77.66 & 80.14\\
    \cline{3-11}
         &  & \makecell[l]{TGPNet~\cite{TGPNet2018mm}} & -- & \textbf{96.45} & -- & -- & \textbf{87.91} & 83.36 & 80.22 & 81.76\\
    \cline{3-11}
         &  & \makecell[l]{Wang~\emph{et al.}~\cite{3wayparsing2019}} & -- & 96.26 & -- & -- & \textbf{87.91} & 84.62 & \textbf{86.41} & \textbf{85.51}\\
    \cline{2-11}
         & \multirow{3}{*}{\makecell[l]{CFD +\\Fashionista +\\CCP}} & %\makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2012CVPR}} & -- & 81.32 & -- & -- & 32.24 & 23.74 & 23.68 & 22.67\\
%    \cline{3-11}
%         &  & \makecell[l]{Yamaguchi~\emph{et al.}~\cite{KYamaguchi2013}} & -- & 87.17 & -- & -- & 50.59 & 45.80 & 34.20 & 35.13\\
%    \cline{3-11}
%         &  & 
        \makecell[l]{Deeplab~\cite{chen2018deeplab}} & -- & 87.68 & -- & -- & 56.08 & 35.35 & 39.00 & 37.09\\
     \cline{3-11}
         &  & \makecell[l]{TGPNet~\cite{TGPNet2018mm}} & -- & 91.25 & -- & -- & 66.37 & 50.71 & 53.18 & 51.92\\
    \cline{3-11}
         &  & \makecell[l]{Wang~\emph{et al.}\cite{3wayparsing2019}} & -- & \textbf{92.20} & -- & -- & \textbf{68.59} & \textbf{56.84} & \textbf{59.47} & \textbf{58.12}\\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:fashion_parsing_results}
    \begin{tablenotes}
      \scriptsize
      \item ``--'' represents detailed results are not available.
    \end{tablenotes}
\end{table*}

\begin{table}[t!]
\scriptsize
    \centering
        \caption{Performance comparisons of some clothing retrieval methods by different evaluation protocols.}
        \vspace{-3mm}
    \begin{tabular}{c|c|c|c|c}
    \Xhline{1.0pt}
        \makecell{Protocol} & \makecell{Evaluation metric} & \makecell{Dataset} & \makecell{Method} & \makecell{Result}\\
    \hline
        \makecell{\cite{ZQCheng2017CVPR}} & \makecell{Top-20 accuracy} & \makecell{Video2Shop} & \makecell{Kiapour~\emph{et al.}~\cite{kiapour:iccv2015} / Wang~\emph{et al.}~\cite{wang:icmr2016} / AsymNet~\cite{ZQCheng2017CVPR}} & \makecell{23.47 / 28.73 / \textbf{36.63}}\\
    \hline
        \makecell{\cite{jiang:mm2016}} & \makecell{Top-20 accuracy} & \makecell{Exact Street2Shop} & \makecell{Jiang~\emph{et al.}~\cite{jiang:mm2016} / Kiapour~\emph{et al.}~\cite{kiapour:iccv2015}} & \makecell{20.35 / \textbf{30.59}}\\
    \hline
        \multirow{2}{*}{\makecell[l]{\cite{ak:cvpr2018}}} & \multirow{2}{*}{\makecell{Top-30 accuracy}} & \makecell{Deep Fashion} & \makecell{AMNet~\cite{zhao:cvpr2017} / FashionSearchNet~\cite{ak:cvpr2018}} & \makecell{24.60 / \textbf{37.60}} \\
    \cline{3-5}
         &  & \makecell{Shopping 100k} & \makecell{AMNet~\cite{zhao:cvpr2017} / FashionSearchNet~\cite{ak:cvpr2018}} & \makecell {40.60 / \textbf{56.60}} \\


    \hline
        \multirow{2}{*}{\makecell[l]{\cite{liao:mm2018}}} & \multirow{2}{*}{\makecell{Recall@20}} & \makecell{Amazon} & \makecell{AMNet~\cite{zhao:cvpr2017} / EI Tree~\cite{liao:mm2018}} & \makecell{31.20 / \textbf{63.60}} \\
    \cline{3-5}
         &  & \makecell{DARN} & \makecell{AMNet~\cite{zhao:cvpr2017} / EI Tree~\cite{liao:mm2018}} & \makecell {60.50 / \textbf{71.40}} \\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:clothing_retrieval_results}
    \begin{tablenotes}
      \scriptsize
      \item The best results are highlighted in bold font.
    \end{tablenotes}
\end{table}


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> src/fashion_analysis.tex <==
\section{Fashion Analysis}
\label{sec:fashion_analysis}




\subsection{Fashion Modelling}



\subsubsection{State-of-the-art methods}



\subsubsection{Benchmark datasets}

%Each study in this task has developed its own dataset varying in the number, modality, and attractiveness score. A summary of characteristics of the benchmark datasets is presented in Table~\ref{tab:modeling_fashionbeauty_datasets}.

%\begin{table*}[t!]
%\footnotesize
%    \centering
%        \caption{Summary of the benchmark datasets for modeling fashion/beauty task.}
%        \vspace{-3mm}
%    \begin{tabular}{l|c|c|c|c|c}
%    \Xhline{1.0pt}
%      \multicolumn{2}{c|}{Dataset name} & \makecell{Publish \\ time} &  \makecell[c]{\# of photos\\ (video clips)} & Key features & Source \\
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{HOTorNOT~\cite{gray:eccv2010}}} & 2010 & 2,056 & \makecell[l]{Female frontal faces aged 18-40; annotated with ratings\\ collected from 30 labelers} & \makecell[l]{Hotornot.com}\\
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{Multi-Modality (face, dressing,\\ and voice) Beauty (M$^2$B)~\cite{nguyen:mm2012}}} & 2012 & \makecell[c]{1,240\\(280)} & \makecell[l]{Annotated with attractiveness scores, attribute categories,\\ and ethnic groups (Western or Eastern)} & \makecell[l]{YouTube.com}\\
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{Chen~\emph{et al.}~\cite{chen:icme2013}}} & 2013 & 2,648 & \makecell[l]{Annotated with fashionable or non-fashionable labels} & \makecell[l]{N/A}\\
%    \hline
%        \multicolumn{2}{c|}{\makecell[l]{Fashion144k\tablefootnote{\url{https://esslab.jp/~ess/en/data/fashion144k_stylenet/}}~\cite{simoserra:cvpr2015}}} & 2015 & 144,169 & \makecell[l]{Annotated with user-provided description, tags, number of\\ \textit{likes}, geographic location; each photo generally shows a\\ different angle of the user or zooms in on different garments} & \makecell[l]{Chictopia.com}\\
%    \hline 
%        \multicolumn{2}{c|}{\makecell[l]{Fashion products ~\cite{wang:icip2015}}} & 2015 & 500 & \makecell[l]{Annotated with the attractiveness score} & \makecell[l]{Photo sharing sites}\\
%    \hline
%        \multirow{6}{*}{\makecell[l]{Jia~\emph{et al.}\\\cite{jia:aaai2016}}} & \makecell[l]{D1: Labeled\\ Dataset} & \multirow{6}{*}{2016} & 5,500 & \makecell[l]{Annotated with 11 categories of upper-body menswear and\\ the coordinate values in the imagescale space} & \makecell[l]{Amazon.com}\\
%    \cline{2-2}\cline{4-6}
%         & \makecell[l]{D2: Unlabeled\\ Dataset} &  & 130,316 & \makecell[l]{Annotated with 11 categories of upper-body menswear} & \makecell[l]{JD.com}\\
%    \cline{2-2}\cline{4-6}
%        & \makecell[l]{D3: Demonstra-\\tion Dataset} &  & 77,160 & \makecell[l]{Consists of 76,360 menswear images from 277 brands cov-\\ering the Spring menswear and Fall menswear and 800 mens-\\wear images appearing in 2016 New York fashion week} & \makecell[l]{Style.com,\\ Thefashionisto.com}\\
%    \hline
%       \multirow{4}{*}{\makecell[l]{Chen and\\ Zhang\cite{chen:neurocomp2016}}} & \makecell[l]{Celebrity face\\ images} & \multirow{2}{*}{2016} & 390 & \multirow{4}{*}{\makecell[l]{Annotated with attractiveness score; confined to be female,\\ frontal with near neutral expressions}} & \makecell[l]{Websites}\\
%    \cline{2-2}\cline{4-4}\cline{6-6}
%        & \makecell[l]{Common face\\ images} & & 390 &  & \makecell[l]{Faceresearch.org, Flickr,\\ XM2VTS database~\cite{messer:avbpa1999},\\ Shanghai database~\cite{zhang:patternrecog2011}}\\
%    \hline
%        \multirow{2}{*}{\makecell[l]{Clothing\\ dataset\\\cite{chen:www2017}}} & \makecell[l]{Online Clothing\\ Shopping Dataset} & \multirow{2}{*}{2017} & 50,000 & \makecell[l]{Clothing products sold on Taobao from June 2014 to June\\ 2015; the associated images and user transaction data} & \makecell[l]{Taobao.com}\\
%    \cline{2-2}\cline{4-6}
%        & \makecell[l]{New York Fashion\\ Show} &  & 7,914 & \makecell[l]{Annotated with fine-grained clothing attributes} & \makecell[l]{Vogue.com}\\
%    \Xhline{1.0pt}
%    \end{tabular}
%    \label{tab:modeling_fashionbeauty_datasets}
%    \begin{tablenotes}
%      \scriptsize
%      \item N/A: there is no reported information to cite.
%    \end{tablenotes}
%\end{table*}

%\subsubsection{Performance evaluations}

%The qualitative analysis of this task uses subjective judgment, while the quantitative analysis is formulated as a classification or regression problem. The most widely used  measures to quantitatively evaluate the model performances are the classification accuracy~\cite{chen:icme2013, simoserra:cvpr2015, rothe:cvpr2016}, Mean Absolute Error (MAE)~\cite{nguyen:mm2012, jia:aaai2016, chen:neurocomp2016}, and Pearson's correlation~\cite{gray:eccv2010, rothe:cvpr2016, xu:iccasp2017}. Besides, some studies also reported their performances in terms of precision~\cite{chen:icme2013, simoserra:cvpr2015}, recall~\cite{chen:icme2013, simoserra:cvpr2015}, F1 measure~\cite{chen:icme2013}, Mean Squared Error (MSE)~\cite{jia:aaai2016}, intersection over union (IOU)~\cite{simoserra:cvpr2015}, and L1 norm~\cite{simoserra:cvpr2015}. Unfortunately, we are not able to compare the performance of each approach discussed in this section due to the unavailability of a standardized evaluation protocol.

%The MAE is defined as the average of the absolute errors between the predicted attractiveness score and the ground 
%Since the classification metrics such as accuracy, precision, recall, and intersection over union (IOU) do not capture the relationship between the different fashionability levels, we also report the L1 norm between the ground truth and the predicted label.
%the average accuracy, which is the percentage of correctly predicted ratings of the testing set, and the Pearson’s correlation.
%The Pearson Correlation is used to evaluate the performance between the ground-truth and the predicted result.


\subsection{Sociological Understanding}

\begin{comment}
In our society and century, clothing is not anymore used only as a means for body protection.
This work presents some research questions that are related to the investigation of the social signals associated to clothing.

Some research works investigated fashion within the social sciences, yang mana fashion styles correlate with personality traits, influencing the impression and behaviour of others towards a person .
clothing affects behavioral responses in the form of impression formation or person self-perception 
st systematic study on which social signals are conveyed by clothing, proposing a framework within the scope of com- puter vision to measure the clothing effect on the impression that we have on ourselves and that we trigger in the others. 
\end{comment}


%\textbf{Clothing Style and Identity.} Clothing is a visual linguistic that every piece of item conveys about the wearer to the viewer. Accordingly, analysing the clothing that people wear gives valuable information in the wearer's identity and personality.
%focuses on exploring the inherent relationship between wearer’s personality type and expressive wearing

%Aghaei~\emph{et al.}~\cite{aghaei:fg2017} presented some research questions to investigate the relationship between clothing styles and social signals. The investigation had two phases: investigation of the basic clothing behavioral cues that could be associated to an individual social signal, and investigation of the types of behaviors that might result from a social interaction taking into account the clothing styles worn by the interacting people. Jaha and Nixon~\cite{jaha:tifs2016} exploited low level image features to derive a biometric signature of soft clothing attributes for an individual. The approach enables subject identification and retrieval by using either an image or a verbal description as a query. a set of 21 soft clothing attributes is proposed for this purpose, including: (1) Head clothing; (2) Head coverage; (3) Face covered; (4) Hat; (5) Upper body clothing; (6) Neckline shape; (7) Neckline size; (8) Sleeve length; (9) Lower body clothing; (10) Shape of lower clothing; (11) Leg length of lower clothing; (12) Belt presence; (13) Shoes category; (14) Heel level; (15) Attached object category; (16) Size of bag; (17) Gun; (18) Object in hand; (19) Gloves; (20) Style category; and (21) Tattoos. %Fig.\ref{fig:sociological_understanding_pipelines} illustrates the overview of the proposed soft clothing biometrics framework in~\cite{jaha:tifs2016}. 

%The correlation between personality type and their wearing was explored in~\cite{wei:mtap2017}. To characterize different style of clothing, Wei~\emph{et al.} first segmented clothing region, verified the significance level of extracted features correlated with personality types through Binary Logistic regression, and then adopted SVM classifier to predict a person's personality.

%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=1\linewidth]{img/sociological_understanding_jahaTIFS2016.png}
%  \caption{The pipeline of soft clothing biometrics framework proposed by Jaha and Nixon~\cite{jaha:tifs2016}.}
%  \label{fig:sociological_understanding_pipelines}
%\end{figure}







%In particular, these models were evaluated in terms of .

%related to CY's recommendation
\textbf{Interaction styles.} Past research~\cite{vaccaro:chi2018} also explored personalized fashion interactions. Specifically, Vaccaro~\emph{et al.}~\cite{vaccaro:chi2018} conducted two independent studies: \textit{in-person} interaction by interviewing five personal stylists that offer in-person wardrobe and image consultations, and \textit{online} stylist interactions by developing a Facebook Messenger bot, namely PSBot, that connects users to one-on-one sessions with a stylist. 




%\cite{yamaguchi:mm2014} - The performance is measured in terms of accuracy
%\cite{park:cscw2016} - AUROC (Area Under the Receiver Operating Characteristic curve), and accuracy scores
%\cite{ha:icwsm2017} -- t-value


==> src/recommendation.tex <==
\section{Recommendation}
\label{sec:recommendation}

Fashion recommendation has attracted increasing attention given its ready applications to online shopping for fashion products. Relevant literature on the research progress of fashion recommendation falls into four main categories, \textit{i.e.}, outfit matching, fashion item retrieval, style classification, and hairstyle suggestion.

\subsection{Outfit Matching}

Each outfit generally involves multiple complementary items, such as tops, bottoms, shoes, and accessories. A key to a stylish outfit lies in the matching fashion items, as illustrated in Fig.~\ref{fig:outfit_matching_example}. However, generating harmonious fashion matching is challenging due to three main reasons. First, a fashion concept is often subtle and subjective. Second, there are a large number of attributes for describing fashion. Third, the notion of fashion item compatibility generally goes across categories and involves complex many-to-many relationships. In the past several years, this problem has attracted a great deal of interest, resulting in a long list of algorithms and techniques. %In the following, we review the current state-of-the-art of recommendation method for outfit matching.


\begin{figure}[t!]
  \centering
  \includegraphics[width=0.8\linewidth]{img/outfit_matching_hsiaoCVPR2018.png}
  \caption{Examples of outfit matching task~\cite{hsiao2018creating}.}
  \label{fig:outfit_matching_example}
\end{figure}


\subsubsection{State-of-the-art methods}

Fashion recommendation for outfit matching was initially introduced by Iwata~\emph{et al.}~\cite{iwata:ijcai2011}. They proposed a probabilistic topic model for learning information about fashion coordinates. Liu~\emph{et al.}~\cite{liu:mm2012} further adopted middle-level clothing attributes (\textit{e.g.}, clothing category, color, pattern) to learn the clothing recommendation model through a unified latent Support Vector Machine (SVM) framework. 

Inspired by the advances of deep learning technique, most of the current researchers have put efforts in modeling the style compatibility based on the data-driven deep learning approaches. Veit~\emph{et al.}~\cite{veit:iccv2015} utilized the co-purchase data from Amazon.com to train a Siamese Convolutional Neural Network (CNN) to learn style compatibility across categories. The study in~\cite{mcauley:sigir2015} modeled human preference to uncover the relationships between the appearances of pairs of items by Low-rank Mahalanobis Transform that mapped compatible items to embeddings close in the latent space. He and McAuley~\cite{he:aaai2016} later extended the work of~\cite{mcauley:sigir2015} by combining visual and historical user feedback data. The proposed study incorporates visual signals into Bayesian Personalized Ranking with Matrix Factorization as the underlying predictor. 

A line with~\cite{veit:iccv2015, mcauley:sigir2015, he:aaai2016} that aim to model item-to-item recommendation based on co-purchasing behaviour, \cite{he:icdm2016} proposed to relax the identity and symmetry assumptions inherent in metric-based recommendation methods \cite{veit:iccv2015, mcauley:sigir2015, he:aaai2016}. The \textit{Mixtures of Non-Metric Embeddings for Recommendation} framework allows \cite{he:icdm2016} to learn multiple notions of relatedness to compete and interact. Later, Veit~\emph{et al.} introduced Conditional Similarity Networks (CSNs) \cite{AVeit2017CVPR}, which learns nonlinear feature embeddings that incorporate multiple notions of similarity within a shared embedding using a shared feature extractor. The CSNs address the issue of a standard triplet embedding that treats all triplet equally and ignores the sources of similarity. In~\cite{hu:mm2015}, Hu~\emph{et al.} addressed the personalized issue by utilizing a functional tensor factorization method to model the user-item and item-item interactions. 

In particular, previous studies mainly focus on visual information but fail to consider the contextual factors. To bridge this gap, Song~\emph{et al.}~\cite{song2017neurostylist} integrated visual and contextual modalities of fashion items by employing the autoencoder neural model to seek the non-linear latent compatibility space. Following this work,~\cite{song:sigir2018} integrated fashion domain knowledge to the neural networks to boost the compatibility modeling performance. 

Most previous works~\cite{iwata:ijcai2011, liu:mm2012,  song2017neurostylist,song:sigir2018} mainly focused on top-bottom matching. However, an outfit generally includes more items, such as shoes, bags, \emph{etc}. To address this issue, Chen and He~\cite{chen2018dress} extent traditional triplet neural network, which usually receives three instances, to accept multiple instances. A mixed-category metric learning method is proposed to adapt the multiple inputs. The similar idea is also employed in~\cite{shih2018compatibility}, where the metric learning is combined with generative neural networks. The proposed generator, referred to as Metric-regularized Conditional Generative Adversarial Network (MrCGAN), is regularized by a projected compatibility distance (PCD) function. It ensures the compatible items are closer in the learned space compared to the incompatible ones. %\textcolor{red}{Given the image of a query item, the well-trained MrCGAN is able to generate an image of a compatible item.}

Other methods designed the end-to-end frameworks for outfit matching. Li \emph{et al.}~\cite{YLi2017TMM} formulated the problem as a classification task, where a given outfit composition is labeled as a popular or unpopular one. They designed a multi-modal multi-instance model based on convolutional neural networks that exploited images and meta-data of fashion items, and information across fashion items. In~\cite{han2017learning}, an end-to-end model is built based on bidirectional LSTM (Bi-LSTM). Specifically, inspired by image captioning of~\cite{donahue2015long}, Han~\emph{et al.} treated an outfit as a sequence of fashion items and each item in the outfit as a time step. A Bi-LSTM model is then utilized to predict the next item conditioned on previously seen ones, where the objective is to maximize the total probability of the given positive sequence. The model is able to achieve three tasks, \emph{i.e.}, fill-in-the-blank (fashion item recommendation given an existing set), outfit generation conditioned on users' text/image inputs, and outfit compatibility prediction. Another work~\cite{hsiao2018creating} also borrowed the idea from natural language processing. That is, an outfit is regarded as a ``document'', an inferred clothing attribute is regarded as a ``word'', and a clothing style is the ``topic''. The problem of outfit matching is formulated with the topic model. The combinations similar to previously assembled outfits should have a higher probability, which can be employed as the prediction for compatibility, and then solve the outfit matching problem. In~\cite{vasileva:eccv2018}, Vasileva~\emph{et al.} presented an approach to learning an image embedding that respects item type. They first learned a single, shared embedding space to measure item similarity, then projected from that shared embedding to subspaces identified by type.

More recently, Kang~\emph{et al.}~\cite{kang:cvpr2019} introduced ``Complete the Look'' task aiming at recommending fashion items that complement (or \textit{go well with}) the given scene. The comparison of the use-cases of product-based and the ``complete the look'' scene-based complementary recommendation is shown in Fig.~\ref{fig:outfit_matching_completeTheLook}. To achieve this task, \cite{kang:cvpr2019} measured both global compatibility (\textit{i.e.}, the compatibility between the scene and product images) and local compatibility (\textit{i.e.}, the compatibility between every scene patch and product image) via Siamese networks and category-guided attention mechanisms.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.85\linewidth]{img/outfit_matching_kangCVPR2019.png}
  \caption{A comparison of product-based complementary recommendation (top) and ``complete the look'' scene-based complementary recommendation (bottom).}
  \label{fig:outfit_matching_completeTheLook}
\end{figure}



%a popular fashion website, where users create and upload outfit data as shown in Figure 3.

\subsubsection{Benchmark datasets}

Since different papers are under various settings and most of the datasets for outfit matching are not publicly available, almost every paper for outfit  matching  collected their own dataset. The datasets were collected  from social media platforms where users can create their own outfits, such as Polyvore.com. We list the benchmark datasets for outfit matching in Table~\ref{tab:outfit_matching_datasets}. Note that the outfit database in~\cite{mcauley:sigir2015, he:aaai2016, hu:mm2015, song2017neurostylist, YLi2017TMM, han2017learning, hsiao2018creating, vasileva:eccv2018, kang:cvpr2019} comprises the images of each single item, while in~\cite{iwata:ijcai2011, liu:mm2012, chen2018dress}, an outfit is in a single image.

\begin{table*}[htbp]
\footnotesize
    \centering
        \caption{Summary of the benchmark datasets for outfit matching task.}
        \vspace{-3mm}
    \begin{tabular}{c|c|c|c|c|c}
    \Xhline{1.0pt}
      \makecell{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ outfits} & \makecell{\# of\\ items} & Key features & Sources \\
     \hline
        \makecell[l]{Iwata~\emph{et al.}~\cite{iwata:ijcai2011}} & 2011 & 14,813 & 5 &   \makecell[l]{Full-body fashion model} & \makecell[l]{Magazine, Chicisimo.com,\\ and Weardrobe.ie}\\ %clothes, bags, shoes, cosmetics, accessories
    \hline
        \makecell[l]{What-to-Wear~\cite{liu:mm2012}} & 2012 & 24,417 & 2 &  \makecell[l]{Annotated with full-body, upper-body, or lower-body} & \makecell[l]{Online shopping and photo\\ sharing sites}\\
    \hline
        \makecell[l]{Styles and Substitutes\\\cite{mcauley:sigir2015}} & 2015 & 773,465 & N/A & \makecell[l]{Annotated with 4 categories of relationship: (1) users who view-\\ed X also viewed Y, (2) users who viewed X eventually bought\\ Y, (3) users who bought X also bought Y, and (4) users bought\\ X and Y simultaneously} & \makecell[l]{Amazon.com}\\
    \hline
        \makecell[l]{Hu~\emph{et al.}~\cite{hu:mm2015}} & 2015 & 28,417 & 3 & \makecell[l]{Annotated with categories, names, and descriptions} & \makecell[l]{Polyvore.com}\\
    \hline
        \makecell[l]{He~\emph{et al.}~\cite{he:aaai2016}} & 2016 & 598.353 & N/A & \makecell[l]{Annotated with users' review histories} & \makecell[l]{Amazon.com, Tradesy.com}\\
    \hline 
        \makecell[l]{Song~\emph{et al.}~\cite{song2017neurostylist}} & 2017 & 20,726 & 2 & \makecell[l]{Annotated with title, category, and description} & \makecell[l]{Polyvore.com} \\
    \hline
        \makecell[l]{Li~\emph{et al.}~\cite{YLi2017TMM}} & 2017 & 195,262 & 4 & \makecell[l]{Annotated with\ title, category, and number of likes} & \makecell[l]{Polyvore.com} \\
    \hline 
        \makecell[l]{Han~\emph{et al.}~\cite{han2017learning}} & 2017 & 21,889 & 8 & \makecell[l]{Each item contains a pair -- product image and a corresponding\\ text description} & \makecell[l]{Polyvore.com} \\
    \hline
        \makecell[l]{Hsiao~\emph{et al.}~\cite{hsiao2018creating}} & 2018 & 3,759 & $\geq 2$ & \makecell[l]{Annotated with meta-labels, \emph{e.g.}, season (winter, spring, sum-\\mer, fall), occasion (work, vacation), and function (date, hike)} & \makecell[l]{Polyvore.com} \\
    \hline
        \makecell[l]{Vasileva~\emph{et al.}\tablefootnote{\url{https://github.com/mvasil/fashion-compatibility}}~\cite{vasileva:eccv2018}} & 2018 & 68,306 & 19 & \makecell[l]{Annotated with outfit and item ID, fine-grained item type,\\ title, and text descriptions} & \makecell[l]{Polyvore.com} \\
    \hline
        \makecell[l]{Fashion Collocation\\\cite{chen2018dress}} & 2018 & 220,000 & 5 & \makecell[l]{Annotated with independent and ready for wearing (off-body\\ module) or dependent (on-body module), or a bounding box} & \makecell[l]{Chictopia.com, Wear.net,\\ and FashionBeans.com} \\
    \hline
        \makecell[l]{Pinterest's Shop\\The Look~\cite{kang:cvpr2019}} & 2019 & 38,111 & 10 & \makecell[l]{Annotated with category} & \makecell[l]{Pinterest.com}\\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:outfit_matching_datasets}
    \begin{tablenotes}
      \scriptsize
      \item N/A: there is no reported information to cite.
    \end{tablenotes}
\end{table*}

\subsubsection{Performance evaluations}

Area Under the ROC curve (AUC) is the evaluation for most of outfit matching methods~\cite{he:aaai2016, veit:iccv2015, song2017neurostylist, song:sigir2018, shih2018compatibility, YLi2017TMM, han2017learning, vasileva:eccv2018}. Some methods are evaluated with Normalized Discounted Cumulative Gain (NDCG)(\textit{i.e.}, \cite{liu:mm2012, hu:mm2015}), prediction accuracy (\textit{i.e.}, \cite{iwata:ijcai2011, hsiao2018creating, mcauley:sigir2015, han2017learning, vasileva:eccv2018, kang:cvpr2019}), recall$@k$ (\textit{i.e.}, \cite{chen2018dress}), or Average Precision (\textit{i.e.}, \cite{YLi2017TMM}). Unfortunately, there is no unified benchmark for outfit matching, both in datasets and evaluation metrics. Therefore, we are unable to give a comparison of different methods.

%~\cite{iwata:ijcai2011}: The similarity evaluation measurement, which calculated as the average similarity between the recommended clothing and the held-out paired clothing.

\subsection{Fashion Image Retrieval}

As fashion e-commerce has grown over the years, there has been high demand for innovative solutions to help customers find preferred fashion items with ease. Though fashion many fashion online shopping sites support keyword-based searches, there are many visual traits of fashion items that are not easily translated into words. It thus attracts tremendous attention from many research communities to develop intelligent image-based fashion retrieval. Given a fashion image query, the goal of image-based fashion retrieval is to find  similar or identical items from the gallery. 


\subsubsection{State-of-the-art methods}

The notable early work on automatic image-based clothing retrieval was presented by Wang and Zhang~\cite{wang2011clothes}. They used dominant color patches to obtain the initial search results and then re-ranked these results using attribute information of clothes learned through least-squares posterior classifier (LSPC)~\cite{sugiyama:iecetis2010}.

To date, extensive research studies have been devoted to addressing the problem of cross-scenario clothing retrieval since there is a large domain discrepancy between daily human photo captured in general environment and clothing images taken in ideal conditions (\textit{i.e.}, embellished photos used in online clothing shops). %The illustration of cross-scenario clothing retrieval is presented in Fig.~\ref{fig:clothing_retrieval_street2shop}. 
In~\cite{liu2012street}, Liu~\emph{et al.} proposed to utilize an unsupervised transfer learning method based on part-based alignment and features derived from sparse reconstruction. Fu~\emph{et al.}~\cite{fu:accv2012} proposed a semantic-preserving visual phrases (SPVP) representation, which encodes the regions of human parts refined with sparse background reconstruction into the vocabulary tree under the bag-of-visual-word (BOW) framework. Kalantidis~\emph{et al.}~\cite{kalantidis:icmr2013} presented clothing retrieval in the perspective of human parsing. A prior probability map of the human body is obtained through pose estimation to guide clothing segmentation, and then the segments are classified through locality-sensitive hashing. The visually similar items are retrieved by summing up the overlap similarities. Chi~\emph{et al.} introduced Visual Part-based Object Representation (VPOR) framework~\cite{chi:mtap2016} that use partial visual appearances to obtain personalized item recommendation results. Conceptually, the VPOR decomposes every item image into a set of disjoint part, with each part represents a meaningful semantic part, then discovers auxiliary features through part-based feature propagation mechanism. The feature propagation can make two items that share a similar part but are different in the rest parts become more similar for improving the relevance of recommended results. Notably,~\cite{wang2011clothes, liu2012street, fu:accv2012, kalantidis:icmr2013, chi:mtap2016} are based on hand-crafted features.

%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=0.45\linewidth]{img/clothing_retrieval_street2shop.png}
%  \caption{\textcolor{red}{An illustration of cross-scenario clothing retrieval model.}}
%  \label{fig:clothing_retrieval_street2shop}
%\end{figure}

%Early works on image-based clothing retrieval are mostly based on hand designed features~\cite{wang2011clothes, liu2012street, fu:accv2012, kalantidis:icmr2013, kovashka:cvpr2012, kovashka:ijcv2015, li:viscomput2016}.

With the advances of deep learning, there has been a trend of building deep neural network architectures to solve the clothing retrieval task. Huang~\emph{et al.}~\cite{huang:mm2014} developed an attribute-aware clothing retrieval system using a holistic tree-structure convolutional neural network that integrates multiple clothing attributes simultaneously. Later, in~\cite{huang2015cross} they exploited the richness of the data obtained by mining images from customer review websites where the customers post photos of the clothing they have purchased. They introduced a Dual Attribute-aware Ranking Network (DARN), two sub-networks with similar structure, one for each domain, to represent deep features using attribute-guided learning. DARN simultaneously embeds semantic attributes and visual similarity constraints into the feature learning stage, while at the same time modeling the discrepancy between domains. Liang~\emph{et al.}~\cite{XLiang2016TMM} incorporated clothing parsing into clothing retrieval. Given a query clothing image, they first parse this query into fine-grained semantic regions by the proposed clothes co-parsing framework formulated as a probabilistic model, then retrieve clothing items from online shopping images. Li~\emph{et al.}~\cite{li:icpr2016} presented a hierarchical superpixel fusion strategy and a sparse coding-based attribute recognition. More explicitly, an over-segmentation hierarchical fusion algorithm with human pose estimation is utilized to get query clothing item and to retrieve similar images from product clothing dataset. To improve the accuracy of the classifiers and the adaptability of the dictionary for recognizing clothing styles in different scenarios, the intermediate domain dictionaries between product clothing dataset and daily clothing dataset are learned sequentially during the recognition phase. A personalized clothing recommendation system, namely i-Stylist, that retrieves clothing items through the analysis of user's own images is developed in \cite{sanchez-riera:mmm2017}. The i-Stylist organizes the visual information and semantic information (clothing properties) of user's clothing items as a fully connected graph. The user's personalized graph model later derives the probability distribution of the likability of an item in shopping website.

The studies in~\cite{wang2011clothes, liu2012street, fu:accv2012, kalantidis:icmr2013, huang:mm2014, huang2015cross, chi:mtap2016, li:icpr2016, sanchez-riera:mmm2017} are designed for similar retrieval. But more often, people desire to find exactly the same clothing item, as illustrated in Fig.~\ref{fig:clothing_retrieval_exactRetrieval}. The first attempt on this task was achieved by Kiapour~\emph{et al.}~\cite{kiapour:iccv2015} who evaluated some existing deep learning feature-based retrieval and similarity learning methods. Wang~\emph{et al.}\cite{wang:icmr2016} adopted a Siamese network that contains two copies of the Inception-6 network with shared weights. They introduced a \textit{robust contrastive loss} to alleviate over-fitting caused by some positive pairs (containing the same product) that are visually different, and a multi-task fine-tuning approach to learning feature representation with a softmax loss for improved results. Jiang~\emph{et al.} learned the discrepancy between street domain and shop domain clothing with a deep bi-directional cross-triplet embedding based on convolutional neural network \cite{jiang:mm2016}, and further expanded the utilization of this approach to retrieve a series of representative and complementary accessories (\textit{e.g.}, bags, shoes) to pair with the shop item~\cite{jiang:tomm2018}. Cheng~\emph{et al.}~\cite{ZQCheng2017CVPR} explored the exact matching clothes in videos to online shopping images. The videos and online shopping images are first encoded by a Long Short-Term Memory (LSTM) network and convolutional neural network, respectively, then are fed into the similarity network for pair-wise matching. Garcia~\emph{et al.}\cite{garcia:iccvw2017} proposed to relate clothing items and video frames in an indexed database and performed frame retrieval with temporal aggregation.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.5\linewidth]{img/clothing_retrieval_exactRetrieval.png}
  \caption{An illustration of exact clothing retrieval~\cite{kiapour:iccv2015}.}
  \label{fig:clothing_retrieval_exactRetrieval}
\end{figure}

In the clothing retrieval methods described above, the search is only based on query images that reflect users' needs, without considering that users may want to provide extra keywords to describe the desired attributes that are absent in the query image. Towards this goal, Kovashka~\emph{et al.} developed the WhittleSearch~\cite{kovashka:cvpr2012, kovashka:ijcv2015} that allows the user to upload a query image and provide additional relative attribute description as feedback for refining the image search results in an iterative manner (see Fig.~\ref{fig:clothing_retrieval_interactiveSearch}). This approach extends the class-based training procedure used in \cite{parikh:iccv2011} to incorporate image-level relative comparisons. In~\cite{li:viscomput2016}, Li~\emph{et al.} incorporated the relevant feedback approach into the optimum-path Forest classifier to enable users to search the clothing items of preferred collar design. Several traditional-based feature extraction methods are proposed to capture three kinds of collar designs -- collar spread, turnover, and front designs.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.95\linewidth]{img/clothing_retrieval_interactiveSearch.png}
  \caption{An example of interactive fashion search~\cite{kovashka:cvpr2012}.}
  \label{fig:clothing_retrieval_interactiveSearch}
\end{figure}

Unlike previous \textit{interactive fashion search} approaches that the user cannot change the attribute from one to another easily~\cite{kovashka:cvpr2012, kovashka:ijcv2015} or are designed for a specific attribute~\cite{li:viscomput2016}, the memory-augmented Attribute Manipulation Network (AMNet)~\cite{zhao:cvpr2017} is capable of manipulating image representation at the attribute level. Given a query image and attribute manipulation request, such as ``\textit{I want to buy a jacket that looks like this query image, but with blue color instead of pink and plush collar instead of round collar},'' AMNet updates the query representation encoding the unwanted attributes and replace them to the desired ones. The manipulated representation is then used to retrieve images with desired attributes from the gallery. Later, Ak~\emph{et al.}~\cite{ak:wacv2018, ak:patternrecogletter2018, ak:cvpr2018} explored the localization aspect of attribute representations to facilitate region-specific attribute manipulation requests. In particular, \cite{ak:wacv2018} estimated clothing item parts using an unsupervised segmentation method and applied CNN with part-based triplet ranking constraint as an attention mechanism.~\cite{ak:patternrecogletter2018} introduced ``Part Guided CNN'', a Convolutional Neural Network (CNN) controlled by constituent parts of clothing items, to conduct learning of the respective attributes of clothing parts. A Markov Random Field based color encoding method is adopted to generate specific color descriptions.~\cite{ak:cvpr2018} presented the FashionSearchNet to learn regions and region-specific attribute representations by exploiting the attribute activation maps (AAMs) generated by global average pooling (GAP) layer. %Fig.~\ref{fig:clothing_retrieval_pipelines}(c) presents an overview of the proposed framework in~\cite{ak:cvpr2018}.

In~\cite{laenen:wsdm2018}, Laenen~\emph{et al.} built a multimodal retrieval model that uses a combination of an image and text as a query and ranks the image results based on their semantic similarity to the query text and their visual similarity to the query image. Different from~\cite{zhao:cvpr2017, ak:wacv2018, ak:patternrecogletter2018, ak:cvpr2018} that used neural networks to construct visual representation of searched item by manipulating the visual representation of query image with the textual attributes in query text, \cite{laenen:wsdm2018} used neural network to infer the semantic relationship between visual and textual attributes in a joint multimodal embedding space. To help facilitate the reasoning of search results and user intent, Liao~\emph{et al.}~\cite{liao:mm2018} built EI (Exclusive and Independent) tree that captures hierarchical structures of the fashion concepts. The EI Tree is generated by  incorporating product hierarchies of online shopping websites and domain knowledge of fashion experts. The generated EI tree is then applied to guide the end-to-end deep learning procedure, mapping the implicit deep features to explicit fashion concepts.

Different problem is tackled in the fashion retrieval literature. Gu~\emph{et al.}~\cite{gu:icmr2015} presented a cross-scenario eyeglasses retrieval system, namely Fashion Glasses Search System (FGSS). They introduced a keypoint-based scheme called \textit{EyeGlass keYPoinT} (EGYPT) to describe the appearances of glasses, making FGSS free from segmentation problems. In the EGYPT, hybrid feature descriptors that combine shape, color, and texture features extracted from the detected keypoints are exploited to form a representative feature vector. Gu~\emph{et al.} later developed iGlasses~\cite{gu:sigir2016}, a recommendation for best-fits glasses that exploits the implicit matching rules between human faces and eyeglasses. Given a frontal face photo as the input, the iGlasses captures the correlation among the fine-grained attributes of human faces and frames of glasses, and then returns a ranked list of candidate eyeglasses. It further produces a synthesized image for the input face to demonstrate the visual effect when wearing the recommended glasses. 

The studies in~\cite{wang:icip2014, wang:tmm2016, wang:tmm2015} dealt with handbag recognition problems. In particular, Wang~\emph{et al.}~\cite{wang:icip2014} introduced a complementary feature obtained by extracting low-level features from a structure enhanced handbag image to compensate the missing details of the feature, called original feature, extracted directly from the original handbag image. The complementary feature is then fused with the original feature for the recognition. \cite{wang:tmm2016} further extended~\cite{wang:icip2014} by utilizing color model based on dominant color naming features. A CNN-based model for end-to-end framework to recognize the handbag models is presented in~\cite{wang:tmm2015}. It proposed feature selective joint classification regression CNN (FSCR-CNN) classification model, which consists of Feature Selective CNN and joint Classification-Regression CNN, to attenuate the illumination changes and inter-class similarity among handbags. The scores from FSCR-CNN classification model and CNN detection model are further eventually combined by a conditional probability model to recognize the handbag. 

Other than fashion image retrieval studies mentioned above, Vittayakorn \emph{et al.}~\cite{vittayakorn:wacv2015} learned human based judgments of outfit similarity. They employed a linear SVM for pairwise comparison of clothing outfits based on a learned combination of features computed over parsed clothing regions. In \cite{semertzidis:tist2016}, Semertzidis~\emph{et al.} designed and evaluated a crowd-powered system for visual fashion similarity search based on user-defined criteria. Different kinds of crowds, ranges from click workers for tedious tasks, such as cleaning content, to mobile fashion crowds, are integrated for this purpose.

%\begin{figure}
%  \centering
%  \subfigure[Wang and Zhang~\cite{wang2011clothes}.]
%  {\includegraphics[width=1\linewidth]{img/clothing_retrieval_wangMM2011.png}}

%  \subfigure[Deep Search~\cite{huang:mm2014}.]
%  {\includegraphics[width=0.9\linewidth]{img/clothing_retrieval_huangMM2014.png}}
  
%  \subfigure[FashionSearchNet~\cite{ak:cvpr2018}.]
%  {\includegraphics[width=1\linewidth]{img/clothing_retrieval_akCVPR2018.png}}

%  \subfigure[EI Tree~\cite{liao:mm2018}.]
%  {\includegraphics[width=1\linewidth]{img/clothing_retrieval_liaoMM2018.png}}
  %\vspace{-2mm}
%  \caption{Pipelines of state-of-the-art clothing retrieval methods.}
%  \label{fig:clothing_retrieval_pipelines}
%\end{figure}

\subsubsection{Benchmark datasets}

The existing clothing retrieval studies mainly focused on a cross-domain scenario. Therefore, most of the benchmark datasets were collected from daily photos and online clothing shopping websites. Table~\ref{tab:clothing_retrieval_datasets} gives a summary and link of the download page (if publicly available) of the benchmark datasets.% used to evaluate the fashion retrieval studies.


\begin{table*}[htbp]
\footnotesize
    \centering
        \caption{Summary of the benchmark datasets for fashion retrieval task.}
        \vspace{-3mm}
    \begin{tabular}{l|c|c|c|l|c}
    \Xhline{1.0pt}
        \multicolumn{2}{c|}{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ photos\\ (videos)}  & \makecell{Key features} & Sources \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{The Gallagher Collection Person\tablefootnote{\url{http://chenlab.ece.cornell.edu/people/Andy/projectpage_clothing.html}}~\cite{gallagher:cvpr2008}}} & 2008 & 589 & \makecell[l]{Annotated 1008 faces with 32 identities} & \makecell[l]{N/A}\\ 
    \hline
        \multirow{2}{*}{\makecell[l]{Liu~\emph{et al.}~\cite{liu2012street}}} & \makecell[l]{Online Shopping} & \multirow{2}{*}{2012} & 16,636 & \multirow{2}{*}{\makecell[l]{Each image consists of either upper- or lower-wear,\\ annotated with clothing-specific attributes}} & \makecell[l]{Online shopping sites}\\ 
        \cline{2-2}\cline{4-4}\cline{6-6}
        & \makecell[l]{Daily Photo} &  & 8,389 & & \makecell[l]{Flickr.com }\\ 
    \hline
        \multirow{2}{*}{\makecell[l]{Fu~\emph{et al.}~\cite{fu:accv2012}}} & \makecell[l]{Online Shopping} & \multirow{2}{*}{2012} & ~110,000 & \multirow{2}{*}{\makecell[l]{Each image consists of either upper- or lower-wear,\\ annotated with clothing-specific attributes}} & \makecell[l]{Amazon.com, eBay.com,\\ vancl.com, taobao.com}\\ 
        \cline{2-2}\cline{4-4}\cline{6-6}
        & \makecell[l]{Daily Photo} &  & \makecell{2,000} & & \makecell[l]{Flickr.com }\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Fashion-focused Creative Commons\\ Social\tablefootnote{\url{http://skuld.cs.umass.edu/traces/mmsys/2013/fashion/}}~\cite{loni:mmsys2013}}} & 2013 & 4,810 & \makecell[l]{Annotated with 154 fashion-focused categories (per-\\formed by crowdsourcing workers and trusted anno-\\tators), user-provided metadata, tags, favorites, com-\\ments, context, and note} & \makecell[l]{Flickr.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Chi~\emph{et al.}~\cite{chi:mtap2016}}} & 2016 & 23,854  & \makecell[l]{Annotated with 5 categories} & \makecell[l]{Amazon.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{UT-Zap50K shoe\tablefootnote{\url{http://vision.cs.utexas.edu/projects/finegrained/}}~\cite{yu:cvpr2014}}} & 2014 & 50,000  & \makecell[l]{Shoe images annotated with associated metadata\\ (shoe type, materials, manufacturer, gender, \emph{etc}.)} & \makecell[l]{Zappos.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Fashion 10000\tablefootnote{\url{http://skuld.cs.umass.edu/traces/mmsys/2014/user05.tar}}~\cite{loni:mmsys2014}}} & 2014 &  32,398 & \makecell[l]{Annotated with 470 fashion categories, associated\\ metadata, ground truth labels} & \makecell[l]{Flickr.com}\\ 
    \hline
        \multirow{2}{*}{\makecell[l]{Li~\emph{et al.}~\cite{li:icpr2016}}} & \makecell[l]{Product Clothing} & \multirow{2}{*}{2016} & 15,690 & \multirow{2}{*}{\makecell[l]{Annotated with clothing category}} & \makecell[l]{Online shopping sites}\\ 
        \cline{2-2}\cline{4-4}\cline{6-6}
        & \makecell[l]{Daily Clothing} &  & \makecell{4,206} & & \makecell[l]{Flickr.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{DARN~\cite{huang2015cross}}} & 2015 & 545,373 & \makecell[l]{Online-offline upper-clothing image pair, annotated\\ with clothing attribute categories} & \makecell[l]{Online-shopping sites\\ and corresponding customer\\ review pages}\\ 
    \hline
        \multirow{2}{*}{\makecell[l]{Exact Street2Shop\tablefootnote{http://www.tamaraberg.com/street2shop}\\\cite{kiapour:iccv2015}}} & \makecell[l]{Street photos} & \multirow{2}{*}{2015} & \makecell{20,357} & \multirow{2}{*}{\makecell[l]{39,479 pairs of exactly matching items worn in\\street photos and shown in shop photos}} & \makecell[l]{ModCloth.com}\\ 
    \cline{2-2}\cline{4-4}\cline{6-6}
         & \makecell[l]{Shop photos} & & 404,683 & & \makecell[l]{Online clothing retailers}\\ 
    \hline 
        \multicolumn{2}{c|}{\makecell[l]{MVC\tablefootnote{http://mvc-datasets.github.io/MVC/}~\cite{liu:icmr2016}}} & 2016 & 161,638 & Annotated with 264 attribute labels & \makecell[l]{Online shopping sites}\\ 
    \hline
        \multirow{2}{*}{\makecell[l]{Video2Shop\cite{ZQCheng2017CVPR}}} & \makecell[l]{Videos} & \multirow{2}{*}{2017} & \makecell{26,352\\(526)} & \multirow{2}{*}{\makecell[l]{39,479 exact matching pairs annotated with 14 cat-\\egories of clothes}} & \makecell[l]{Tmall MagicBox}\\ 
    \cline{2-2}\cline{4-4}\cline{6-6}
         & \makecell[l]{Online shopping} & & 85,677 & & \makecell[l]{Tmall.com, Taobao.com}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Shopping100k~\cite{ak:wacv2018}}} & 2018 & 101,021 & \makecell[l]{Annotated with 12 fashion attributes} & \makecell[l]{Online shopping sites}\\ 
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Amazon~\cite{liao:mm2018}}} & 2018 & 489,000 & Annotated with 200 clothing categories & \makecell[l]{Amazon.com}\\ 
    \hline
        \multirow{3}{*}{\makecell[l]{iGlasses~\cite{gu:sigir2016}}} & \makecell[l]{Face Photo} & \multirow{3}{*}{2016} & 3,039 & \multirow{3}{*}{\makecell[l]{Annotated with both facial attributes and frame\\ attributes}} & \makecell[l]{Search engines and photo\\ sharing site}\\ 
    \cline{2-2}\cline{4-4}\cline{6-6}
         & \makecell[l]{Eyeglasses\\ Product} &  & 2,035 &  & \makecell[l]{Online eyeglasses stores}\\ 
    \hline
        \multirow{2}{*}{\makecell[l]{BrandBag~\cite{wang:icip2014}}} & \makecell[l]{BrandBag-I}  & \multirow{2}{*}{2014} & 5,545  & \makecell[l]{220 Louis Vuitton  handbag models, annotated with\\ associated style name} & \multirow{4}{*}{\makecell[l]{Google and Flickr image\\ search}}\\
        \cline{2-2}\cline{4-5}
        & \makecell[l]{BrandBag-II} &  & 4,000 & \makecell[l]{181 Coach handbag models, annotated with associ-\\ated style name} & \\ 
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:clothing_retrieval_datasets}
    \begin{tablenotes}
      \scriptsize
      \item N/A: there is no reported information to cite.
    \end{tablenotes}
\end{table*}


\subsubsection{Performance evaluations}

There are some evaluation metrics used to assess the performance of clothing retrieval methods. The different evaluation metrics used are as follows. (1) Top-\textit{k} retrieval accuracy, which is the ratio of queries with at least one matching item retrieved within the top-\textit{k} returned results. This metric is used in \cite{huang2015cross, kiapour:iccv2015, wang:icmr2016, ZQCheng2017CVPR, garcia:iccvw2017, jiang:mm2016, XLiang2016TMM, liao:mm2018, huang:mm2014, zhao:cvpr2017, ak:wacv2018, ak:patternrecogletter2018, ak:cvpr2018, wang:icip2014, wang:tmm2015, wang:tmm2016}. (2) Precision@\textit{k}, which measures the ratio of items in the top-\textit{k} returned results that are matched with the queries. This metric is used in \cite{wang2011clothes, liu2012street, fu:accv2012, kalantidis:icmr2013, li:icpr2016, sanchez-riera:mmm2017, laenen:wsdm2018}. (3) Recall@\textit{k}, which measures the ratio of matching items that are covered in the top-\textit{k} returned results. This metric is used in \cite{wang2011clothes, sanchez-riera:mmm2017}. (4) Normalized Discounted Cumulative Gain (NDCG@\textit{k}), which is the relative orders among matching and non-matching items within the top-\textit{k} returned results. %It is defined as
%\begin{equation}
%NDCG@k = \frac{1}{N}\sum_{i}^k \frac{2^{r(i)}-1}{log(i+1)},
%\label{equ:ndcg_at_k}
%\end{equation}
%the proportion of relevant documents in the top k positions.
%where $r(i)$ is the ground truth relevance indicated the matched attributes between the query image and the $i$-th ranked image, $N$ is a constant for normalization. 
This metric is used in \cite{huang2015cross, zhao:cvpr2017, gu:icmr2015, gu:sigir2016}. (5) Mean Average Precision (MAP), which measures the precision of returned results at every position in the ranked sequence of returned results across all queries. This metric evaluates the ranking performance of \cite{laenen:wsdm2018}. (6) The area under the precision recall curve (AUC), which is used to evaluate the model performance of \cite{vittayakorn:wacv2015}. (7) The ultimate percentile rank assigned to the query image, which measures the ratio of database images ranked below the matched items. (8) The correlation between the full ranking, which is computed by the method's relevance scoring function and a ground truth ranking. Both evaluation metrics (7) and (8) are used in \cite{kovashka:cvpr2012, kovashka:ijcv2015}.

Table~\ref{tab:clothing_retrieval_results} presents the performance comparisons of some retrieval methods reviewed in this survey. The best results are highlighted in bold font. We are unable to give comparisons for all different retrieval methods because the benchmarks they used are not consistent.


\begin{table}[htbp]
\footnotesize
    \centering
        \caption{Performance comparisons of some clothing retrieval methods.}
        \vspace{-3mm}
    \begin{tabular}{c|c|c|c|c}
    \Xhline{1.0pt}
        \makecell{Evaluation protocol} & \makecell{Evaluation metric} & \makecell{Dataset} & \makecell{Method} & \makecell{Result}\\
    \hline
        \multirow{4}{*}{\makecell[l]{\cite{ZQCheng2017CVPR}}} & \multirow{4}{*}{\makecell{Top-20 accuracy}} & \multirow{4}{*}{\makecell[l]{Video2Shop}} & \makecell[l]{Deep Search~\cite{huang:mm2014}} & 21.44 \\ 
    \cline{4-5}
        &  &  & \makecell[l]{Kiapour~\emph{et al.}~\cite{kiapour:iccv2015}} & 23.47 \\ 
    \cline{4-5}
        &  &  & \makecell[l]{Wang~\emph{et al.}~\cite{wang:icmr2016}} & 28.73 \\
    \cline{4-5}
        &  &  & \makecell[l]{AsymNet~\cite{ZQCheng2017CVPR}} & \textbf{36.63} \\
    \hline\hline
        \multirow{2}{*}{\makecell[l]{\cite{jiang:mm2016}}} & \multirow{2}{*}{\makecell{Top-20 accuracy}} & \multirow{2}{*}{\makecell[l]{Exact Street2Shop}}  & \makecell[l]{Kiapour~\emph{et al.}~\cite{kiapour:iccv2015}} & \textbf{30.59} \\
    \cline{4-5}
         &  &  & \makecell[l]{Jiang~\emph{et al.}~\cite{jiang:mm2016}} & 20.35 \\
    \hline\hline
        \multirow{4}{*}{\makecell[l]{\cite{ak:cvpr2018}}} & \multirow{4}{*}{\makecell{Top-30 accuracy}} & \multirow{2}{*}{\makecell[l]{Deep Fashion}}  & \makecell[l]{AMNet~\cite{zhao:cvpr2017}} & 24.60 \\
    \cline{4-5}
         &  &  & \makecell[l]{FashionSearchNet~\cite{ak:cvpr2018}} & \textbf{37.60} \\
    \cline{3-5}
         &  & \multirow{2}{*}{\makecell[l]{Shopping 100k}} & \makecell[l]{AMNet~\cite{zhao:cvpr2017}} & 40.60 \\
    \cline{4-5}
         &  &  & \makecell[l]{FashionSearchNet~\cite{ak:cvpr2018}} & \textbf{56.60} \\
    \hline\hline
        \multirow{4}{*}{\makecell[l]{\cite{liao:mm2018}}} & \multirow{4}{*}{Recall@20} & \multirow{2}{*}{\makecell[l]{Amazon}}  & \makecell[l]{AMNet~\cite{zhao:cvpr2017}} & 31.20 \\
    \cline{4-5}
         &  &  & \makecell[l]{EI Tree~\cite{liao:mm2018}} & \textbf{63.60} \\
    \cline{3-5}
         &  & \multirow{2}{*}{\makecell[l]{DARN}} & \makecell[l]{AMNet~\cite{zhao:cvpr2017}} & 60.50 \\
    \cline{4-5}
         &  &  & \makecell[l]{EI Tree~\cite{liao:mm2018}} & \textbf{71.40} \\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:clothing_retrieval_results}
\end{table}

%However, we are unable to give comparisons for all different retrieval methods due to the inconsistent benchmarks.

%--++--++

\subsection{Style Classification}

Being well dressed and knowing how to dress well is extremely important. Dressing well will make everyone look and feel confident and energetic. What is more, Tom Ford, a fashion expert and a film director, once even said, ``Dressing well is a form of good manners.'' However, not everyone is a natural-born fashion stylist. In support of this need, there have been several attempts to develop intelligent fashion style recommendations, with focused on classifying styles according to occasion, location, body shape, or social circle.


\subsubsection{State-of-the-art methods}

Liu~\emph{et al.}~\cite{liu:mm2012} explored occasion-oriented clothing recommendation by considering the \textit{wearing properly} and \textit{wearing aesthetically} principles. They adopted a unified latent Support Vector Machine (SVM) to learn the recommendation model that incorporates clothing matching rules among visual feature, attribute, and occasion. 

A location-oriented clothing recommendation is presented in \cite{zhang:tmm2017}. Different from \cite{liu:mm2012} that constrained the aesthetic matching rule to the clothing items only, Zhang~\emph{et al.}~\cite{zhang:tmm2017} considered the visual match between the foreground clothing and the background scenery. To this aim, they proposed a hybrid multi-label convolutional neural network combined with the support vector machine (mCNN-SVM), which captures the uneven distribution of clothing attributes and explicitly formulates the correlations between clothing attributes and location attributes. 

The works in \cite{hidayati:mm2018, sattar:wacv2019} developed frameworks for learning the compatibility of clothing styles and body shapes. Hidayati~\emph{et al.}~\cite{hidayati:mm2018} exploited human body measurements and images of stylish celebrities. They presented a body shape calculator to determine the type of body shape based on a set of body measurements, and a style propagation mechanism to model the correlation between body shapes and clothing styles by constructing graphs of images by the visual appearance of clothing items and body shape information respectively. Sattar~\emph{et al.}~\cite{sattar:wacv2019} used multiple photos of the same person to estimate the body shape, whereby the body shape model is built based on 2D positions of body joints and silhouette. A conditional distribution of clothing category given the inferred body shape is computed to predict the best fitting clothing.

Another work~\cite{sun:mtap2018} studied social-based recommendation on fashion style. The recommendation is implemented by combining user social circle and style consistency of clothing items. With this aim, the authors integrated a Siamese CNN-based learning model employed to analyze the fashion style consistency with social factors (\emph{i.e.}, personal interest, interpersonal interest similarity, and interpersonal influence) into a Probabilistic matrix factorization (PMF) framework.


%\begin{figure}
%  \centering
%  \subfigure[Magic Closet~\cite{liu:mm2012}.]
%  {\includegraphics[width=1\linewidth]{img/style_recommendation_liuMM2012.png}}

%  \subfigure[Trip Outfits Advisor~\cite{zhang:tmm2017}.]
%  {\includegraphics[width=0.9\linewidth]{img/style_recommendation_zhangTMM2016.png}}
  
%  \subfigure[Style for Body Shape~\cite{hidayati:mm2018}.]
%  {\includegraphics[width=1\linewidth]{img/style_recommendation_hidayatiMM2018.png}}

  %\subfigure[EI Tree~\cite{liao:mm2018}]
  %{\includegraphics[width=1\linewidth]{img/clothing_retrieval_liaoMM2018.png}}
  %\vspace{-2mm}
%  \caption{Pipelines of state-of-the-art style recommendation methods.}
%  \label{fig:clothing_retrieval_pipelines}
%\end{figure}

\subsubsection{Benchmark datasets}

Table~\ref{tab:style_recommendation_datasets} lists and compares the benchmark datasets used in~\cite{liu:mm2012, zhang:tmm2017, sun:mtap2018, hidayati:mm2018, sattar:wacv2019}. In particular, these datasets are mainly different in terms of the tasks covered.%Worthy to note, the rich social media provide valuable clues to solve the problems of fashion recommendations.

\begin{table*}[htbp]
\footnotesize
    \centering
        \caption{Summary of the benchmark datasets for style recommendation task.}
        \vspace{-3mm}
    \begin{tabular}{l|c|c|c|c|l|l}
    \Xhline{1.0pt}
      \multicolumn{2}{c|}{Dataset name} & \makecell{Publish \\ time} & \makecell{\# of \\ photos} & \makecell[c]{Task oriented} & \makecell[c]{Key features} & \makecell[c]{Source} \\
    \hline
        \multirow{3}{*}{\makecell[l]{What-to-Wear\\ (WoW)~\cite{liu:mm2012}}} & \makecell[l]{WOW\_Full} & \multirow{3}{*}{2012} & 9,469 & \multirow{3}{*}{\makecell{Occasion}} & \multirow{3}{*}{\makecell[l]{Annotated with 7 multi-value clothing attributes\\and 10 occasion categories via Amazon Mechan-\\ical Turk}} & \multirow{3}{*}{\makecell[l]{Online shopping \\sites, photo sharing\\ sites}} \\
    \cline{2-2}\cline{4-4}
        & \makecell[l]{WoW\_Upper} & & 8,421 & & & \\
    \cline{2-2}\cline{4-4}
        & \makecell[l]{WoW\_Lower} & & 6,527 & & & \\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Journey Outfit~\cite{zhang:tmm2017}}} & 2017 & 3,392 & \makecell{Location} & \makecell[l]{Annotated with 14 travel destinations} & \makecell[l]{Online travel review\\ sites}\\
    \hline
        \multirow{2}{*}{\makecell[l]{Sun\\\emph{et al.}~\cite{sun:mtap2018}}} & \makecell[l]{Mogujie\_1} & \multirow{2}{*}{2017} & 74,686 & \multirow{2}{*}{\makecell{Social circle}} & \makecell[l]{Consists of 37,343 pairs of clothing items (tops\\ and bottoms) shared by fashion icons} & \multirow{2}{*}{\makecell[l]{Mogujie.com}}\\
    \cline{2-2}\cline{4-4}\cline{6-6}
         & \makecell[l]{Mogujie\_2} & & 30,050 &  & \makecell[l]{Contains 1031 users with their relationships} & \\
    \hline
        \multirow{6}{*}{\makecell[l]{Style for \\Body Shape\tablefootnote{\url{ http://bit.ly/Style4BodyShape}}\\\cite{hidayati:mm2018}}} & \makecell[l]{Stylish Celeb-\\rity Names} & \multirow{6}{*}{2018} & -- & \multirow{6}{*}{\makecell{Body shape}} & \makecell[l]{270 names of the top stylish female celebrities} & \makecell[l]{Ranker.com, fashion\\ magazine sites}\\
    \cline{2-2}\cline{4-4}\cline{6-7}
         & \makecell[l]{Body Measure-\\ments} &  & -- & & \makecell[l]{Body measurements of 3,150 female celebrities} & \makecell[l]{Bodymeasurements.org}\\
    \cline{2-2}\cline{4-4}\cline{6-7}
         & \makecell[l]{Stylish Celeb-\\rity Images} &  & 347,948 & & \makecell[l]{Annotated with clothing categories and celebrity\\names} & \makecell[l]{Google Image Search}\\
    \hline
        \multicolumn{2}{c|}{\makecell[l]{Fashion Takes Shape~\cite{sattar:wacv2019}}} & 2019 & 18,413 & \makecell{Body shape} & \makecell[l]{Annotated with metadata including clothing cate-\\gory, and a manual shape annotation indicating \\ the person's shape is above average or average} & \makecell[l]{Chictopia.com}\\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:style_recommendation_datasets}
\end{table*}


\subsubsection{Performance evaluations}

A subjective evaluation was conducted in~\cite{liu:mm2012, sun:mtap2018, hidayati:mm2018, sattar:wacv2019} to ensure the usability and functionality of the suggested styles match with users' preferences. Zhang~\emph{et al.}~\cite{zhang:tmm2017} used three common multi-label criteria, \textit{i.e.,} Macro-F, mean Average Precision (mAP), and Area under curve (AUC), to evaluate the quality of the results. In~\cite{hidayati:mm2018}, in addition to the subjective ratings of user satisfaction, the mean Average Precision (mAP) was computed to measure the overall ranks.



\subsection{Hairstyle Suggestion}

Hairstyle plays an important role in physical appearance. People can look completely different with a different hairstyle. The right hairstyle can enhance the best facial features while concealing the flaws, bringing out natural beauty and style. However, choosing the right hairstyle needs a careful selection as not all hairstyles suit all facial features.

In recent years, a lot of papers have been published related to hairstyles focusing on how to model and render hairstyles with computer graphics~\cite{chai:tog2016, paris:tog2004, selle:tog2008, xu:tog2014, fei:tog2017} or on how to segment hair automatically~\cite{yacoob:tpami2006, rousset:icip2008, wang:accv2010, wang:cvpr2012, qin:icme2017}. Only little studies have been devoted to finding the right hairstyle to suit one's face. In the following, we will review the literature concerning hairstyle recommendation.

\subsubsection{State-of-the-art methods}

The pioneer work in~\cite{yang:mmm2012} suggested suitable hairstyles for a given face by learning the relationship between facial shapes and successful hairstyle examples. The proposed example-based framework consists of two steps: the statistical learning step and the composition step. The purpose of statistical learning step is to find the most suitable hairstyle through Bayesian inference-based model that estimates the probability distributions of hairstyles to a face image. They proposed to use the ratio of line segments as the feature vector for characterizing the shape of each face, and $\alpha$-matting-based method to indicate hair area in the image. The most suitable hairstyle obtained from the statistical learning step is further superimposed over a given face image to output the face in a suitable hairstyle.

Liu~\emph{et al.} later developed the Beauty e-Experts system~\cite{liu:mm2013, liu:tomm14} to automatically recommend the most suitable facial hairstyle and makeup, and produces the synthesized visual effects. They proposed to use the extracted facial and clothing features to simultaneously learn multiple tree-structured super-graphs to collaboratively model the underlying relationships among the high-level beauty attributes (\emph{e.g.}, hair length, eye shadow color), mid-level beauty-related attributes (\emph{e.g.}, eye shape and mouth width), and low-level image features. Besides, they also proposed a facial image synthesis module that synthesis the beauty attributes recommended by the multiple tree-structured super-graphs model into the testing image. %Fig.~\ref{fig:hairstyle_suggestion_pipelines} illustrates the pipeline of the Beauty e-Experts system. 


%\begin{figure}[t!]
%  \centering
%%  \includegraphics[width=1\linewidth]{img/hairstyle_suggestion_liuMM2013.png}
%  \caption{Pipeline of the Beauty e-Experts system~\cite{liu:mm2013, liu:tomm14}.}
%  \label{fig:hairstyle_suggestion_pipelines}
%\end{figure}

\subsubsection{Benchmark datasets}

Table~\ref{tab:hairstyle_suggestion_dataset} provides benchmark datasets for assessing the performance of hairstyle suggestion methods described above. In particular, these datasets were collected from hairstyle experts. 

\begin{table*}[t!]
\footnotesize
    \centering
        \caption{Summary of the benchmark datasets for hairstyle suggestion task.}
        \vspace{-3mm}
    \begin{tabular}{c|c|c|c|c}
    \Xhline{1.0pt}
      Dataset name & \makecell{Publish \\ time} & \makecell{\# of \\ photos} &  Key features & Sources \\
    \hline
        \makecell[l]{Yang~\emph{et al.}~\cite{yang:mmm2012}} & 2012 & 84 & \makecell[l]{Frontal face photos} & \makecell[l]{Hair stylists from 3 salons}\\
     \hline
        \makecell[l]{Beauty e-Experts\\\cite{liu:mm2013}} & 2013 & 1,605 & \makecell[l]{1,505 face images with makeup and 100 face images with short/bound\\ hair and no/light makeup, annotated with 87 key points of facial land-\\mark and high-level beauty attributes} & \makecell[l]{Professional hairstyle and makeup\\ websites (\emph{e.g.,} Stylebistro.com)}\\
    \Xhline{1.0pt}
    \end{tabular}
    \label{tab:hairstyle_suggestion_dataset}
\end{table*}


\subsubsection{Performance evaluations}

Yang~\emph{et al.}~\cite{yang:mmm2012} conducted a user study to evaluate the effectiveness of their proposed system, while Liu~\emph{et al.}~\cite{liu:mm2013, liu:tomm14} computed the normalized discounted cumulative gain (NDCG) that measures how close the ranking of the top-\textit{k} recommended styles is to the optimal ranking. However, we are unable to give comparisons on different hairstyle suggestion methods due to inconsistent benchmarks for different papers.
